Benign Overfitting in Out-of-Distribution Generalization of Linear Models

Benign overfitting refers to the phenomenon where an over-parameterized model fits the training data perfectly, including noise in the data, but still generalizes well to the unseen test data. While prior work provides some theoretical understanding of this phenomenon under the in-distribution setup, modern machine learning often operates in a more challenging Out-of-Distribution (OOD) regime, where the target (test) distribution can be rather different from the source (training) distribution. In this work, we take an initial step towards understanding benign overfitting in the OOD regime by focusing on the basic setup of over-parameterized linear models under covariate shift. We provide non-asymptotic guarantees proving that benign overfitting occurs in standard ridge regression, even under the OOD regime when the target covariance satisfies certain structural conditions. We identify several vital quantities relating to source and target covariance, which govern the performance of OOD generalization. Our result is sharp, which provably recovers prior in-distribution benign overfitting guarantee [Tsigler and Bartlett, 2023], as well as under-parameterized OOD guarantee [Ge et al., 2024] when specializing to each setup. Moreover, we also present theoretical results for a more general family of target covariance matrix, where standard ridge regression only achieves a slow statistical rate of $O(1/\sqrt{n})$ for the excess risk, while Principal Component Regression (PCR) is guaranteed to achieve the fast rate $O(1/n)$, where $n$ is the number of samples.

==> introduction_deprecated.tex <==
\section{Introduction}
% In modern machine learning, distribution shift has become a ubiquitous challenge where models trained on a source data distribution are tested on a different target distribution~\citep{zou2018unsupervised,hendrycks2019benchmarking,guan2021domain,koh2021wilds}. Generalization under distribution shift, known as Out-of-Distribution (OOD) generalization, remains a fundamental issue in the practical application of machine learning~\citep{recht2019imagenet,hendrycks2021many,miller2021accuracy,wenzel2022assaying}. While there has been extensive work on the theoretical understanding of OOD generalization, most of it has focused on under-parameterized models~\citep{shimodaira2000improving,lei2021near,DBLP:conf/iclr/GeTFM024,zhang2022class}. However, over-parameterized models, such as deep neural networks and large language models (LLMs), which have more parameters than training samples, are widely used in modern machine learning. Surprisingly, despite the classic bias-variance tradeoff for under-parameterized models, over-parameterized models tend to overfit the data while still achieving strong in-distribution generalization, a phenomenon known as benign overfitting~\citep{muthukumar2020harmless, hastie2022surprises,shamir2023implicit}. Therefore, it is crucial to  theoretically understand how benign overfitting shapes OOD generalization in over-parameterized models.

% It is established in over-parameterized models that ``benign overfitting" occurs when the data essentially resides on a low-dimensional manifold. The manifold assumption~\citep{belkin2003laplacian} is widely applicable across image, speech and language data, where although features are embedded in a high-dimensional ambient space, their generation is governed by a few degrees of freedom imposed by physical constraints~\citep{niyogi2013manifold}. Specifically, the covariance matrix of the data should be characterized by a small number of major directions with large eigenvalues, while the remaining minor directions are high-dimensional but have smaller scale. In this setting, even though the estimator may overfit the noise, it can still capture the signal in the major directions while the noise is dampened in the minor directions. Recent non-asymptotic analyses have provided upper bounds on the excess risk for over-parameterized models under this framework~\citep{bartlett2020benign,hastie2022surprises,DBLP:journals/jmlr/TsiglerB23}.

% However, theoretical characterization of OOD generalization in over-parameterized models remains elusive. For an initial step toward theoretical understanding of OOD generalization in over-parameterized models, we investigate over-parameterized linear models under covariate shift, a standard and widely-studied assumption of OOD generalization, where the marginal distributions of the input covariates $X$ on source and target may differ, but the relationship between the input $X$ and the output $Y$ remains the same across domains. 

% In this paper, we aim to study whether the ``benign overfitting" phenomenon can also happen in OOD generalization. Concretely, this paper makes the following contributions:




% % Recent works \citep{hao2024benefits,mallinar2024minimum} consider the natural scenario where the source covariance matrix $\Sigma_S$ is effectively low rank, so that "benign overfitting" is possible, as shown by \cite{bartlett2020benign}. They provide excess risk upper bounds under this scenario, but they both pose strong assumptions on the target covariance matrix $\Sigma_T$: \cite{hao2024benefits} requires the shift to be characterized by a small $\delta$, namely $\Sigma_T = \Sigma_S + \mathbb{E}\delta\delta^T$. \cite{mallinar2024minimum} assumes the simultaneously diagonalizability of $\Sigma_S$ and $\Sigma_T$, and further requires the whitening samples to have independent coordinates. Those assumptions are overly strong, thus the aformentioned results may not provide a thorough understanding of OOD generalization for over-parameterized linear models under general setups. This leads to a natural question: Can we characterize OOD generalization for over-parameterized linear models, under \emph{general} covariate shift? Namely, can we provide excess risk bounds for \emph{arbitrary} $\Sigma_T$? In this paper, we address this problem by providing sharp excess risk bounds of over-parameterized linear regression under covariate shift. 

% \paragraph{Our contributions} 
% \begin{enumerate}[leftmargin=*]
% \item We give a sharp instance-dependent characterization of the excess risk for ridge regression. Our result holds for any target distribution, only requiring the source distribution to be sub-Gaussian and the tail components to be essentially high-dimension. We show that "benign overfitting" also happens under covariate shift, given that the target distribution’s covariance structure remains dominated by the $k$ major directions. To be specific, we show that ridge regression will achieve a excess risk comparable to the in-distribution setting, if the \emph{overall magnitude} of the target covariance on minor directions scales similarly to or smaller than those of the source, where no special spectral structure of the target covariance is required. Our results recover \cite{DBLP:journals/jmlr/TsiglerB23}'s bound when there is no covariate shift, and also recover \cite{DBLP:conf/iclr/GeTFM024}'s sharp bound for under-parameterized linear regression under covariate shift when the minor components vanish. 
 

% \item We further complement the study by considering the scenario when the target does not retain a similar structure as the source, under which ridge regression does not perform well. Under this scenario, we show that Principal Component Regression (PCR) is guaranteed to have a small excess risk, provided that the true signal almost lies in the major directions of the source. Further more, PCR does not require the minor directions to have high effective rank, which shows its superioirty against ridge regression under certain scenarios.
% \end{enumerate}
In modern machine learning, distribution shift has become a ubiquitous challenge where models trained on a source data distribution are tested on a different target distribution~\citep{zou2018unsupervised,hendrycks2019benchmarking,guan2021domain,koh2021wilds}. Generalization under distribution shift, known as Out-of-Distribution (OOD) generalization, remains a fundamental issue in the practical application of machine learning~\citep{recht2019imagenet,hendrycks2021many,miller2021accuracy,wenzel2022assaying}. While there has been extensive work on the theoretical understanding of OOD generalization, most of it has focused on under-parameterized models~\citep{shimodaira2000improving,lei2021near,DBLP:conf/iclr/GeTFM024,zhang2022class}. However, over-parameterized models, such as deep neural networks and large language models (LLMs) in the fine-tuning stage, which have more parameters than training samples, are widely used in modern machine learning. Surprisingly, despite the classic bias-variance tradeoff for under-parameterized models, over-parameterized models tend to overfit the data while still achieving strong in-distribution generalization, a phenomenon known as benign overfitting~\citep{hastie2022surprises,shamir2023implicit} or harmless interpolation~\citep{muthukumar2020harmless}. Therefore, it is crucial to theoretically understand how benign overfitting shapes OOD generalization in over-parameterized models.

It is established in over-parameterized models that ``benign overfitting" occurs when the data essentially resides on a low-dimensional manifold. The manifold assumption~\citep{belkin2003laplacian} is widely applicable across image, speech, and language data, where although features are embedded in a high-dimensional ambient space, their generation is governed by a few degrees of freedom imposed by physical constraints~\citep{niyogi2013manifold}. Specifically, the covariance matrix of the data should be characterized by several major directions corresponding to large eigenvalues, while the remaining directions are high-dimensional but associated with small eigenvalues. In this setting, even though the estimator may overfit the noise in the low-variance directions, it can still capture the signal along the major directions while the noise is dampened in the minor directions. Recent non-asymptotic analyses have provided upper bounds on the excess risk for the minimum-norm interpolant and over-parameterized ridge estimator under this framework~\citep{bartlett2020benign,hastie2022surprises,DBLP:journals/jmlr/TsiglerB23}.

However, a theoretical understanding of OOD generalization in over-parameterized models remains elusive. In this paper, we take an initial step towards characterizing OOD generalization in over-parameterized models under \emph{general} covariate shift, a standard assumption in the OOD regime~\citep{ben2006analysis}, where the conditional distribution of the outcome given the covariates remains invariant. We derive the first vanishing, non-asymptotic excess risk bound for ridge regression and minimum-norm interpolation, assuming that the source covariance is dominated by a few major eigenvalues, which satisfies the in-distribution benign overfitting condition. Notably, we allow the target covariance to be arbitrary. This result stands in contrast to recent work that either addresses only a restrictive form of covariate shift~\citep{hao2024benefits,mallinar2024minimum} or provides excess risk bounds that asymptotically remain above a constant~\citep{tripuraneni2021provable,hao2024benefits}. 
\chijin{be more careful and explain better about the last two sentences.}

In summary, our excess risk bound identifies several key quantities that relate to the source and target covariance, suggesting that “benign overfitting” occurs when these quantities are well controlled. In such cases, the target distribution data lies on the low-dimensional manifold of the source distribution. Otherwise, ridge regression may incur excess risk, lower bounded by the slow statistical rate of \(\mathcal{O}(1/\sqrt{n})\). In contrast, we show that Principal Component Regression (PCR) achieves the fast rate of \(\mathcal{O}(1/n)\) in such scenarios. 
\ifarxiv
    The non-asymptotic rates of both ridge regression and PCR are validated through simulation experiments on multivariate Gaussian data.
\else
    The non-asymptotic rates of both ridge regression and PCR are validated through simulation experiments on multivariate Gaussian data in Appendix~\ref{sec:simulation_app}.
\fi
% Recent works \citep{hao2024benefits,mallinar2024minimum} consider the natural scenario where the source covariance matrix $\Sigma_S$ is effectively low rank, so that "benign overfitting" is possible, as shown by \cite{bartlett2020benign}. They provide excess risk upper bounds under this scenario, but they both pose strong assumptions on the target covariance matrix $\Sigma_T$: \cite{hao2024benefits} requires the shift to be characterized by a small $\delta$, namely $\Sigma_T = \Sigma_S + \mathbb{E}\delta\delta^T$. \cite{mallinar2024minimum} assumes the simultaneously diagonalizability of $\Sigma_S$ and $\Sigma_T$, and further requires the whitening samples to have independent coordinates. Those assumptions are overly strong, thus the aformentioned results may not provide a thorough understanding of OOD generalization for over-parameterized linear models under general setups. This leads to a natural question: Can we characterize OOD generalization for over-parameterized linear models, under \emph{general} covariate shift? Namely, can we provide excess risk bounds for \emph{arbitrary} $\Sigma_T$? In this paper, we address this problem by providing sharp excess risk bounds of over-parameterized linear regression under covariate shift. 
\chijin{change this paragraph to say case 1 and case 2 to make it crystal clear that we are talking about two settings in this paper.}

\ifarxiv
    \paragraph{Our contributions.}
\else
    \textbf{Our contributions.} 
\fi
\begin{enumerate}[leftmargin=*]
\item We provide a sharp, instance-dependent excess risk bound for ridge regression (Theorem~\ref{theo_maintext:ridge_main}). \chijin{under OOD? add more quantifier to make the first sentence sounds interesting. Classical results of ridge regression have been done for decades, I'm sure this is not what we want to talk about.}
Our result applies to any target distribution, requiring only that the source covariance be dominated by a few major eigenvectors and that the minor components are high-dimensional. We show that ridge regression exhibits “benign overfitting,” achieving excess risk comparable to the in-distribution case, provided that certain key quantities relating to the source and target distributions are bounded. Importantly, this condition requires that the \emph{overall magnitude} of the target covariance along the minor directions scales similarly to, or smaller than, that of the source, but it does not depend on the spectral structure of the target covariance. Our results recover the in-distribution bound from  \cite{DBLP:journals/jmlr/TsiglerB23} when the source and target match and also recover the sharp bound from \cite{DBLP:conf/iclr/GeTFM024} for under-parameterized linear regression under covariate shift when the minor components vanish. 

\item We extend our analysis to examine the scenario where the target distribution exhibits significant variance in the minor directions. In this setting, ridge regression incurs a higher error rate compared to the in-distribution case, specifically the slow statistical rate of $\mathcal O(1/\sqrt n)$ in certain instances (Theorem~\ref{thm:ridge_lower_bound_main}). However, we demonstrate that Principal Component Regression ensures a fast rate of $\mathcal O(1/n)$ in these cases, provided that the true signal primarily lies in the major directions of the source (Theorem~\ref{thm:pcr_upper_bound_main}). Additionally, PCR does not rely on the minor directions of the source distribution being high-dimensional, highlighting its advantage over ridge regression in such settings.
\end{enumerate}
\chijin{It's quite unclear from the description how the setting of 1 is different from the setting of 2. Especially in 1 we say our result applies to any target distribution, in 2 we say the target distribution exhibits xx. It sounds like 2 is a sub case of 1. Please modify the description and make it clear.}

\subsection{Related work}
% over-parameterization
\ifarxiv
    \paragraph{Over-parameterization.}
\else
    \textbf{Over-parameterization.}  
\fi
% Harmless Interpolation, Benign Overfitting, Double Descent
The success of over-parameterized models in machine learning has sparked significant research on their theoretical foundations. Harmless interpolation~\citep{muthukumar2020harmless} or benign overfitting~\citep{shamir2023implicit} describes cases where linear models interpolate noise yet still generalize well. Double descent in prediction error is also observed as the ambient dimension surpasses the number of training samples~\citep{nakkiran2019more,xu2019number}.

Research in this field can be divided into two categories based on assumptions about the spectral structure of the sample covariance.
% isotropic covariance structure, controlled by a constant, asymptoctic, n/d is constant and tend to $\infty$, weak signal, positive ridge regression is optimal, unless SNR tend to infty, impractical in reality
The first category assumes an almost isotropic sample covariance matrix with a bounded condition number or an isotropic prior distribution of parameters~\citep{belkin2020two}.  In this case, a limiting covariance spectral structure may emerge when $n\asymp d$ \chijin{why such setting is called over-parameterization?} and both tend to infinity, allowing for asymptotic risk bounds~\citep{dobriban2018high,richards2021asymptotics}. However, ridgeless regression is sub-optimal in this setting unless the signal-to-noise ratio is infinite~\citep{wu2020optimal}, and non-asymptotic error bounds are lacking.
% Spiked Covariance Model, optimal ridge penalty can be zero due to implicit regularization, more practical gradient descent, non-asymptotic rate bias and variance.
Our work falls into the second category, focusing on the covariance model where a small number of eigenvalues dominate the sample covariance, and the signal is concentrated in the subspace spanned by the leading eigenvectors~\citep{bibas2019new, chinot2022robustness, hastie2022surprises}. Linear regression can be optimal without regularization under this covariance structure~\citep{kobak2020optimal}, which is of practical interest because ridgeless regression is equivalent as gradient descent from zero initialization~\citep{zhou2020uniform}. Sharp non-asymptotic bounds for variance and bias in ridge and ridgeless regression have been derived~ \citep{bartlett2020benign,DBLP:journals/jmlr/TsiglerB23}.

% Uniform Convergence Bound, any sample covariance and hypothesis, strong assumption on gaussian distribution, predicor with given norm or surrogate class with specific structure.
Extending the analysis of ridgeless estimators (i.e., minimum norm interpolants), uniform convergence bounds for generalization error have been studied for all interpolants with arbitrary norms. 
However, uniformly bounding the difference between population and empirical errors generally fails to ensure a consistent predictor~\citep{zhou2020uniform}, necessitating strong assumptions on distributions~\citep{ koehler2021uniform} or hypothesis classes~\citep{negrea2020defense}. 
Over-parameterization theory for linear models has also been applied to two-layer neural networks approximated via kernel ridge regression~\citep{liang2020multiple,ghorbani2020neural,ghorbani2021linearized,bartlett2021deep,mei2022generalizationa,mei2022generalizationb,montanari2022interpolation,simon2023more}, though this lies beyond the scope of the present work.

\ifarxiv
    \paragraph{Out-of-Distribution generalization.}
\else
    \textbf{Out-of-Distribution generalization.}
\fi
% ood: covariate shift, empirical risk minimization/ridgeless regression, linear models, well specified
% underparameterized
Out-of-distribution generalization is well studied for under-parameterized models, particularly in transfer learning between two distributions, where labeled source data is combined with unlabeled target data to train models. For covariate shift, importance weighting~\citep{cortes2010learning,agapiou2017importance} is asymptotically optimal when using density ratio as weights~\citep{shimodaira2000improving}. More generally, the theoretical limits of transfer learning are explored through minimax lower bounds for distribution shifts bounded by divergence metrics~\citep{mousavi2020minimax,zhang2022class}. A number of algorithms are proposed to achieve matching upper bounds~\citep{lei2021near}. However, \citet{DBLP:conf/iclr/GeTFM024} shows that even without target data, vanilla MLE (Empirical Risk Minimization, ERM) is minimax optimal for well-specified models under covariate shift, with a sharp $1/n$ excess risk bound based on Fisher information.

% % non-parametric
% Minimax bounds for transfer learning are also studied in non-parametric settings, primarily under covariate shift~\citep{kpotufe2018marginal}, with respect to hypothesis classes such as Hölder continuous functions~\citep{hanneke2019value,pathak2022new} and RKHSs~\citep{ma2023optimally}. Some of these approaches rely on limited labeled samples from the target distribution~\citep{DBLP:journals/corr/abs-2302-10160}. Distributionally robust optimization~\citep{duchi2019distributionally} is another non-parametric method that directly optimizes the minimax risk over a bounded set of distributions without leveraging target data. Additionally, some methods address concept shift by exploiting the causal structure within the data~\citep{peters2016causal,arjovsky2019invariant}, which falls outside the scope of the present work.

% over-parameterized
Research on over-parameterized models under distribution shift has largely focused on covariate shifts in linear regression. Importance weighting for over-parameterized models~\citep{DBLP:conf/icml/Chen0SC24} and general sample reweighting offer no advantage over ERM since both converge to the same estimator via gradient descent~\citep{zhai2022understanding}. 
% though \citet{DBLP:conf/icml/Chen0SC24} demonstrate a reduction in asymptotic variance when the model is misspecified. 
Consequently, much literature focuses on minimum-norm interpolation as the natural ERM solution.
For isotropic signals, \citet{DBLP:conf/nips/TripuraneniAP21} prove that over-parameterization improves robustness to covariate shift, deriving an asymptotic generalization bound decreasing with $d/n$. Under the covariance model dominated by several major eigenvectors, \citet{hao2024benefits} derive a non-asymptotic bound for a specific instance of covariate shift where features are translated by a constant, but the covariance matrix is preserved. However, a constant excess risk remains in their bound due to estimation variance. \citet{DBLP:journals/tmlr/KausikSS24} study a linear model with additive noise on covariates when data strictly lies in a low-dimensional subspace, also showing a non-vanishing bound. \citet{mallinar2024minimum} investigate minimum-norm interpolation with independent covariates and simultaneously diagonal source and target covariance matrices, allowing them to directly extend in-distribution bounds of \citet{bartlett2020benign,DBLP:journals/jmlr/TsiglerB23}. Still, their estimation bias bound is looser than ours, as it exhibits a gap compared to \cite{DBLP:journals/jmlr/TsiglerB23}'s sharp bound even when the source and target distributions are aligned. In contrast, our work achieves the first vanishing non-asymptotic error bound for general covariate shift, assuming only finite second moments for the target covariance matrix.

Another line of research considers non-parametric models under covariate shift \citep{kpotufe2018marginal,hanneke2019value,pathak2022new,ma2023optimally}, presenting minimax results governed by a transfer-exponent that measures the similarity between source and target distributions. However, this falls outside the scope of our work.

\chijin{I think we can improve a bit on the related work. Currently, the related work is unnecessarily dense/technical with many jargons. We can leave out some highly irrelevant details that we can't explain well in a few words (especially the details of methodology in some works that are not very relevant), and convey more clearly the main message, i.e. categorically what has been done, and what has not been done, where lies our contribution.}


% pcr
\ifarxiv
    \paragraph{Principal Component Regression.}
\else
    \textbf{Principal Component Regression.}
\fi
Principal Component Regression (PCR) has been designed to treat multicollinearity in high-dimensional linear regression, where the covariates possess a latent, low-dimensional representation~\citep{massy1965principal,jeffers1967two,jolliffe1982note,jeffers1981investigation}. PCR has been widely used in statistics \citep{liu2003principal,fan2021robust,fan2023factor}, econometrics \citep{stock2002forecasting, bai2002determining,fan2020factor}, chemometrics \citep{naes1988principal,sun1995correlation,vigneau1997principal,depczynski2000genetic,keithley2009multivariate}, construction management \citep{chan2005project}, environmental science \citep{kumar2011forecasting,hidalgo2000alternative}, signal processing \citep{huang2012improved} and etc. 

Regarding the theory of PCR, \citet{hadi1998some} identify conditions under which PCR will fail. \citet{bair2006prediction} suggest selecting principal components based on their association with the outcome and provide corresponding asymptotic consistency results. 
\citet{xu2019number} establish asymptotic risk bounds for PCR with varying numbers of selected components $k$. They show that the ``double descent" behavior also happens in PCR as $k/d$ increases, where $d$ represents the data dimension. Most relevant to our work, \citet{agarwal2019robustness} derive non-asymptotic error bounds for PCR, and show that the error decays at a rate of $\mathcal{O}(1/\sqrt{n})$ ($n$ is the sample size), assuming all singular values of the data matrix are of similar magnitude. \citet{agarwal2020model} further improves this rate to $\mathcal{O}(1/n)$. However, both results consider a fixed design with strict low-rank assumptions, making them inapplicable to our setting of OOD generalization.




==> loss.tex <==
\section{A Proof with Loss Functions}
% Need to formalize the assumptions. Conjecture assumptions 1,2 suffices to give an upper bound. 

Consider the linear regression problem, where $y = x^T \beta^* +\epsilon$, $\beta^*\in \RR^d$ and $\epsilon \sim \mathcal N(0,1)$. Assume $x$ is a gaussian random vector with zero mean. Define the effective rank of the source covariance matrix as:
\begin{align*}
    r = \frac{\operatorname{tr}(\Sigma_S)}{\|\Sigma_S\|_2}.
\end{align*}
Consider the loss function of ridge regression for samples $\{(x_i,y_i)\}_{i=1}^n$ and some $\lambda > 0$:
\begin{align*}
    \ell_n(\beta) =\left( \frac{1}{n} \sum_{i=1}^n \frac{1}{2} (y_i-x_i^T\beta)^2 \right) + \frac{1}{2} \lambda \|\beta\|^2.
\end{align*}
Consider the ridge estimator:
\begin{align*}
    \hat \beta = \arg\min_\beta \ell_n(\beta).
\end{align*}
\begin{myassumption}
\label{asm:effective_dim}
Let $\tilde \Sigma_S = \Sigma_S +\lambda I_d$.
\begin{align*}
     &\lim_{n\to \infty} \frac{r}{n} = 0. \\
     &\lim_{n\to \infty} \|\tilde \Sigma_S^{-1}\|_2 \|\Sigma_S\|_2 \sqrt{\frac{r}{n}} = 0.
\end{align*}
\end{myassumption}
Let $\epsilon_i = y_i - x_i^T\beta^\star$ and $X = (x_1, ..., x_n)^T \in \mathbb R^{n\times d}$. Compute the gradient and hessian matrix of the loss function:
\begin{align*}
    \nabla \ell_n(\beta^\star) &= - \frac{1}{n} \sum_{i=1}^n  \epsilon_ix_i + \lambda\beta^\star. \\
    \mathbb E[\nabla \ell_n(\beta^\star)] &= \lambda\beta^\star. \\
    \nabla^2  \ell_n(\beta^\star) &= \frac{1}{n} X^TX + \lambda I_d. \\
    \mathbb E[\nabla^2  \ell_n(\beta^\star)] &= \Sigma_S + \lambda I_d.
\end{align*}
\begin{lemma}[Proposition 2 of \cite{koltchinskii2011nuclear}]
\label{lem:vector_bernsterin}
Let \(u, u_1, \dots, u_n\) be i.i.d. mean-zero random vectors. We denote \(V = \mathbb{E}[\|u\|_2^2]\) and
\[
B_u^{(\alpha)} := \inf \left\{ t > 0 : \mathbb{E}\left[\exp\left(\frac{\|u\|^\alpha}{t^\alpha}\right)\right] \leq 2 \right\}, \quad \alpha \geq 1.
\]
Suppose \(B_u^{(\alpha)} < \infty\) for some \(\alpha \geq 1\). Then there exists an absolute constant \(C > 0\) such that for all \(\delta \in (0,1)\), with probability at least \(1 - \delta\):
\[
\left\| \frac{1}{n} \sum_{i=1}^n u_i \right\|_2 \leq C \left( \sqrt{\frac{V \log \frac{d}{\delta}}{n}} + B_u^{(\alpha)}  \left( \log\frac{B_u^{\alpha}}{\sqrt V}\right)^{1/\alpha} \frac{\log \frac{d}{\delta}}{n} \right).
\]
\end{lemma}
\begin{lemma}
\label{lem:gradient_concentration}
There exist $B_1\geq 0$ and an absolute constant $C>0$ such that for any fixed matrix $A\in \mathrm R^{d\times d}$ and any $\delta \in (0,1)$, with probability at least $1-\delta$:
\begin{align*}
    \|A (\nabla \ell_n(\beta^*) - \mathbb{E}[\nabla \ell_n(\beta^*)])\|_2 \leq C \left( \sqrt{\frac{V \log \frac{d}{\delta}}{n}} + B_1 \sqrt{r} \|A\|_2 \log \frac{B_1 \sqrt r \|A\|_2}{\sqrt{V}} \frac{\log \frac{d}{\delta}}{n} \right),
\end{align*}
where $V = \operatorname{tr}(A \Sigma_S A^T)$.
\end{lemma}
\begin{proof}
For any matrix $A\in \mathrm R^{d\times d}$,
\begin{align*}
A(\nabla \ell_n(\beta^\star)) - \mathbb{E}[\nabla \ell_n(\beta^\star)]) = - \frac{1}{n} \sum_{i=1}^n \epsilon_i A x_i.
\end{align*}
Let $u_i = \epsilon_i A x_i$ and $u=\epsilon A x$. Since $\|x\|$ is $c \sqrt {\operatorname{tr}(\Sigma_S)}$ sub-gaussian and $|\epsilon|$ is 1 sub-gaussian, we have $\|u\| \leq  |\epsilon| \|A\|_2  \|x\|$ is $c \|A\|_2 \sqrt {\operatorname{tr}(\Sigma_S)}$ sub-exponential. 

Apply Lemma~\ref{lem:vector_bernsterin} with $\alpha=1$, $B_u^{(\alpha)} = c \|A\|_2 \sqrt {\operatorname{tr}(\Sigma_S)} = c \|A\|_2 \sqrt r \| \Sigma_S \|_2^{1/2}$, and:
\begin{align*}
    V &= \mathbb{E}[\|u\|^2] \\
    &= \frac{1}{n} \sum_{i=1}^n \mathbb E\|\epsilon_i A x_i\|^2 \\
    &= n \mathbb{E}\left[\left\|\frac{1}{n} \sum_{i=1}^n \epsilon_i A x_i \right\|^2\right] \\
    &= n \mathbb{E} \left[ \left( \frac{1}{n} \sum_{i=1}^n \epsilon_i x_i \right)^T A^T A \left( \frac{1}{n} \sum_{i=1}^n \epsilon_i x_i \right) \right] \\
    &= n \mathbb{E}\left[\operatorname{tr}\left(A \left( \frac{1}{n} \sum_{i=1}^n \epsilon_i x_i \right) \left( \frac{1}{n} \sum_{i=1}^n \epsilon_i x_i \right)^T A^T\right) \right] \\
    &= \operatorname{tr}\left(A \mathbb E  \left[ \frac{1}{n} \sum_{i=1}^n \epsilon_i^2 x_ix_i^T  \right] A^T\right ) \\
    &= \operatorname{tr}(A \Sigma_S A^T).
\end{align*}
The third equation follows from $\mathbb E[\epsilon_i A x_i]=0$. The second last equation follows from $\mathbb E[\epsilon_ix_i] = 0$. The last equation follows from $\mathbb E[\epsilon_i^2]=1$.

There exists an absolute constant \(C > 0\) such that for all \(\delta \in (0,1)\), with probability at least \(1 - \delta\):
\begin{align*}
     \|A (\nabla \ell_n(\beta^*) - \mathbb{E}[\nabla \ell_n(\beta^*)])\|_2 &\leq C \left( \sqrt{\frac{V \log \frac{d}{\delta}}{n}} \right.  \\ & \;\;\;\; \left.
     +  c \|A\|_2 \sqrt r \| \Sigma_S \|_2^{1/2} \log \frac{ c \|A\|_2 \sqrt r \| \Sigma_S \|_2^{1/2}}{\sqrt{V}} \frac{\log \frac{d}{\delta}}{n} \right).
\end{align*}
Let $B_1 = c\| \Sigma_S\|_2^{1/2}$ and the proof is complete.
\end{proof}
\begin{lemma}[Corollary 2 of \citet{koltchinskii2017concentration}]
\label{lem:hessian_concentration}
There exists a constant $B_2 > 0$ such that for all $\delta \in (0, e^{-1}) $, with probability at least $1 - \delta$,
\begin{align*}
 \|\nabla^2 \ell_n(\beta^*) - \mathbb{E}[\nabla^2 \ell_n(\beta^*)]\|_2 
&= \|\frac{1}{n}X^TX - \Sigma_S\|_2  \\
&\leq B_2 \|\Sigma_S\|_2 \max \left\{ \sqrt{\frac{r+\log \frac{1}{\delta}}{n}}, \frac{r+\log \frac{1}{\delta}}{n}  \right\}.
\end{align*}
\end{lemma}
\begin{proposition}
Under Assumption~\ref{asm:effective_dim}, for any $\delta\in(0,e^{-1})$ there exist constants $B_1,B_2,C$ and a positive integer $N(\delta)$ such that for any $n>N(\delta)$, with probability at least $1-3\delta$,
\begin{align*}
    \mathcal R(\hat \beta) 
    &\leq 
     8C^2  \frac{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1} \Sigma_T ) \log \frac{d}{\delta}}{n} \\
&\quad + 8C^2 B_1^{2} r \|\Sigma_T^{1/2} \tilde{\Sigma}_S^{-1}\|_2^2 \log^2 \left( \frac{B_1 \sqrt{r}\|\Sigma_T^{1/2} \tilde{\Sigma}_S^{-1}\|_2 }{\sqrt{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1} \Sigma_T)}} \right) \left( \frac{\log \frac{d}{\delta}}{n} \right)^2  \\
&\quad + 4 \lambda^2 \|\Sigma_T^{1/2} \tilde{\Sigma}_S^{-1} \beta^\star\|^2 \\
&\quad + 16 B_2 \| \Sigma_T^{1/2}\tilde{\Sigma}_S^{-1/2} \|_2^2 \|\Sigma_S\|_2 \sqrt{\frac{r + \log \frac{1}{\delta}}{n}} \left( 
    4C^2 \frac{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1}) \log \frac{d}{\delta}}{n} 
     \right.   \\
    & \quad  \left.
    + 4C^2 B_1^{2} r \|\tilde{\Sigma}_S^{-1}\|_2^2 \log^2 \left( \frac{B_1 \sqrt{r} \|\tilde{\Sigma}_S^{-1}\|_2 }{\sqrt{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1})}} \right) \left( \frac{\log \frac{d}{\delta}}{n} \right)^2 
     + 2 \lambda^2 \|\tilde{\Sigma}_S^{-1} \beta^\star\|^2
    \right).
\end{align*}
\end{proposition}
\begin{proof}
By taking $A=\tilde\Sigma_S^{-1}$ in Lemma~\ref{lem:gradient_concentration}, for any $\delta \in (0,e^{-1})$, with probability at least $1-\delta$ we have:
\begin{align}
\begin{split}
\label{eq:gradient_concentration}
& \quad \|\tilde\Sigma_S^{-1} \nabla \ell_n (\beta^\star)\|^2 \\
&\leq 2 \|\tilde\Sigma_S^{-1} (\nabla \ell_n (\beta^\star) - \mathbb{E}[\nabla \ell_n (\beta^\star)])\|^2 
+ 2 \| \lambda\tilde{\Sigma}_S^{-1} \beta^\star \|^2 \\
&\leq 4C^2  \frac{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1}) \log \frac{d}{\delta}}{n} 
+ 4C^2 B_1^{2} r \|\tilde{\Sigma}_S^{-1}\|_2^2 \log^2 \left( \frac{B_1 \sqrt{r}\|\tilde{\Sigma}_S^{-1}\|_2 }{\sqrt{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1})}} \right) \left( \frac{\log \frac{d}{\delta}}{n} \right)^2  \\
&\quad + 2 \lambda^2 \|\tilde{\Sigma}_S^{-1} \beta^\star\|^2.
\end{split}
\end{align}
It follows from Lemma~\ref{lem:hessian_concentration}, for any $\delta \in (0,e^{-1})$, with probability at least $1-\delta$ we have:
\begin{align}
\begin{split}
\label{eq:hessian_concentration}
 \|\nabla^2 \ell_n(\beta^*) - \mathbb{E}[\nabla^2 \ell_n(\beta^*)]\|_2 
&\leq B_2 \|\Sigma_S\|_2 \max \left\{ \sqrt{\frac{r+\log \frac{1}{\delta}}{n}}, \frac{r+\log \frac{1}{\delta}}{n}  \right\} \\
&= B_2 \|\Sigma_S\|_2 \sqrt{\frac{r+\log \frac{1}{\delta}}{n}}.
\end{split}
\end{align}
The last equation follows from $\lim_{n\to \infty} \frac{r}{n} = 0$, according to Assumption~\ref{asm:effective_dim}.

Let $\Delta_\beta = \beta - \beta^\star$. For any $\delta \in (0,e^{-1})$, with probability at least $1-2\delta$, both Equation~\ref{eq:gradient_concentration} and \ref{eq:hessian_concentration} hold. Under such event, we have:
\begin{align}
\begin{split}
\label{eq:regret_upper_bound}
    &\quad \ell_n(\beta) - \ell_n(\beta^\star) \\ 
    &= (\beta - \beta^\star)^T \nabla \ell_n(\beta^\star) + \frac{1}{2} (\beta - \beta^\star)^T \nabla^2\ell_n(\beta^\star)(\beta - \beta^\star) \\
    &\leq (\beta - \beta^\star)^T \nabla \ell_n(\beta^\star) + \frac{1}{2} (\beta - \beta^\star)^T \tilde{\Sigma}_S (\beta - \beta^\star) + B_2 \|\Sigma_S\|_2 \sqrt{\frac{r+\log \frac{1}{\delta}}{n}} \| \beta - \beta^\star \|^2 \\
    &= \frac{1}{2} (\Delta_\beta +\tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star) )^T \tilde{\Sigma}_S (\Delta_\beta +\tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star) )  \\
    &\quad - \frac{1}{2} (\tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star) )^T  \tilde{\Sigma}_S (\tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star) ) 
    + B_2 \|\Sigma_S\|_2 \sqrt{\frac{r+\log \frac{1}{\delta}}{n}} \| \Delta_\beta \|^2.
\end{split}
\end{align}
Similarly, we have:
\begin{align}
\begin{split}
\label{eq:regret_lower_bound}
     &\quad \ell_n(\beta) - \ell_n(\beta^\star) \\ 
    &\geq \frac{1}{2} (\Delta_\beta +\tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star) )^T \tilde{\Sigma}_S (\Delta_\beta +\tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star) ) \\
    &\quad - \frac{1}{2} (\tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star) )^T  \tilde{\Sigma}_S (\tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star) ) 
     - B_2 \|\Sigma_S\|_2 \sqrt{\frac{r+\log \frac{1}{\delta}}{n}} \| \Delta_\beta \|^2.
\end{split}
\end{align}
By taking $\beta = \beta^\star - \tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star)$ in Equation~\ref{eq:regret_upper_bound}, we have:
\begin{align}
\begin{split}
\label{eq:regret_solution}
    &\quad \ell_n(\beta^\star - \tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star)) - \ell_n(\beta^\star) \\
    &\leq  - \frac{1}{2} (\tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star) )^T  \tilde{\Sigma}_S (\tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star) ) 
    + B_2 \|\Sigma_S\|_2 \sqrt{\frac{r+\log \frac{1}{\delta}}{n}} \|  \tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star) \|^2 \\
    &\leq - \frac{1}{2} (\tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star) )^T  \tilde{\Sigma}_S (\tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star) ) 
    + B_2 \|\Sigma_S\|_2 \sqrt{\frac{r+\log \frac{1}{\delta}}{n}} 
    \left( 
    4C^2  \frac{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1}) \log \frac{d}{\delta}}{n} 
    \right. \\
    &\quad \left. 
    + 4C^2 B_1^{2} r \|\tilde{\Sigma}_S^{-1}\|_2^2 \log^2 \left( \frac{B_1 \sqrt{r}\|\tilde{\Sigma}_S^{-1}\|_2 }{\sqrt{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1})}} \right) \left( \frac{\log \frac{d}{\delta}}{n} \right)^2 
     + 2 \lambda^2 \|\tilde{\Sigma}_S^{-1} \beta^\star\|^2
    \right).
\end{split}
\end{align}
Let $E$ be an undetermined coefficient. For any $\beta$ satisfying: 
\begin{align}
\begin{split}
\label{eq:ball}
    \|\Delta_\beta\|^2 &\leq E \left( 
    4C^2  \frac{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1}) \log \frac{d}{\delta}}{n} 
     \right. \\
    &\quad \left. 
    + 4C^2 B_1^{2} r \|\tilde{\Sigma}_S^{-1}\|_2^2 \log^2 \left( \frac{B_1 \sqrt{r}\|\tilde{\Sigma}_S^{-1}\|_2 }{\sqrt{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1})}} \right) \left( \frac{\log \frac{d}{\delta}}{n} \right)^2 
     + 2 \lambda^2 \|\tilde{\Sigma}_S^{-1} \beta^\star\|^2
    \right),
\end{split}
\end{align}
subtracting Equation~\ref{eq:regret_solution} from Equation~\ref{eq:regret_lower_bound} gives:
\begin{align}
\begin{split}
\label{eq:regret_ellipsoid}
     &\quad \ell_n(\beta) - \ell_n(\beta^\star - \tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star)) \\
    &\geq \frac{1}{2} (\Delta_\beta +\tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star) )^T \tilde{\Sigma}_S (\Delta_\beta +\tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star) ) \\
    &\quad - (1+E) B_2 \|\Sigma_S\|_2 \sqrt{\frac{r+\log \frac{1}{\delta}}{n}} \left( 
    4C^2  \frac{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1}) \log \frac{d}{\delta}}{n} 
     \right. \\
    &\quad \left. 
    + 4C^2 B_1^{2} r \|\tilde{\Sigma}_S^{-1}\|_2^2 \log^2 \left( \frac{B_1 \sqrt{r}\|\tilde{\Sigma}_S^{-1}\|_2 }{\sqrt{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1})}} \right) \left( \frac{\log \frac{d}{\delta}}{n} \right)^2 
     + 2 \lambda^2 \|\tilde{\Sigma}_S^{-1} \beta^\star\|^2
    \right).
\end{split}
\end{align}
Consider an ellipsoid:
\begin{align*}
    &  D = \left\{   
    \beta \in \mathbb{R}^d : 
    \frac{1}{2} (\Delta_\beta + \tilde{\Sigma}_S^{-1} \nabla \ell_n(\beta^\star) )^T \tilde{\Sigma}_S (\Delta_\beta + \tilde{\Sigma}_S^{-1} \nabla \ell_n(\beta^\star) ) \right. \\
    & \quad\quad\quad\quad\quad\quad \left. \leq   (1+E) B_2 \|\Sigma_S\|_2 \sqrt{\frac{r + \log \frac{1}{\delta}}{n}} \left( 
    4C^2 \frac{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1}) \log \frac{d}{\delta}}{n} 
     \right. \right.  \\
    & \quad\quad\quad\quad\quad\quad \left. \left.
    + 4C^2 B_1^{2} r \|\tilde{\Sigma}_S^{-1}\|_2^2 \log^2 \left( \frac{B_1 \sqrt{r} \|\tilde{\Sigma}_S^{-1}\|_2 }{\sqrt{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1})}} \right) \left( \frac{\log \frac{d}{\delta}}{n} \right)^2 
     + 2 \lambda^2 \|\tilde{\Sigma}_S^{-1} \beta^\star\|^2
    \right) 
    \right\}.
\end{align*}
For any $\beta \in D$, we have:
\begin{align*}
    &\quad \| \Delta_\beta + \tilde{\Sigma}_S^{-1} \nabla \ell_n(\beta^\star) \|^2 \\
    &\leq \| \tilde{\Sigma}_S^{-1} \|_2 (\Delta_\beta + \tilde{\Sigma}_S^{-1} \nabla \ell_n(\beta^\star) )^T \tilde{\Sigma}_S (\Delta_\beta + \tilde{\Sigma}_S^{-1} \nabla \ell_n(\beta^\star) ) \\
    &\leq 2 \| \tilde{\Sigma}_S^{-1} \|_2 (1+E)
    B_2 \|\Sigma_S\|_2 \sqrt{\frac{r + \log \frac{1}{\delta}}{n}} \left( 
    4C^2 \frac{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1}) \log \frac{d}{\delta}}{n} 
     \right.  \\
    & \quad  \left.
    + 4C^2 B_1^{2} r \|\tilde{\Sigma}_S^{-1}\|_2^2 \log^2 \left( \frac{B_1 \sqrt{r} \|\tilde{\Sigma}_S^{-1}\|_2 }{\sqrt{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1})}} \right) \left( \frac{\log \frac{d}{\delta}}{n} \right)^2 
     + 2 \lambda^2 \|\tilde{\Sigma}_S^{-1} \beta^\star\|^2
    \right). 
\end{align*}
Subsequently, 
\begin{align*}
    &\quad \| \Delta_\beta \|^2  \\
    &\leq 2 \| \Delta_\beta + \tilde{\Sigma}_S^{-1} \nabla \ell_n(\beta^\star) \|^2 + 2  \|\tilde\Sigma_S^{-1} \nabla \ell_n (\beta^\star)\|^2 \\
    &\leq 4 \| \tilde{\Sigma}_S^{-1} \|_2 (1+E)
    B_2 \|\Sigma_S\|_2 \sqrt{\frac{r + \log \frac{1}{\delta}}{n}} \left( 
    4C^2 \frac{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1}) \log \frac{d}{\delta}}{n} 
     \right.  \\
    & \quad  \left.
    + 4C^2 B_1^{2} r \|\tilde{\Sigma}_S^{-1}\|_2^2 \log^2 \left( \frac{B_1 \sqrt{r} \|\tilde{\Sigma}_S^{-1}\|_2 }{\sqrt{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1})}} \right) \left( \frac{\log \frac{d}{\delta}}{n} \right)^2 
     + 2 \lambda^2 \|\tilde{\Sigma}_S^{-1} \beta^\star\|^2
    \right) \\
    &\quad + 
    2 \times \left( 
    4C^2 \frac{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1}) \log \frac{d}{\delta}}{n} 
     \right.  \\
    & \quad  \left.
    + 4C^2 B_1^{2} r \|\tilde{\Sigma}_S^{-1}\|_2^2 \log^2 \left( \frac{B_1 \sqrt{r} \|\tilde{\Sigma}_S^{-1}\|_2 }{\sqrt{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1})}} \right) \left( \frac{\log \frac{d}{\delta}}{n} \right)^2 
     + 2 \lambda^2 \|\tilde{\Sigma}_S^{-1} \beta^\star\|^2
    \right). \\
    &= \left( 4 \| \tilde{\Sigma}_S^{-1} \|_2 (1+E)
    B_2 \|\Sigma_S\|_2 \sqrt{\frac{r + \log \frac{1}{\delta}}{n}} + 2  \right) \times \left( 
    4C^2 \frac{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1}) \log \frac{d}{\delta}}{n} 
     \right.  \\
    & \quad  \left.
    + 4C^2 B_1^{2} r \|\tilde{\Sigma}_S^{-1}\|_2^2 \log^2 \left( \frac{B_1 \sqrt{r} \|\tilde{\Sigma}_S^{-1}\|_2 }{\sqrt{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1})}} \right) \left( \frac{\log \frac{d}{\delta}}{n} \right)^2 
     + 2 \lambda^2 \|\tilde{\Sigma}_S^{-1} \beta^\star\|^2
    \right).
\end{align*}
Let $E=3$. Since $\lim_{n\to \infty} \|\tilde \Sigma_S^{-1}\|_2 \|\Sigma_S\|_2 \sqrt{\frac{r}{n}} = 0$ according to Assumption~\ref{asm:effective_dim}, there exists a positve integer $N(\delta)$ such that for any $n > N(\delta)$, 
\begin{align*}
    4 \| \tilde{\Sigma}_S^{-1} \|_2 (1+E)
    B_2 \|\Sigma_S\|_2 \sqrt{\frac{r + \log \frac{1}{\delta}}{n}} < 1.
\end{align*}
Subsequently, 
\begin{align}
     \| \Delta_\beta \|^2  
     & < E \left( 
    4C^2  \frac{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1}) \log \frac{d}{\delta}}{n} 
     \right. \\
    &\quad \left. 
    + 4C^2 B_1^{2} r \|\tilde{\Sigma}_S^{-1}\|_2^2 \log^2 \left( \frac{B_1 \sqrt{r}\|\tilde{\Sigma}_S^{-1}\|_2 }{\sqrt{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1})}} \right) \left( \frac{\log \frac{d}{\delta}}{n} \right)^2 
     + 2 \lambda^2 \|\tilde{\Sigma}_S^{-1} \beta^\star\|^2
    \right).
\end{align}
Thus, $D$ is a subset of the ball defined by Equation~\ref{eq:ball} for any $n>N(\delta)$. For any $\beta \not \in D$ such that $\beta$ is in the ball defined by Equation~\ref{eq:ball}, it follows from Equation~\ref{eq:regret_ellipsoid}:
\begin{align*}
    &\quad \ell_n(\beta) - \ell_n(\beta^\star - \tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star)) \\
    &\geq \frac{1}{2} (\Delta_\beta +\tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star) )^T \tilde{\Sigma}_S (\Delta_\beta +\tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star) ) \\
    &\quad - (1+E) B_2 \|\Sigma_S\|_2 \sqrt{\frac{r+\log \frac{1}{\delta}}{n}} \left( 
    4C^2  \frac{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1}) \log \frac{d}{\delta}}{n} 
     \right. \\
    &\quad \left. 
    + 4C^2 B_1^{2} r \|\tilde{\Sigma}_S^{-1}\|_2^2 \log^2 \left( \frac{B_1 \sqrt{r}\|\tilde{\Sigma}_S^{-1}\|_2 }{\sqrt{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1})}} \right) \left( \frac{\log \frac{d}{\delta}}{n} \right)^2 
     + 2 \lambda^2 \|\tilde{\Sigma}_S^{-1} \beta^\star\|^2
    \right) \\
    &> 0.
\end{align*}
Since $\beta^\star - \tilde \Sigma_S^{-1} \nabla \ell_n(\beta^\star) \in D$, there exists a local minima of $\ell_n(\beta)$ in $D$. Since $\ell_n(\beta)$ is strictly convex, the global minima $\hat \beta$ is also in $D$.

So far we have proved for any $\delta \in (0,e^{-1})$ there exists a positive integer $N(\delta)$ such that for any $n>N(\delta)$, $\hat \beta \in D$ with probability at least $1-2\delta$. It follows:
\begin{align*}
    &\quad \| \tilde\Sigma_S^{1/2} (\Delta_{\hat \beta} + \tilde{\Sigma}_S^{-1} \nabla \ell_n(\beta^\star)) \|^2 \\
    &\leq 2\times (1+E) B_2 \|\Sigma_S\|_2 \sqrt{\frac{r + \log \frac{1}{\delta}}{n}} \left( 
    4C^2 \frac{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1}) \log \frac{d}{\delta}}{n} 
     \right.   \\
    & \quad  \left.
    + 4C^2 B_1^{2} r \|\tilde{\Sigma}_S^{-1}\|_2^2 \log^2 \left( \frac{B_1 \sqrt{r} \|\tilde{\Sigma}_S^{-1}\|_2 }{\sqrt{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1})}} \right) \left( \frac{\log \frac{d}{\delta}}{n} \right)^2 
     + 2 \lambda^2 \|\tilde{\Sigma}_S^{-1} \beta^\star\|^2
    \right) \\
    &= 8 B_2 \|\Sigma_S\|_2 \sqrt{\frac{r + \log \frac{1}{\delta}}{n}} \left( 
    4C^2 \frac{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1}) \log \frac{d}{\delta}}{n} 
     \right.   \\
    & \quad  \left.
    + 4C^2 B_1^{2} r \|\tilde{\Sigma}_S^{-1}\|_2^2 \log^2 \left( \frac{B_1 \sqrt{r} \|\tilde{\Sigma}_S^{-1}\|_2 }{\sqrt{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1})}} \right) \left( \frac{\log \frac{d}{\delta}}{n} \right)^2 
     + 2 \lambda^2 \|\tilde{\Sigma}_S^{-1} \beta^\star\|^2
    \right).
\end{align*}

According to Lemma~\ref{lem:gradient_concentration}, we have with probability at least $1-\delta$:
\begin{align*}
   & \quad \|\Sigma_T^{1/2} \tilde\Sigma_S^{-1} \nabla \ell_n (\beta^\star)\|^2 \\
   &\leq 2 \| \Sigma_T^{1/2} \tilde\Sigma_S^{-1} (\nabla \ell_n (\beta^\star) -\mathbb E[\nabla \ell_n (\beta^\star) ] )  \|^2 
   + 2 \| \lambda \Sigma_T^{1/2} \tilde\Sigma_S^{-1} \beta^\star  \|^2 \\
   &\leq 4C^2  \frac{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1} \Sigma_T ) \log \frac{d}{\delta}}{n} \\
&\quad + 4C^2 B_1^{2} r \|\Sigma_T^{1/2} \tilde{\Sigma}_S^{-1}\|_2^2 \log^2 \left( \frac{B_1 \sqrt{r}\|\Sigma_T^{1/2} \tilde{\Sigma}_S^{-1}\|_2 }{\sqrt{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1} \Sigma_T)}} \right) \left( \frac{\log \frac{d}{\delta}}{n} \right)^2  
+ 2 \lambda^2 \|\Sigma_T^{1/2} \tilde{\Sigma}_S^{-1} \beta^\star\|^2.
\end{align*}
Thus, for any $\delta\in(0,e^{-1})$ there exists a positive integer $N(\delta)$ such that for any $n>N(\delta)$, with probability at least $1-3\delta$,
\begin{align*}
    &\quad \mathcal R(\hat \beta) \\
    &= \| \Sigma_T^{1/2} (\hat \beta - \beta^\star) \|^2  \\
    &\leq 2 \| \Sigma_T^{1/2} (\Delta_{\hat \beta} + \tilde{\Sigma}_S^{-1} \nabla \ell_n(\beta^\star)) \|^2
    +  2 \|\Sigma_T^{1/2} \tilde\Sigma_S^{-1} \nabla \ell_n (\beta^\star)\|^2  \\
    &\leq  2 \| \Sigma_T^{1/2}\tilde{\Sigma}_S^{-1/2} \|_2^2 \| \tilde{\Sigma}_S^{1/2} (\Delta_{\hat \beta} + \tilde{\Sigma}_S^{-1} \nabla \ell_n(\beta^\star)) \|^2
    +  2 \|\Sigma_T^{1/2} \tilde\Sigma_S^{-1} \nabla \ell_n (\beta^\star)\|^2 \\
    &\leq 16 B_2 \| \Sigma_T^{1/2}\tilde{\Sigma}_S^{-1/2} \|_2^2 \|\Sigma_S\|_2 \sqrt{\frac{r + \log \frac{1}{\delta}}{n}} \left( 
    4C^2 \frac{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1}) \log \frac{d}{\delta}}{n} 
     \right.   \\
    & \quad  \left.
    + 4C^2 B_1^{2} r \|\tilde{\Sigma}_S^{-1}\|_2^2 \log^2 \left( \frac{B_1 \sqrt{r} \|\tilde{\Sigma}_S^{-1}\|_2 }{\sqrt{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1})}} \right) \left( \frac{\log \frac{d}{\delta}}{n} \right)^2 
     + 2 \lambda^2 \|\tilde{\Sigma}_S^{-1} \beta^\star\|^2
    \right) \\
    &\quad + 8C^2  \frac{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1} \Sigma_T ) \log \frac{d}{\delta}}{n} \\
&\quad + 8C^2 B_1^{2} r \|\Sigma_T^{1/2} \tilde{\Sigma}_S^{-1}\|_2^2 \log^2 \left( \frac{B_1 \sqrt{r}\|\Sigma_T^{1/2} \tilde{\Sigma}_S^{-1}\|_2 }{\sqrt{\operatorname{tr}(\tilde{\Sigma}_S^{-1} \Sigma_S \tilde{\Sigma}_S^{-1} \Sigma_T)}} \right) \left( \frac{\log \frac{d}{\delta}}{n} \right)^2  
+ 4 \lambda^2 \|\Sigma_T^{1/2} \tilde{\Sigma}_S^{-1} \beta^\star\|^2.
\end{align*}

\end{proof}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> pcr_deprecated.tex <==
\section{Results for high-dimensional shift}
In the previous section, we established an upper bound for overparameterized ridge regression under covariate shift. As we have mentioned, ridge regression will achieve the same error rate as in \cite{DBLP:journals/jmlr/TsiglerB23} under the ``low-dimensional shift" scenario, where the last $d-k$ components of the target covariance matrix $\Sigma_T$ scale similarly to or smaller than those of the source. However, when the shift is ``high-dimensional", namely the target covariance matrix can have many large eigenvalues whose corresponding eigenvectors do not lie in the top-$k$ subspace of the source, the guarantee for ridge regression deteriorates. In the section, we will further demonstrate the inadequacy of ridge regression under this scenario, by providing a lower bound for ridge regression under ``high-dimensional shift", i.e., $\|\Sigma_{T, -k}\|$ is large.  
 

Given ridge regression's  incapability, it is natural to consider alternative algorithms that can achieve small excess risk under this scenario. We will show that, even though $\|\Sigma_{T, -k}\|$ is large, principal component regression (PCR) can still be guaranteed to have a small excess risk, provided that the signal $\beta^{\star}$ nearly lies in subspace spanned by the top-$k$ eigenvectors of $\Sigma_S$.


\subsection{Lower bound for ridge regression}
In this subsection, we will show the incapability for ridge regression when $\|\Sigma_{T, -k}\|$ is large. For simplicity, we consider the case $\Sigma_T = I_d$. The excess risk for $\hat{\beta}$ is then $\mathbb{E}_{\epsilon}[(\hat{\beta} - \beta^{\star})^T \Sigma_T (\hat{\beta} - \beta^{\star})] = \mathbb{E}_{\epsilon}\|\hat{\beta} - \beta^{\star}\|^2$. Recall the bias-variance decomposition $\mathbb{E}_{\epsilon}\|\hat{\beta} - \beta^{\star}\|^2  := B +  V,$
where $B=\frac{\lambda^2}{n^2}\|(\hat\Sigma_S + \frac{\lambda}{n} I_d)^{-1} \beta^{\star}\|^2$ is the bias ,$V=  \frac{v^2}{n} \Tr((\hat\Sigma_S + \frac{\lambda}{n} I_d)^{-2} \hat\Sigma_S )$ is the variance, and $\hat\Sigma_S = \frac{1}{n} X^T X$ is the sample covariance. 
% One can see that in order to achieve a $\mathcal{O}(1/n)$ rate as in underparameterized linear regression, we need to choose a regularization parameter $\lambda \leq \sqrt{n}$ so that the bias will not be too large. 
In the following we will show that for certain instances, when choosing a standard regularization parameter $\lambda = \sqrt{n}$, the variance will be greater than some constant, leading to a non-vanishing excess risk. Further more, we will show that no matter how we choose $\lambda$, ridge regression will still suffer from a loss of at least $1/\sqrt{n}$. 


\begin{theorem}\label{thm:ridge_lower_bound}
There exist an instance of $\Sigma_S$ which has a low effective rank, such that when $n$ is larger than some constant $N > 0$, with probability $1-\delta$,
$\frac{V}{v^2} \geq C$ for some constant $C>0$ when choosing $\lambda= \sqrt{n}$. Further more, when $\lambda \leq n^{3/4}$, we have $\frac{V}{v^2} \geq \frac{C}{\sqrt{n}}$. When $\lambda \geq n^{3/4}$, $B \geq \frac{\|\beta^{\star}\|^2}{9\sqrt{n}}$.
\end{theorem}



% \begin{theorem} \label{thm:ridge_lower_bound}
% Suppose $\lambda_1, \cdots, \lambda_d$ satisfies $\lambda_1=\cdots=\lambda_k=1$, $\lambda_{k+1} = \cdots = \lambda_{k+\lfloor \sqrt{n}/C_2 \rfloor} = C_1/\sqrt{n}$, $\lambda_{k+ \lfloor \sqrt{n}/C_2 \rfloor +1} = \cdots = \lambda_{d} = 0 $. Also assume $\sigma = 1$, $C_2 \geq C_1 ((\frac{C_1}{4C})^2 - k -\log \frac{1}{\delta})^{-1}$ for some absolute constant $C$, and $n \geq (\frac{3C_1}{2})^4$. \jiayuncomment{We need $(C_1/4C)^2>k+\log(1/\delta)$. Shall we clarify $C_1,C_2$'s dependence on $k$? Or just set $C_1,C_2$ to fixed value.}  When $\lambda \leq n^{3/4}$, with probability at least $1-\delta$, we have $\frac{V}{v^2} \geq \frac{C'}{\sqrt{n}}$, where $C'>0$ is some absolute constant. When $\lambda \geq n^{3/4}$, with probability at least $1-\delta$, $B \geq \frac{\|\beta^{\star}\|^2}{3\sqrt{n}}$. \jiayuncomment{Typo: $\|\beta^\star\|^2$. Same in appendix.}
% \end{theorem}

% The instance in Theorem \ref{thm:ridge_lower_bound} is constructed as the following. $\lambda_1, \cdots, \lambda_d$ satisfies $\lambda_1=\cdots=\lambda_k=1$, $\lambda_{k+1} = \cdots = \lambda_{k+\lfloor \sqrt{n}/C_2 \rfloor} = C_1/\sqrt{n}$, $\lambda_{k+ \lfloor \sqrt{n}/C_2 \rfloor +1} = \cdots = \lambda_{d} = 0 $. Under this instance, in contrast to the "benign overfitting" regime that our Theorem \ref{theo_maintext:ridge_main} considers, ridge regression, or the minimum norm interpolating solution, will have a large excess risk. The reason is that although the signal from the essentially low-dimensional subspace of data is effectively learned, the learning of the true signal on the essentially high-dimensional component is very difficult, since the source distribution has very small components on these directions. However, the learned signal on the essentially high-dimensional component appears to be crucial in this case, since the target distribution has non-vanishing components on these directions. This can be further illustrated through applying Theorem \ref{theo_maintext:ridge_main} to the source distribution instance in Theorem \ref{thm:ridge_lower_bound}. 
% Firstly, if the first $k$ components of the target is of the same order as the source, and the last $d-k$ components of the target vanish, i.e.,  $\Sigma_{T,-k} = 0$, plug in $\lambda_1, \cdots, \lambda_k$ to Theorem \ref{theo_maintext:ridge_main},we have the following upper bound when $\beta^{\star}_{-k} = 0$: $V \leq \mathcal{O}(\frac{k}{n})$, $B \leq \mathcal{O}(\|\beta^{\star}_{k}\|^2 \frac{\lambda^2}{n^2})$. One can see that when $\lambda \leq \sqrt{n}$, the excess risk will be upper bounded by $\mathcal{O}(1/n)$. However, when $\Sigma_T = I_d$, the upper bounds are $V \leq \mathcal{O}(\frac{k}{n} + \frac{n}{\lambda^2})$ and $B \leq \mathcal{O}(\|\beta^{\star}_{k}\|^2 \frac{\lambda^2}{n^2}(1 + \frac{n}{\lambda}) )$. Therefore when choosing $\lambda = \sqrt{n}$, the guarantee for variance becomes a constant. And when $\lambda \leq n^{3/4}$, the guarantee for variance is at least $\mathcal{O}(1/\sqrt{n})$. As for the bias, when  $\lambda \geq n^{3/4}$, the upper bound for bias becomes $\mathcal{O}(n^{-1/4})$. We can see that when $\|\Sigma_{T,-k}\|$ becomes larger, the upper bound we can derive exhibits a significant deterioration. In fact, this deterioration can be further justified by our lower bound. Theorem \ref{thm:ridge_lower_bound} shows that, under the scenario that $\Sigma_T = I_d$, when $\lambda \geq n^{3/4}$, we have $B \geq \Omega(\frac{1}{\sqrt{n}})$, and when $\lambda \leq n^{3/4}$, we have $V \geq \Omega(\frac{1}{\sqrt{n}})$. Therefore the excess risk will always be lower bounded by $1/\sqrt{n}$, significantly worse than the rate achieved by ridge regression when $\Sigma_{T,-k} = 0$. However, alternative algorithm, such as principal component regression, can achieve $\mathcal{O}(1/n)$ rate under this instance even when $\Sigma_T = I_d$, as we will show in the next subsection.



The instance in Theorem \ref{thm:ridge_lower_bound} is constructed as follows: $\lambda_1, \dots, \lambda_d$ satisfy $\lambda_1 = \dots = \lambda_k = 1$, $\lambda_{k+1} = \dots = \lambda_{k + \lfloor \sqrt{n}/C_2 \rfloor} = C_1/\sqrt{n}$, and $\lambda_{k + \lfloor \sqrt{n}/C_2 \rfloor + 1} = \dots = \lambda_d = 0$. In contrast to the “benign overfitting” regime in Theorem \ref{theo_maintext:ridge_main}, ridge regression will have a large excess risk under this instance. Although the signal from the low-dimensional subspace is effectively learned, learning the true signal in the essentially high-dimensional components is difficult because the source distribution has small components in those directions. However, the learned signal in the essentially high-dimensional components is crucial since the target distribution has non-negligible components in these directions. Applying Theorem \ref{theo_maintext:ridge_main} to this instance, if the last $d-k$ components of the source and the signal are both vanished, i.e., $\Sigma_{T,-k} = 0$ and $\beta^{\star}_{-k} = 0$, we get upper bounds of $V \leq \mathcal{O}(\frac{k}{n})$ and $B \leq \mathcal{O}(\|\beta^{\star}_{k}\|^2 \frac{\lambda^2}{n^2})$. For $\lambda \leq \sqrt{n}$, the excess risk is bounded by $\mathcal{O}(1/n)$. However, when $\Sigma_T = I_d$, the upper bounds become $V \leq \mathcal{O}(\frac{k}{n} + \frac{n}{\lambda^2})$ and $B \leq \mathcal{O}(\|\beta^{\star}_{k}\|^2 \frac{\lambda^2}{n^2}(1 + \frac{n}{\lambda}))$. Choosing $\lambda = \sqrt{n}$ makes the variance a constant, and for $\lambda \leq n^{3/4}$, the variance guarantee is at least $\mathcal{O}(1/\sqrt{n})$. When $\lambda \geq n^{3/4}$, the bias upper bound becomes $\mathcal{O}(n^{-1/4})$. As $\|\Sigma_{T,-k}\|$ increases, the upper bound worsens significantly. This deterioration is further supported by the lower bound in Theorem \ref{thm:ridge_lower_bound}. It shows that for $\Sigma_T = I_d$, $B \geq \Omega(1/\sqrt{n})$ when $\lambda \geq n^{3/4}$, and $V \geq \Omega(1/\sqrt{n})$ when $\lambda \leq n^{3/4}$. Hence, the excess risk when $\Sigma_T = I_d$ is always lower bounded by $1/\sqrt{n}$, worse than rate when $\Sigma_{T,-k} = 0$. However, methods like principal component regression can achieve $\mathcal{O}(1/n)$ under this instance, even with $\Sigma_T = I_d$, as shown in the next subsection.







% \begin{remark}
% Theorem \ref{thm:ridge_lower_bound} shows that, when $\lambda \geq n^{3/4}$, we have $B \geq \Omega(\frac{1}{\sqrt{n}})$, and when $\lambda \leq n^{3/4}$, we have $V \geq \Omega(\frac{1}{\sqrt{n}})$. Therefore the excess risk $\mathbb{E}_{\epsilon}\|\hat{\beta} - \beta^{\star}\|^2  = B + V $ will always be lower bounded by $1/\sqrt{n}$. 


% This means in general the $O(1/n)$ rate \jiayuncomment{In general Barlett's i.i.d. result also doesn't achieve 1/n rate. Shall we say $n<r_k$ in this setting, so applying Theorem 1 gives 1/n rate if $\|\Sigma_{T,-k}\|$ is small. Then we highlight ridge can achieve poorer error rate than over-parameterized in-distribution generalization in the scenario where $\|\Sigma_{T,-k}\| = O(1)$. } (achievable by OLS and ridge regression when underparameterized) can not always be achieved by ridge regression under the overparameterized scenario. \jiayuncomment{Possible explanation about failure of ridge. Only interpolating the signals in the high-dimensional components....}
% \end{remark}


\subsection{Upper bound for principal component regression}
From previous discussions we see the limitation of ridge regression under covariate shift. A natural question arising is, whether it is possible to specify certain conditions that OOD generalization is possible, and design suitable algorithms for addressing OOD generalization, under the scenario where $\|\Sigma_{T,-k}\|$ is large?

We begin with specifying appropriate conditions. If some component of $\Sigma_S$ is very small, i.e., $\lambda_i \approx 0$, it essentially means $y = x^T \beta^{\star} + \epsilon$ will contain very little information about $\beta^{\star}_i$, the $i$-th component of the true signal. Therefore either the corresponding component of $\Sigma_T$ should be small (so that this component will not contribute heavily to the excess risk) or we have some prior knowledge about the true signal, otherwise OOD generalization can be hard to achieve. The former one is the  ``low-dimensional shift" scenario, under which ridge regression works, as the previous section shows. For the latter one, we consider
the scenario where the true signal $\beta^{\star}$ almost lies in the subspace spanned by the top-$k$ eigenvectors of $\Sigma_S$. Namely, on the directions that $\Sigma_S$ has small eigenvalues, $\beta^{\star}$ also has small components.

Under this scenario, a very natural algorithm is the principal component regression (PCR), i.e., we first estimate the top-$k$ subspace of $\Sigma_S$ and project data onto this subspace. Then we do usual linear regression on the projected data, and finally project back to the original space. To be specific, for simplicity we assume we have a sample size of $2n$, and in the first step we obtain an estimator $\hat{U} \in \mathbb{R}^{d \times k}$ of the top-$k$ subspace represented by $U = 
\begin{pmatrix}
I_k  \\
0 
\end{pmatrix} \in \mathbb{R}^{d \times k}
$, by using principal component analysis on the sample covariance matrix $\hat\Sigma_S := \frac1n XX^T = \frac{1}{n}\sum_{i=1}^{n}x_{i}x_{i}^{T}$, namely $\hat{U} = (\hat{u}_1, \cdots, \hat{u}_k)$ where $\hat{u}_i$ is the $i$-th eigenvector of $\hat\Sigma_S$. In the second step, after obtaining $\hat{U}$, we do linear regression on the projected (second half) data. With a little abuse of notation, we use $X\in \mathbb{R}^{n \times d}$ to denote the data matrix $(x_{n+1}, \cdots, x_{2n})^{T}$, and $Y \in \mathbb{R}^{n}$ to denote $(y_{n+1}, \cdots, y_{2n})^{T}$. If we let $Z:= X\hat{U} \in \mathbb{R}^{n \times k}$ be the projected data matrix, the estimator $\hat{\beta}$ we obtained is given by
\begin{align*}
\hat{\beta} = \hat{U} (Z^T Z)^{-1}Z^T Y 
= \hat{U} (\hat{U}^TX^{T}X\hat{U})^{-1}\hat{U}^TX^{T}Y.
\end{align*}
We have the following upper bound for the excess risk of PCR:
\begin{theorem} \label{thm:pcr_upper_bound} Under the setting in Section \ref{sec:setup}, when $n \gtrsim \sigma^{8}(r + \log \frac{1}{\delta})  (\frac{\lambda_1}{\lambda_k - \lambda_{k+1}})^2 \frac{\lambda_1^2 k^2\|\Sigma_{T}\|^2}{\lambda_k^4 \Tr (\mathcal{T})^2}$, then with probability at least $1-\delta$, the excess risk of PCR estimator $\hat{\beta}$ can be upper bounded by
\begin{align*}
  \frac{V}{v^2} & \leq \mathcal{O}(\frac{\Tr (\mathcal{T})}{n}), \\
  B & \leq \mathcal{O} ((\frac{\lambda_{k+1}}{\lambda_k})\|\Sigma_{T,k} \|\|\beta_{-k}^{\star}\|^2  + \beta^{\star T}_{-k} \Sigma_{T,-k} \beta^{\star}_{-k}
  \\ 
& + \sigma^8 ( \frac{\lambda_1}{\lambda_k - \lambda_{k+1}})^2 (\frac{\lambda_1}{\lambda_k})^2\|\Sigma_T\| (  \frac{r + \log{\frac{1}{\delta}}}{n})\|\beta^{\star}_{k}\|^2),
\end{align*}
where we define the variance as $V:=\EE_{\boldsymbol{\epsilon}} \big\|\hbeta(\boldsymbol{\epsilon}) \big\|_{\Sigma_T}^2$ and the bias as $B:=\big\|\hbeta(X\beta^\star)-\beta^\star\big\|_{\Sigma_T}^2$.

% \begin{align*}
%   \mathbb{E}_{\epsilon} \|\hat{\beta}-\beta^{\star}\|_{\Sigma_T}^2 & \leq \mathcal{O} (\frac{v^2}{n} \Tr (\mathcal{T})+ (\frac{\lambda_{k+1}}{\lambda_k})\|\Sigma_{T,k} \|\|\beta_{-k}^{\star}\|^2  + \beta^{\star T}_{-k} \Sigma_{T,-k} \beta^{\star}_{-k}
%   \\ 
% & + \sigma^8 ( \frac{\lambda_1}{\lambda_k - \lambda_{k+1}})^2 (\frac{\lambda_1}{\lambda_k})^2\|\Sigma_T\| (  \frac{r + \log{\frac{1}{\delta}}}{n})\|\beta^{\star}_{k}\|^2)
% \end{align*}


% \jiayuncomment{Overfull equation. Consider writing B,V separately for better presentation.}

% where $r = \frac{\sum_{i=1}^{d} \lambda_i}{\lambda_1}$.
\end{theorem}



% \begin{remark}
% An intermediate result for proving Theorem \ref{thm:pcr_upper_bound} is that we can establish an upper bound given an upper bound of the estimation error $\Delta := \text{dist}(\hat{U}, U) = \|UU^T - \hat{U}\hat{U}^T\|$ (in this case $\hat{U}$ not necessarily comes from the first half of data). For those who are interested, see Lemma \ref{step2_lemma} in the appendix.
% \end{remark}

\begin{remark}
The variance term $\frac{\tr (\mathcal{T})}{n}$ also appears in the first term of variance in Theorem \ref{theo_maintext:ridge_main},and exactly matches the $\tr[\Sigma_S^{-1}\Sigma_T]/n$ rate for under-parameterized linear regression under covariate shift~\citep{DBLP:conf/iclr/GeTFM024}. As for the bias terms, the first two terms $ (\frac{\lambda_{k+1}}{\lambda_k})\|\Sigma_{T,k} \|\|\beta_{-k}^{\star}\|^2$ and $\beta^{\star T}_{-k} \Sigma_{T,-k} \beta^{\star}_{-k}$ correspond to the bias in the first $k$ components and the last $d-k$ components respectively, which are incurred by a non-vanishing $\beta^{\star}_{-k}$. The aforementioned terms are in general not largely affected by $\Delta := \text{dist}(\hat{U}, U) = \|UU^T - \hat{U}\hat{U}^T\|$, the error when estimating the top-$k$ subspace. However, the remaining term $\sigma^8 ( \frac{\lambda_1}{\lambda_k - \lambda_{k+1}})^2 (\frac{\lambda_1}{\lambda_k})^2\|\Sigma_T\| (  \frac{r + \log{\frac{1}{\delta}}}{n})\|\beta^{\star}_{k}\|^2$, the bias term in first $k$ component that is caused by the estimation error of the top-$k$ subspace, is largely affected by $\Delta$. Lemma \ref{bias_term} shows that this term is bounded by $\mathcal{O} (\|\beta^{\star}_{k}\|^2 \Delta^2 (\frac{\lambda_1}{\lambda_k})^2\|\Sigma_T\|)$, that is, it has a quadratic dependence on $\Delta$. As for controlling $\Delta$, we have Lemma \ref{Delta_lemma} showing that
$\Delta \lesssim \sigma^4 (\frac{r + \log{\frac{1}{\delta}}}{n}) (\frac{\lambda_1}{\lambda_k - \lambda_{k+1}})$. We can see that $\Delta$ is mainly affected by the effective rank $r = \lambda_1^{-1}(\sum_{i=1}^{d}\lambda_i)$ and the eigenvalue gap $\lambda_k - \lambda_{k+1}$.
\end{remark}

% \begin{remark}[Choosing $k$.]
% The correctnumber of principal components k to use is
% not known a priori. However, under reasonable signal-to-noise scenarios, Weyl’s inequality
% implies that a “sharp” threshold or gap should exist between the top r singular values and remaining singular values of the observed data Ze. This gives rise to a natural “elbow” point and
% suggests choosing a threshold within this gap. Another standard approach is to use a “universal” thresholding scheme that preserves singular values above a precomputed threshold ([7]
% and [11]). Data-driven approaches developed around cross-validation can also be employed.
% \end{remark}



Theorem \ref{thm:pcr_upper_bound} demonstrates the effectiveness of PCR in achieving low excess risk under the aforementioned scenario (i.e., $\|\Sigma_{T,-k}\|$ is large, while the true signal almost lies in the top-$k$ subspace of $\Sigma_S$). Consider the case where $\beta^{\star}_{-k} = 0$, i.e., the true signal $\beta^{\star}$ completely lies in the top-$k$ subspace of $\Sigma_S$. In this case, the first two terms of the bias will be zero. Under the "spiked covariance model", where the last $d-k$ components of the source are small, when $k, \|\Sigma_T\|, \lambda_1, \lambda_k$ are all $\Theta(1)$, the variance term scales as $1/n$, and the remaining bias term becomes $\mathcal{O}( \frac{r}{n} \|\Sigma_T\|\|\beta^{\star}_{k}\|^2)$, which means the excess risk for PCR will be bounded by $\mathcal{O}( \frac{r}{n} \|\Sigma_T\|\|\beta^{\star}_{k}\|^2)$. As an example, under the assumptions of Theorem \ref{thm:ridge_lower_bound}, $r = k +\frac{C_1}{C_2}$, therefore PCR will achieve a $\mathcal{O}(1/n)$ rate even when $\Sigma_T = I_d$. Comparing with the excess risk for ridge regression, which is at least $1/\sqrt{n}$, PCR shows its superiority against ridge regression under the ``high-dimensional shift" scenario.

% A further example is the case we considered in the previous section,
% \shange{mention the upper bound by ridge}

% i.e., $k~=~\mathcal O(1)$, $\lambda_{k+1}^{-1}\sum_{j=1}^{d}\lambda_j =\Omega(n^2)$, $\sum_{j>k}\lambda_j = \mathcal O(\sqrt {n})$. Under this scenario $r$ becomes $\mathcal{O}(\sqrt{n})$ and $\lambda_{k+1} \leq \mathcal O(n^{-3/2})$. And if the eigenvalue gap is larger than a constant (this holds when $\lambda_k = \Omega(1)$), PCR will achieve a $1/\sqrt{n}$ rate. 





% Here the columns of $\hat{U}$ are the basis of the estimated $k-$dimensional subspace. 

% We denote the distance between the estimated subspace and the original one by $\Delta:=\text{dist}(U, \hat{U})= \|UU^T -\hat{U}\hat{U}^T\|$.

==> ridge_deprecated.tex <==
\section{Over-parameterized ridge regression}
% add discussion: 1. overparameterization improve robustness to shift (bias)
% 2. from minimum-norm interpolant to ridge regression
% 3. Barlett theorem
% why ridge regression: successful for overparameterization without shift. investigate under covariate shift.
% summarize what we do: a bound for overparameterized ridge under covariate shift 1) where the rank structure is preserved: tail components shall still be tail (not essentially high dimension). 2) well reduce to barlett and covariate shift.
When the covariance matrix has a low effective rank, \cite{DBLP:journals/jmlr/TsiglerB23} demonstrates that the minimum-norm interpolant can effectively learn the signal from the essentially low-dimensional subspace of data while suppressing noise from the essentially high-dimensional components. Their results extend to ridge regression by demonstrating that the high-dimensional components inherently provide implicit regularization, similar to ridge. In this section, we explore whether the mechanism holds under covariate shift and derive upper bounds for the excess risk of the ridge estimator, where the source covariance has a low-rank structure but the target covariance matrix may or may not share the same low-rank structure as the source. Our analysis applies to the over-paramerized setting where $k<n<r_k$.
\subsection{Warm-up: in-distribution benign overfitting}
% introduce assumption, cite barlett.  
\citet{DBLP:journals/jmlr/TsiglerB23} assume that the data consists of $k$ essentially low-dimensional components and $d-k$ essentially high-dimensional components. In other words, the covariance matrix of the source distribution has a high effective rank relative to the sample size, once the $k$ low-dimensional components are removed. This intuition is formalized through an assumption that controls the condition number of the Gram matrix for the remaining $d-k$ dimensions.
\begin{myassumption}[CondNum$(k,\delta,L)$, \citep{DBLP:journals/jmlr/TsiglerB23}]
\label{assum_maintext:condNum}
    Define a matrix $A_k = \lambda I_n + X_{-k}X_{-k}^T$. With probability at least $1-\delta$, $A_k$ is positive definite and has a condition number no greater than $L$, i.e.,
    \begin{align*}
        \frac{\mu_1(A_k)}{\mu_n(A_k)} \leq L.
    \end{align*}
\end{myassumption}
% implies essentially high dimension. sufficient and necessary condition.
\begin{remark}
The assumption holds if the effective rank for the last $d-k$ dimensions is significantly larger than $n$. As evidence, \citet{DBLP:journals/jmlr/TsiglerB23}~(Lemma 3) provides a sufficient and almost necessary condition for the condition number of $A_k$ to be smaller than $L$: $r_k~\gtrsim~L^2n$, and with high probability, $\lambda+\|x_{-k}\|^2 \gtrsim (\lambda+\EE \|x_{-k}\|^2)/L$. The latter condition is also satisfied when the effective rank $r_k$ is high, if the components of $x_{-k}$ are independent.
\end{remark}
Assuming CondNum,  \citet{DBLP:journals/jmlr/TsiglerB23} obtain sharp upper bounds for both the variance and bias of the ridge estimator, with matching lower bounds (see their Theorem~2).
\begin{theorem}[\citet{DBLP:journals/jmlr/TsiglerB23}]
\label{theo:main_barlett}
There exists a constant $c$ that only depends on $\sigma,L$, such that for any $n>ck$, if the assumption condNum$(k,\delta,L)$~(Assumption~\ref{assum_maintext:condNum}) is satisfied, then it holds that $n<cr_k$, and with probability at least $1-\delta-ce^{-n/c}$,
\begin{align*}
        \frac{V}{cv^2} &\leq \frac{k}{n}+\frac{n}{R_k}.\\
        \frac{B}{c} &\leq \left\|\beta^\star_{k}\right\|_{\Sigma_{S,k}^{-1}}^2   \Big(\frac{\lambda+\sum_{j>k}\lambda_j}{n}\Big)^2 + \left\|\beta^\star_{-k}\right\|_{\Sigma_{S,-k}}^2.
\end{align*}
\end{theorem}

\subsection{Out-of-Distribution benign overfitting}
We now derive upper bounds for both the variance and bias of the ridge estimator under covariate shift, assuming an essentially low-rank covariance in the source distribution. Our bound applies to general target distributions, but we also show that ridge regression can match the same non-asymptotic excess risk rate of the in-distribution setting, even under covariate shift, as long as the target distribution retains the same low-rank covariance structure as the source distribution--i.e., the tail components remain in the tail after the distribution shift. Our upper bound is sharp, reducing to \citet{DBLP:journals/jmlr/TsiglerB23}'s bound~(Theorem~\ref{theo:main_barlett}) when the target and source distributions are aligned. Additionally, we recover \cite{DBLP:conf/iclr/GeTFM024}'s sharp bound for under-parameterized linear regression under covariate shift when the high-dimensional components vanish.
\begin{theorem}
\label{theo_maintext:ridge_main}
Let $\calT = \Sigma_{S,k}^{-\frac{1}{2}} \Sigma_{T,k}  \Sigma_{S,k}^{-\frac{1}{2}}$, $\calU = \Sigma_{S,-k}\Sigma_{T,-k}$ and $\calV =  \Sigma_{S,-k}^2$. There exists a constant $c>2$ depending only on $\sigma,L$, such that for any $cN<n<r_k$, if the assumption condNum$(k,\delta,L)$~(Assumption~\ref{assum_maintext:condNum}) is satisfied, then with probability at least $1-3\delta$,
\begin{align*}
    \frac{V}{cv^2} &\leq \frac{k}{n}\frac{\tr[\calT]}{k} + \frac{n}{R_k} \frac{\tr[\calU] }{\tr[\calV]}.\\
    \frac{B}{c} &\leq \Big(\left\|\beta^\star_{k}\right\|_{\Sigma_{S,k}^{-1}}^2   \Big(\frac{\lambda+\sum_{j>k}\lambda_j}{n}\Big)^2 + \left\|\beta^\star_{-k}\right\|_{\Sigma_{S,-k}}^2 \Big) \Big[\|\calT\| + \frac{n}{r_k}\frac{\|\Sigma_{T,-k}\|}{\|\Sigma_{S,-k}\|}\Big].
\end{align*}
$N$ is a polynomial function of $k+\ln (1/\delta)$, $\lambda_1\lambda_k^{-1}$, $1+\big(\lambda+\sum_{j>k}\lambda_j\big)\lambda_k^{-1}$.
\end{theorem}
% explain each item with intuition. 1. variance of underparameterized linear estimator under covaraite shift. cite mle. reduce to classical k/n without shift.
% 2. variance from the noise of high dimensional components, dampened by ridge and implicit regularization. taking \lamda_j,s = \lamda_j,t, var <= n/(d-k). 
% 3. bias for estimating first k components because of ridge and implicit regularization. 
% 4. bias for not learning the noisy signals in last d-k dimensions but just interpolating.
% role of last d-k components as implicit regularization.
\begin{remark}[Implicit regularization]
    The expression $\lambda+\sum_{j>k} \lambda_j$ appears as a unified term in the theorem, implying that the last $d-k$ high-dimensional components act as implicit regularization when learning the signal from the first $k$ low-dimensional components. The first variance term for estimating the first $k$ signal dimensions shows a $1/n$ rate, simplifying to the classic $k/n$ variance for $k$-dimensional OLS when $\Sigma_{S,k}=\Sigma_{T,k}$.  The second variance term for the last $d-k$ dimensions reduces to $n/R_k$, up to the constant $L$, when $\Sigma_{S,-k}=\Sigma_{T,-k}$. It reveals that implicit regularization mitigates noise from the high dimensions, since the variance deceases with $R_k$. Regarding the bias, the first term relates to the signal estimation in the first $k$ dimensions and is introduced by both ridge and implicit regularization. The second bias term arises because the signal in the high-dimensional components,  $\left\|\beta^\star_{-k}\right\|_{\Sigma_{S,-k}}^2$, is merely interpolated rather than learned. 
\end{remark}
% sample number threshold. n<rk: effective rank of last d-k dimension is larger than sample number. consistent with Assmpt 1 & covariance structure for over-parameterized setting. 
% n>N. first argument of N says n>>k. T=S, n>k, classical; T concentrates a single component of S, at most n>k^3. consistent with MLE.
% second argument of N says n>>\lamda+\sum \lambda_j. better than a constant bias term for learning the first k dimensions.
\begin{remark}[Sample complexity]
    We have assumed $n\geq c_xN$ in Theorem~\ref{theo_maintext:ridge_main}. The explicit formula for $N$ is deferred to Theorem~\ref{theo:ridge_main} and Remark~\ref{rem:app_sample}. Here we summarize the sample complexity required for the bound to hold. The dependence on $k$ varies between $\Omega(k)$ and $\Omega(k^3)$, depending on the degree of covariate shift. The optimal case, aligning with the sample complexity of classic linear regression, occurs when $\Sigma_{S,k} \approx \Sigma_{T,k}$. The worst case arises when there is significant covariate shift in the first $k$ dimensions, such as when the test data lies predominantly in the subspace of the first dimension. This variation in sample complexity under covariate shift parallels the analysis of \citet{DBLP:conf/iclr/GeTFM024}~(see theire Theorem~4.2) for the under-parameterized setting. Additionally, we require $n\gg \lambda+\sum_{j>k}\lambda_j$, ensuring that the regularization is not too strong to introduce a bias exceeding a constant (as reflected in the first bias term). On the other hand, we assume $n<r_k$ in the theorem, consistent with the over-parameterized regime and Assumption~\ref{assum_maintext:condNum}, where the last $d-k$ components are considered to be essentially high-dimensional.
\end{remark}
\begin{remark}[Dependence on $L$]
    Theorem~\ref{theo_maintext:ridge_main} does not explicitly show how the excess risk depends on the condition number $L$ of $A_k$. However, we demonstrate in Theorem~\ref{theo:ridge_main} that out bounds scale at most as $L^2$. Notably, we maintain the same order of dependence on $L$ in each term of the upper bounds as in the analysis by \citet{DBLP:journals/jmlr/TsiglerB23}~(see their Theorem~5).
\end{remark}
% comparison with mle ridgeless. lambda_-k,s,t = 0. variance trace(T)/n. bias term.
Theorem~\ref{theo_maintext:ridge_main} establishes an upper bound for the excess risk of ridge regression under general covariate shift. In order to examine how the generalization error adapts to distribution shfit, we present the following corollary, where the upper bounds are expressed as a multiplicative form of Theorem~\ref{theo:main_barlett}'s results. This formulation enables a direct analysis of the impact of covariate shift on the bias and variance of ridge estimators, compared to the in-distribution case. 
% \begin{corollary}
% \label{coroly:maintext_resemble_barlett}
%     Under the same notation as in Theorem~\ref{theo_maintext:ridge_main}, there exists a constant $c>2$ depending only on $\sigma, L$, such that for any $cN<n<r_k$, if the assumption condNum$(k,\delta,L)$ is satisfied, then with probability at least $1-2\delta-ce^{-n/c}$,
%     \begin{align*}
%         \frac{V}{cv^2} &\leq \frac{k}{n}\|\calT\|+\frac{n}{R_k} \frac{\|\Sigma_{T,-k}\|_\rF }{\|\Sigma_{S,-k}\|_\rF}.\\
%         \frac{B}{c} &\leq \Big(\left\|\beta^\star_{k}\right\|_{\Sigma_{S,k}^{-1}}^2   \Big(\frac{\lambda+\sum_{j>k}\lambda_j}{n}\Big)^2 + \left\|\beta^\star_{-k}\right\|_{\Sigma_{S,-k}}^2 \Big) \Big[\|\calT\| + \frac{n}{r_k}\frac{\|\Sigma_{T,-k}\|}{\|\Sigma_{S,-k}\|}\Big].
%     \end{align*}
% \end{corollary}
% comparison with barlett when s=t. variance is the same. refer to a corollary for bias. same rate as barlett when \|\calT\|, \|\Sigma_{t,-k}\| / \lambda_{k+1} are controlled by constant. i.e. tails are in the tails. 
% 1/n rate for k=O(1) r_k=\omega(n^2) \beta norm \Sigma_{k} = O(1) \beta norm \Sigma_{-k} = O(1/n).
% dependence on L is the same.
The first conclusion is that the corollary well reduces to the corresponding result in Theorem~\ref{theo:main_barlett} when no distribution shift occurs--i.e., $\Sigma_S=\Sigma_T$. This connection follows directly from the condition  $n<r_k$. The second conclusion is that covariate shift in the first $k$ dimensions and last $d-k$ dimensions introduce multiplicative factors of $\|\calT\|$ and $\frac{\|\Sigma_{T,-k}\|_\rF }{\|\Sigma_{S,-k}\|_\rF}$, $nr_k^{-1}\frac{ \|\Sigma_{T,-k}\|}{\|\Sigma_{S,-k}\|}$, respectively, on the excess risk. Therefore, as long as these factors are bounded by constants, over-parameterized ridge regression achieves the same non-asymptotic rate of excess risk under covariate shift as the in-distribution setting. This scenario, well addressed by ridge regression, occurs when the target distribution’s covariance structure remains dominated by the first $k$ dimensions. 

In the following, we analyze the impact of the factors introduced by covariate shift on both the low-dimensional and high-dimensional components.

\begin{enumerate}[leftmargin=*]
\item \textbf{Low-dimensional factor.} 
The matrix $\calT$ plays a central role in Theorem~\ref{theo_maintext:ridge_main} to quantify covariate shift within the first $k$ dimensions. This echoes with \citet{DBLP:conf/iclr/GeTFM024}'s finding that $\tr[\calT]$ captures the difficulty of covariate shift for under-parameterized ridgeless regression (MLE). They establish a sharp upper bound on excess risk using Fisher information (see their Theorem~3.1), which simplifies to a rate of $\Tilde{\mathcal{O}}(\tr[\calT]/n)$ for linear models. Theorem~\ref{theo_maintext:ridge_main} recovers this result when applied to a $k$-dimensional under-parameterized setting where all high-dimensional components vanish,  specifically when $\Sigma_{S,-k}=\Sigma_{T,-k}=\zeros$. Under the same condition as Theorem~\ref{theo_maintext:ridge_main}, for a constant $c$ depending only on $\sigma,L$, with high probability the variance and bias terms are bounded by:
\begin{align*}
    \frac{V}{cv^2} \leq \frac{\tr[\calT]}{n}, \quad \frac{B}{c} \leq \left\|\beta^\star_{k}\right\|_{\Sigma_{S,k}^{-1}}^2 \Big(\frac{\lambda}{n}\Big)^2 \|\calT\|.
\end{align*}
The variance bound aligns with \citet{DBLP:conf/iclr/GeTFM024}'s result while the bias vanishes as $\lambda \to 0$. 
\item \textbf{High-dimensional factors.} 
Under covariate shift within the last $d-k$ dimensions, we achieve the same non-asymptotic error rate as in Theorem~\ref{theo:main_barlett}, only if both $\frac{\|\Sigma_{T,-k}\|_\rF }{\|\Sigma_{S,-k}\|_\rF}$ and $nr_k^{-1}\frac{ \|\Sigma_{T,-k}\|}{\|\Sigma_{S,-k}\|}$ are bounded by constants. In other words, the last $d-k$ components of target covariates must scale similarly to or smaller than those of the source, in terms of the covariance norms. Importantly, this condition does not impose constraints on the internal spectral structure of the last $d-k$ components of target covariance. For example, we do not force each eigenvalue of $\Sigma_{T,-k}$ to scale with its corresponding eigenvalue of $\Sigma_{S,-k}$ in decreasing order, as assumed in prior work~\citep{mallinar2024minimum}. This reflects the intuition that the high-dimensional components of covariates function primarily as implicit regularization, implying that only their overall magnitude is relevant.

Another observation is that the bias scales with $nr_k^{-1}\frac{ \|\Sigma_{T,-k}\|}{\|\Sigma_{S,-k}\|}$, meaning that we only require $\frac{ \|\Sigma_{T,-k}\|}{\|\Sigma_{S,-k}\|} = \mathcal O(r_k/n)$, which is a less restrictive condition for larger $r_k$. Thus, over-parameterization improves robustness of the estimation bias against covariate shift in the high-dimensional components.
\end{enumerate}

 Finally, Corollary~\ref{coroly:maintext_resemble_barlett} suggests an $\mathcal O(1/n)$ error rate under several conditions that naturally follow from the previous discussions, which we now state rigorously. First, the covariate space decomposes into an essentially low-dimensional subspace and an essentially high-dimensional subspace, with $k=\mathcal O(1)$ and $R_k=\Omega(n^2)$. Second, the low-rank covariance structure is preserved after covariate shift, such that $\|\calT\|,\frac{\|\Sigma_{T,-k}\|_\rF }{\|\Sigma_{S,-k}\|_\rF},nr_k^{-1}\frac{ \|\Sigma_{T,-k}\|}{\|\Sigma_{S,-k}\|}=\mathcal O(1)$. Third, the signal lies predominantly in the low-dimensional subspace, with $\left\|\beta^\star_{k}\right\|_{\Sigma_{S,k}^{-1}} =\mathcal O(1)$ and $\left\|\beta^\star_{-k}\right\|_{\Sigma_{S,-k}}=\mathcal O(1/\sqrt{n})$. Lastly, the regularization is not excessively strong to introduce a significant bias, with $\lambda+\sum_{j>k}\lambda_j = \mathcal O(\sqrt {n})$. 

% proof


==> ridge_deprecated_V2.tex <==
\section{Over-parameterized ridge regression}
% add discussion: 1. overparameterization improve robustness to shift (bias)
% 2. from minimum-norm interpolant to ridge regression
% 3. Barlett theorem
% why ridge regression: successful for overparameterization without shift. investigate under covariate shift.
% summarize what we do: a bound for overparameterized ridge under covariate shift 1) where the rank structure is preserved: tail components shall still be tail (not essentially high dimension). 2) well reduce to barlett and covariate shift.
When the covariance matrix is essentially low-rank, \cite{DBLP:journals/jmlr/TsiglerB23} demonstrates that the minimum-norm interpolant can effectively learn the signal from the subspace of data spanned by the major eigenvectors, while benignly overfitting noise from the minor directions. Their results extend to ridge regression, showing that the minor components of the covariance matrix inherently provide implicit regularization similar to ridge. In this section, we explore whether the mechanism holds under covariate shift and derive upper bounds for the excess risk of the ridge estimator. We specifically consider cases where the source covariance matrix has a low-rank structure, which the target covariance may or may not share. Our analysis applies to the over-paramerized regime where $k<n<r_k$.
\subsection{Warm-up: in-distribution benign overfitting}
% introduce assumption, cite barlett.  
As a warm-up case, we introduce \citet{DBLP:journals/jmlr/TsiglerB23}'s in-distribution result on benign overfitting in ridge regression. They assume that the data lies within a space spanned by $k$ major directions and $d-k$ minor directions, where the minor components are weak but high-dimensional. In other words, the covariance matrix of the source distribution has a high effective rank relative to the sample size, once the $k$ major components are removed. This intuition is formalized through an assumption that controls the condition number of the Gram matrix for the remaining $d-k$ dimensions.
\begin{myassumption}[CondNum$(k,\delta,L)$, \citep{DBLP:journals/jmlr/TsiglerB23}]
\label{assum_maintext:condNum}
    Define a matrix $A_k = \lambda I_n + X_{-k}X_{-k}^T$. With probability at least $1-\delta$, $A_k$ is positive definite and has a condition number no greater than $L$, i.e.,
    \begin{align*}
        \frac{\mu_1(A_k)}{\mu_n(A_k)} \leq L.
    \end{align*}
\end{myassumption}
% implies essentially high dimension. sufficient and necessary condition.
\begin{remark}
The assumption holds if the effective rank for the last $d-k$ dimensions is significantly larger than $n$. As evidence, \citet{DBLP:journals/jmlr/TsiglerB23}~(Lemma 3) provides a sufficient and almost necessary condition for the condition number of $A_k$ to be smaller than $L$: $r_k~\gtrsim~L^2n$, and with high probability, $\lambda+\|x_{-k}\|^2 \gtrsim (\lambda+\EE \|x_{-k}\|^2)/L$. The latter condition is also satisfied when the effective rank $r_k$ is high, if the components of $x_{-k}$ are independent.
\end{remark}
Assuming CondNum,  \citet{DBLP:journals/jmlr/TsiglerB23} obtain sharp upper bounds for both the variance and bias of the ridge estimator, with matching lower bounds (see their Theorem~2).
\begin{theorem}[\citet{DBLP:journals/jmlr/TsiglerB23}]
\label{theo:main_barlett}
There exists a constant $c$ that only depends on $\sigma,L$, such that for any $n>ck$, if the assumption condNum$(k,\delta,L)$~(Assumption~\ref{assum_maintext:condNum}) is satisfied, then it holds that $n<cr_k$, and with probability at least $1-\delta-ce^{-n/c}$,
\begin{align*}
        \frac{V}{cv^2} &\leq \frac{k}{n}+\frac{n}{R_k}.\\
        \frac{B}{c} &\leq \left\|\beta^\star_{k}\right\|_{\Sigma_{S,k}^{-1}}^2   \Big(\frac{\lambda+\sum_{j>k}\lambda_j}{n}\Big)^2 + \left\|\beta^\star_{-k}\right\|_{\Sigma_{S,-k}}^2.
\end{align*}
\end{theorem}
% explain each item with intuition. 1. variance of underparameterized linear estimator under covaraite shift. cite mle. reduce to classical k/n without shift.
% 2. variance from the noise of high dimensional components, dampened by ridge and implicit regularization. taking \lamda_j,s = \lamda_j,t, var <= n/(d-k). 
% 3. bias for estimating first k components because of ridge and implicit regularization. 
% 4. bias for not learning the noisy signals in last d-k dimensions but just interpolating.
% role of last d-k components as implicit regularization.
The theorem demonstrates that benign overfitting happens due to the implicit regularization of the minor components of the sample covariance. The second term in the variance bound, $n/R_k$, vanishes when the minor directions are sufficiently high-dimensional, i.e., when $R_k \gg n$. In this scenario, noise interpolation leads to an estimator $\hbeta$ that lies in the subspace spanned by $n$ samples, while a new test data point from the $d$-dimensional space is orthogonal to the $n$-dimensional sample space with high probability. As a result, noise does not propagate into the prediction. However, the signal in the minor directions, $\left\|\beta^\star_{-k}\right\|_{\Sigma_{S,-k}}^2$, is nearly lost when projected from the high-dimensional ambient space onto the low-dimensional sample space, contributing to the second bias term. The first variance term arises from estimating the $k$ major signal dimensions, corresponding to the classic variance for $k$-dimensional OLS. Finally, the first bias term relates to the signal estimation in the first $k$ dimensions and is introduced by both ridge and implicit regularization.

\subsection{Out-of-Distribution benign overfitting}
We now investigate benign overfitting when the ridge estimator is evaluated out-of-distribution. We derive upper bounds for both the variance and bias of ridge regression under covariate shift, assuming an essentially low-rank covariance in the source distribution, similar to the in-distribution case. However, our bound applies to general target distributions. Moreover, we show that ridge regression can achieve the same non-asymptotic excess risk rate of the in-distribution setting~(Theorem~\ref{theo:main_barlett}), even under covariate shift, as long as the target distribution retains the same low-rank covariance structure as the source distribution--i.e., the minor components remain in the tail after the distribution shift. Our upper bound is sharp, reducing to \citet{DBLP:journals/jmlr/TsiglerB23}'s bound~(Theorem~\ref{theo:main_barlett}) when the target and source distributions are aligned. Additionally, we recover \cite{DBLP:conf/iclr/GeTFM024}'s sharp bound for under-parameterized linear regression under covariate shift when the high-dimensional minor components vanish.
\begin{theorem}
\label{theo_maintext:ridge_main}
Let $\calT = \Sigma_{S,k}^{-\frac{1}{2}} \Sigma_{T,k}  \Sigma_{S,k}^{-\frac{1}{2}}$, $\calU = \Sigma_{S,-k}\Sigma_{T,-k}$ and $\calV =  \Sigma_{S,-k}^2$. There exists a constant $c>2$ depending only on $\sigma,L$, such that for any $cN<n<r_k$, if the assumption condNum$(k,\delta,L)$~(Assumption~\ref{assum_maintext:condNum}) is satisfied, then with probability at least $1-3\delta$,
\begin{align*}
    \frac{V}{cv^2} &\leq \frac{k}{n}\frac{\tr[\calT]}{k} + \frac{n}{R_k} \frac{\tr[\calU] }{\tr[\calV]}.\\
    \frac{B}{c} &\leq \Big(\left\|\beta^\star_{k}\right\|_{\Sigma_{S,k}^{-1}}^2   \Big(\frac{\lambda+\sum_{j>k}\lambda_j}{n}\Big)^2 + \left\|\beta^\star_{-k}\right\|_{\Sigma_{S,-k}}^2 \Big) \Big[\|\calT\| + \frac{n}{r_k}\frac{\|\Sigma_{T,-k}\|}{\|\Sigma_{S,-k}\|}\Big].
\end{align*}
$N$ is a polynomial function of $k+\ln (1/\delta)$, $\lambda_1\lambda_k^{-1}$, $1+\big(\lambda+\sum_{j>k}\lambda_j\big)\lambda_k^{-1}$.
\end{theorem}
% comparison with mle ridgeless. lambda_-k,s,t = 0. variance trace(T)/n. bias term.
Theorem~\ref{theo_maintext:ridge_main} establishes an upper bound for the excess risk of ridge regression under general covariate shift, expressed as a multiplicative form of Theorem~\ref{theo:main_barlett}'s results. This formulation enables a direct analysis of the impact of covariate shift on the bias and variance of ridge estimators, compared to the in-distribution case. 
% \begin{corollary}
% \label{coroly:maintext_resemble_barlett}
%     Under the same notation as in Theorem~\ref{theo_maintext:ridge_main}, there exists a constant $c>2$ depending only on $\sigma, L$, such that for any $cN<n<r_k$, if the assumption condNum$(k,\delta,L)$ is satisfied, then with probability at least $1-2\delta-ce^{-n/c}$,
%     \begin{align*}
%         \frac{V}{cv^2} &\leq \frac{k}{n}\|\calT\|+\frac{n}{R_k} \frac{\|\Sigma_{T,-k}\|_\rF }{\|\Sigma_{S,-k}\|_\rF}.\\
%         \frac{B}{c} &\leq \Big(\left\|\beta^\star_{k}\right\|_{\Sigma_{S,k}^{-1}}^2   \Big(\frac{\lambda+\sum_{j>k}\lambda_j}{n}\Big)^2 + \left\|\beta^\star_{-k}\right\|_{\Sigma_{S,-k}}^2 \Big) \Big[\|\calT\| + \frac{n}{r_k}\frac{\|\Sigma_{T,-k}\|}{\|\Sigma_{S,-k}\|}\Big].
%     \end{align*}
% \end{corollary}
% comparison with barlett when s=t. variance is the same. refer to a corollary for bias. same rate as barlett when \|\calT\|, \|\Sigma_{t,-k}\| / \lambda_{k+1} are controlled by constant. i.e. tails are in the tails. 
% 1/n rate for k=O(1) r_k=\omega(n^2) \beta norm \Sigma_{k} = O(1) \beta norm \Sigma_{-k} = O(1/n).
% dependence on L is the same.
The first conclusion is that the corollary well reduces to the corresponding result in Theorem~\ref{theo:main_barlett} when no distribution shift occurs--i.e., $\Sigma_S=\Sigma_T$. This connection follows directly from the condition  $n<r_k$. 

The second conclusion is that covariate shift in the first $k$ dimensions and last $d-k$ dimensions introduce multiplicative factors of $\frac{\tr[\calT]}{k}$, $\|\calT\|$ and $\frac{\tr[\calU] }{\tr[\calV]}$, $nr_k^{-1}\frac{ \|\Sigma_{T,-k}\|}{\|\Sigma_{S,-k}\|}$, respectively, on the excess risk. Therefore, as long as these factors are bounded by constants, over-parameterized ridge regression achieves the same non-asymptotic rate of excess risk under covariate shift as the in-distribution setting. This scenario, well addressed by ridge regression, occurs when the target distribution’s covariance structure remains dominated by the first $k$ dimensions. 
In the following, we analyze the impact of the factors introduced by covariate shift on both the major and minor directions.

\begin{enumerate}[leftmargin=*]
\item \textbf{Factors on major directions.} 
Under covariate shift within the first $k$ dimensions, we obtain the same non-asymptotic error rate as in Theorem~\ref{theo:main_barlett}, only if $\|\calT\|$ is bounded by a constant, as $\tr[\calT]/k \leq\|\calT\|$.
The matrix $\calT$ plays a central role in Theorem~\ref{theo_maintext:ridge_main} to quantify covariate shift within the first $k$ dimensions. This echoes with \citet{DBLP:conf/iclr/GeTFM024}'s finding that $\tr[\calT]$ captures the difficulty of covariate shift for under-parameterized ridgeless regression (MLE). They establish a sharp upper bound on excess risk using Fisher information (see their Theorem~3.1), which simplifies to a rate of $\Tilde{\mathcal{O}}(\tr[\calT]/n)$ for linear models. Theorem~\ref{theo_maintext:ridge_main} recovers this result when applied to a $k$-dimensional under-parameterized setting where all high-dimensional minor components vanish,  specifically when $\Sigma_{S,-k}=\Sigma_{T,-k}=\zeros$. Under the same condition as Theorem~\ref{theo_maintext:ridge_main}, for a constant $c$ depending only on $\sigma,L$, with high probability the variance and bias terms are bounded by:
\begin{align*}
    \frac{V}{cv^2} \leq \frac{\tr[\calT]}{n}, \quad \frac{B}{c} \leq \left\|\beta^\star_{k}\right\|_{\Sigma_{S,k}^{-1}}^2 \Big(\frac{\lambda}{n}\Big)^2 \|\calT\|.
\end{align*}
The variance bound aligns with \citet{DBLP:conf/iclr/GeTFM024}'s result while the bias vanishes as $\lambda \to 0$. 
\item \textbf{Factors on minor directions.} 
Under covariate shift within the last $d-k$ dimensions, we achieve the same non-asymptotic error rate as in Theorem~\ref{theo:main_barlett}, only if both $\frac{\tr[\calU] }{\tr[\calV]}$ and $nr_k^{-1}\frac{ \|\Sigma_{T,-k}\|}{\|\Sigma_{S,-k}\|}$ are bounded by constants. Note that $\frac{\tr[\calU] }{\tr[\calV]}\leq \frac{\|\Sigma_{T,-k}\|_\rF}{\|\Sigma_{S,-k}\|_\rF}$. In other words, the last $d-k$ components of target covariates must scale similarly to or smaller than those of the source, in terms of the covariance norms. Importantly, this condition does not impose constraints on the internal spectral structure of the last $d-k$ components of target covariance. For example, we do not force each eigenvalue of $\Sigma_{T,-k}$ to scale with its corresponding eigenvalue of $\Sigma_{S,-k}$ in decreasing order, as assumed in prior work~\citep{mallinar2024minimum}. This reflects the intuition that the minor components of covariates function primarily as implicit regularization, implying that only their overall magnitude is relevant.

Another observation is that the bias scales with $nr_k^{-1}\frac{ \|\Sigma_{T,-k}\|}{\|\Sigma_{S,-k}\|}$, meaning that we only require $\frac{ \|\Sigma_{T,-k}\|}{\|\Sigma_{S,-k}\|} = \mathcal O(r_k/n)$, which is a less restrictive condition for larger $r_k$. Thus, over-parameterization improves robustness of the estimation bias against covariate shift in the minor direction.
\end{enumerate}
% sample number threshold. n<rk: effective rank of last d-k dimension is larger than sample number. consistent with Assmpt 1 & covariance structure for over-parameterized setting. 
% n>N. first argument of N says n>>k. T=S, n>k, classical; T concentrates a single component of S, at most n>k^3. consistent with MLE.
% second argument of N says n>>\lamda+\sum \lambda_j. better than a constant bias term for learning the first k dimensions.
\begin{remark}[Sample complexity]
    We have assumed $n\geq c_xN$ in Theorem~\ref{theo_maintext:ridge_main}. The explicit formula for $N$ is deferred to Theorem~\ref{theo:ridge_main} and Remark~\ref{rem:app_sample}. Here we summarize the sample complexity required for the bound to hold. The dependence on $k$ varies between $\Omega(k)$ and $\Omega(k^3)$, depending on the degree of covariate shift. The optimal case, aligning with the sample complexity of classic linear regression, occurs when $\Sigma_{S,k} \approx \Sigma_{T,k}$. The worst case arises when there is significant covariate shift in the first $k$ dimensions, such as when the test data lies predominantly in the subspace of the first dimension. This variation in sample complexity under covariate shift parallels the analysis of \citet{DBLP:conf/iclr/GeTFM024}~(see theire Theorem~4.2) for the under-parameterized setting. Additionally, we require $n\gg \lambda+\sum_{j>k}\lambda_j$, ensuring that the regularization is not too strong to introduce a bias exceeding a constant (as reflected in the first bias term). On the other hand, we assume $n<r_k$ in the theorem, consistent with the over-parameterized regime and Assumption~\ref{assum_maintext:condNum}, where the last $d-k$ components are considered to be essentially high-dimensional.
\end{remark}
\begin{remark}[Dependence on $L$]
    Theorem~\ref{theo_maintext:ridge_main} does not explicitly show how the excess risk depends on the condition number $L$ of $A_k$. However, we demonstrate in Theorem~\ref{theo:ridge_main} that out bounds scale at most as $L^2$. Notably, we maintain the same order of dependence on $L$ in each term of the upper bounds as in the analysis by \citet{DBLP:journals/jmlr/TsiglerB23}~(see their Theorem~5).
\end{remark}
 Finally, Theorem~\ref{theo_maintext:ridge_main} suggests an $\mathcal O(1/n)$ vanishing error under several conditions that naturally follow from the previous discussions, which we now state rigorously. First, the covariate space decomposes into subspaces spanned by low-dimensional major directions and high-dimensional minor directions, with $k=\mathcal O(1)$ and $R_k=\Omega(n^2)$. Second, the low-rank covariance structure is preserved after covariate shift, such that$\|\calT\|, \frac{\tr[\calU] }{\tr[\calV]}, nr_k^{-1}\frac{ \|\Sigma_{T,-k}\|}{\|\Sigma_{S,-k}\|}=\mathcal O(1)$. Third, the signal lies predominantly in the major directions, with $\left\|\beta^\star_{k}\right\|_{\Sigma_{S,k}^{-1}} =\mathcal O(1)$ and $\left\|\beta^\star_{-k}\right\|_{\Sigma_{S,-k}}=\mathcal O(1/\sqrt{n})$. Lastly, the regularization is not excessively strong to introduce a significant bias, with $\lambda+\sum_{j>k}\lambda_j = \mathcal O(\sqrt {n})$. 

% proof


==> ridge_proof_deprecated_v1.tex <==
\section{Ridge Regression}
Let $X = (x_1, ..., x_n)^T \in \mathbb R^{n\times d}$, $Y = (y_1,...,y_n)^T \in \RR^d$ and $\boldsymbol{\epsilon}=(\epsilon_1,...,\epsilon_n)^T\in\RR^d$. We denote the first $k$ columns of $X$ as $X_{0:k}$ and the remaining $d-k$ columns as $X_{k:d}$. Similarly, $\beta^\star_{0:k}$ and $\beta^\star_{k:d}$ represent the corresponding components of $\beta^\star$. $\Sigma_{S,0:k}$, $\Sigma_{S,k:d}$ are the corresponding blocks on the diagonal of $\Sigma_S$. The $i$-th eigenvalue of a matrix is denoted by $\mu_i(\cdot)$. Define $Z = X\Sigma_S^{-1/2}$, where the rows of $Z$ are i.i.d. centered isotropic random vectors. Additionally, we assume the rows of $Z$ are $\sigma_x$-sub-gaussian, where the sub-gaussian norm is defined as follows. 

For a random variable $s$, the sub-gaussian norm $\|s\|_{\psi_2}$ is given by:
\begin{align*}
    \|s\|_{\psi_2} = \inf\left\{t>0: \EE\left[\exp \frac{s^2}{t^2} \right] \leq 2 \right\}.
\end{align*}

For a random vector $S$, the sub-gaussian norm $\|S\|_{\psi_2}$ is given by:
\begin{align*}
    \|S\|_{\psi_2} = \sup_{v\neq 0} \frac{\| \langle S, v \rangle \|_{\psi_2}}{\|v\|}.
\end{align*}

For $\lambda>0$, consider the ridge estimator:
\begin{align*}
    \hbeta(Y) &= X^T(XX^T+\lambda I_n)^{-1}Y \\
    &= X^T(XX^T+\lambda I_n)^{-1}X\beta^\star + X^T(XX^T+\lambda I_n)^{-1}\boldsymbol{\epsilon} \\
    &= \hbeta(X\beta^\star) + \hbeta(\boldsymbol{\epsilon}),
\end{align*}
where we define $\hbeta(X\beta^\star)=X^T(XX^T+\lambda I_n)^{-1}X\beta^\star$ and $\hbeta(\boldsymbol{\epsilon})=X^T(XX^T+\lambda I_n)^{-1}\boldsymbol{\epsilon}$. Additionally, we define $\tilde{\Sigma}_S = \Sigma_S + \frac{\lambda}{n}I_d$.
\begin{myassumption}[CondNum$(k,\delta,L)$]
\label{assum:condNum}
    With probability at least $1-\delta$, the matrix $X_{k:d}X_{k:d}^T$ is positive definite and has a condition number no greater than $L$, i.e.,
    \begin{align*}
        \frac{\mu_1(X_{k:d}X_{k:d}^T)}{\mu_n(X_{k:d}X_{k:d}^T)} \leq L.
    \end{align*}
\end{myassumption}

\subsection{Concentration Inequalities}
Denote the element of a matrix $X$ in the $i$-th row and the $j$-th column as $X[i,j]$, and the $i$-th row of the matrix $X$ as $X[i,*]$.

\begin{lemma}[Lemma~20 of \cite{DBLP:journals/jmlr/TsiglerB23}]
\label{lem:sigmaz}
Let $z$ be a sub-gaussian vector in $\mathbb{R}^p$ with $\|z\|_{\psi_2} \leq \sigma_x$, and consider $\Sigma = \operatorname{diag}(\lambda_1, \dots, \lambda_p)$ where the sequence $\{\lambda_j\}_{j=1}^p$ is positive and non-increasing. Then there exists some absolute constant $c$, for any $t > 0$, with probability at least $1-2e^{-t/c}$:
\begin{align*}
    \|\Sigma^{1/2} z\|^2 \leq c \sigma_x^2 \left( t \lambda_1 + \sum_{j=1}^p \lambda_j \right).
\end{align*}
\end{lemma}

\begin{lemma}[Lemma~23 of \cite{DBLP:journals/jmlr/TsiglerB23}]
\label{lem:ringAk}
Let \( \mathring{A}_k \) represent the matrix $X_{k:d}X_{k:d}^T$ with its diagonal elements set to zero: 
\begin{align*}
    \mathring{A}_k[i,j] = (1 - \delta_{i,j})(X_{k:d}X_{k:d}^T)[i,j].
\end{align*}
Then there exists some absolute constant \( c \), for any \( t > 0 \), with probability at least \( 1 - 4e^{-t/c} \):
\[
\|\mathring{A}_k\| \leq c\sigma_x^2 \sqrt{(t+n) \left( \lambda_{k+1}^2 (t+n) + \sum_{j > k} \lambda_j^2 \right)}.
\]
\end{lemma} 

\begin{lemma}[Lemma~21 of \cite{DBLP:journals/jmlr/TsiglerB23}] 
\label{lem:sum_sigmaz}
Suppose $\{z_i\}_{i=1}^n$ is a sequence of independent isotropic sub-gaussian random vectors, where \(\| z_i \|_{\psi_2} \leq \sigma\). Let \(\Sigma = \text{diag}(\lambda_1, \dots, \lambda_p)\) represent a diagonal matrix with a positive, non-increasing sequence \(\{ \lambda_i \}_{i=1}^p\). Then there exists some absolute constant \(c\), for any \(t \in (0, n)\), with probability at least \(1 - 2 e^{-ct}\):
\[
(n - \sqrt{nt} \sigma^2) \sum_{j=1}^p \lambda_j \leq \sum_{i=1}^n \|\Sigma^{1/2} z_i\|^2 
\leq (n + \sqrt{nt} \sigma^2) \sum_{j=1}^p \lambda_j.
\]
\end{lemma}

\begin{lemma}
\label{lem:xxT_concentration}
    Under the assumption CondNum$(k,\delta,L)$ (Assumption~\ref{assum:condNum}), there exists a constant $c_x$, depending only on $\sigma_x$, such that 
    for any $n<\frac{1}{\lambda_{k+1}} 
    \sum_{j>k}\lambda_j$, % without this assumption, the upper bound will be n \lambda_{k+1} + \sum \lambda_j.
    with probability at least $1-\delta-c_xe^{-n/c_x}$:
    \begin{align*}
        \frac{1}{c_xL} \sum_{j>k} \lambda_j \leq \mu_n(X_{k:d}X_{k:d}^T) \leq \mu_1(X_{k:d}X_{k:d}^T) \leq c_x \sum_{j>k} \lambda_j.
    \end{align*}
\end{lemma}
\begin{proof}
This result follows from the proof of Lemma~3 in \cite{DBLP:journals/jmlr/TsiglerB23}, which establishes both upper and lower bounds of $\mu_1(X_{k:d}X_{k:d}^T)$. By combining the lower bound with the assumption CondNum, we derive a lower bound of $\mu_n(X_{k:d}X_{k:d}^T)$. For completeness, we restate the entire proof here.

According to lemma~\ref{lem:sigmaz} and lemma~\ref{lem:ringAk}, there exists an absolute constant c, such that for any $t>0$:
\begin{enumerate}
    \item for all $1\leq i \leq n$, with probability at least $1-2e^{-t/c}$:
    \begin{align*}
        \| X_{k:d}[i,*]\|^2 \leq c \sigma_x^2 \left( t \lambda_{k+1} + \sum_{j>k} \lambda_j \right).
    \end{align*}
    \item with probability at least $1-4e^{-t/c}$:
    \begin{align*}
        \|\mathring{A}_k\| \leq c\sigma_x^2 \sqrt{(t+n) \left( \lambda_{k+1}^2 (t+n) + \sum_{j > k} \lambda_j^2 \right)}.
    \end{align*}
\end{enumerate}
Since $\mu_1(X_{k:d}X_{k:d}^T) \leq \|\mathring{A}_k\| + \max_i \| X_{k:d}[i,*] \|^2$,
by setting $t=n$, we have with probability at least $1-(2n+4)e^{-n/c}$:
\begin{align}
\begin{split}
\label{eq:lem_xxT_concentration_1}
    \mu_1(X_{k:d}X_{k:d}^T) &\leq c\sigma_x^2 \left( n\lambda_{k+1} + \sum_{j > k} \lambda_j + \sqrt{(2n \lambda_{k+1})^2 + 2n\sum_{j > k} \lambda_j^2 } 
     \right) \\
     &\leq c\sigma_x^2 \left( n\lambda_{k+1} + \sum_{j > k} \lambda_j + 2n \lambda_{k+1} + \sqrt{2n\sum_{j > k} \lambda_j^2} \right) \\
     &\leq c\sigma_x^2 \left( n\lambda_{k+1} + \sum_{j > k} \lambda_j + 2n \lambda_{k+1} + \sqrt{2n\lambda_{k+1}\sum_{j > k} \lambda_j} \right) \\
     &\leq c\sigma_x^2 \left( n\lambda_{k+1} + \sum_{j > k} \lambda_j + 2n \lambda_{k+1} + n\lambda_{k+1} + \frac{1}{2}\sum_{j > k} \lambda_j \right) \\
     &\leq 4c\sigma_x^2 \left( n\lambda_{k+1} + \sum_{j > k} \lambda_j \right) \\
     &\leq 8c\sigma_x^2  \sum_{j > k} \lambda_j.
\end{split}
\end{align}
The last inequality follows from $n<\frac{1}{\lambda_{k+1}} \sum_{j>k}\lambda_j$.

On the other hand, by applying Lemma~\ref{lem:sum_sigmaz} with $t=\frac{n}{4\sigma_x^4}$, there exists an absolute constant $c'$, such that with probability at least $1 - 2 \exp\left\{-\frac{c'}{4\sigma_x^4}n \right\}$:
\begin{align*}
    \sum_{i=1}^n \|X_{k:d}[i,*]\|^2 \geq \frac{1}{2}n \sum_{j>k} \lambda_j.
\end{align*}
On this event,
\begin{align*}
    \mu_1(X_{k:d}X_{k:d}^T) &\geq \frac{1}{n} \operatorname{tr} (X_{k:d}X_{k:d}^T) \\
    &= \frac{1}{n} \sum_{i=1}^n \|X_{k:d}[i,*]\|^2 \\
    &\geq \frac{1}{2} \sum_{j>k} \lambda_j.
\end{align*}
By the assumption CondNum$(k,\delta,L)$, we have with probability at least $1-\delta-2 \exp\left\{-\frac{c'}{4\sigma_x^4}n \right\}$:
\begin{align}
\begin{split}
\label{eq:lem_xxT_concentration_2}
    \mu_n(X_{k:d}X_{k:d}^T) \geq \frac{1}{L} \mu_1(X_{k:d}X_{k:d}^T) \geq \frac{1}{2L} 
    \sum_{j>k} \lambda_j.
\end{split}
\end{align}
Combining Equation~\ref{eq:lem_xxT_concentration_1} and~\ref{eq:lem_xxT_concentration_2}, there exists a constant $c_x$ depending only on $\sigma_x$, such that with probability at least $1-\delta-c_x e^{-n/c_x}$:
\begin{align*}
    \frac{1}{c_xL} \sum_{j>k} \lambda_j \leq \mu_n(X_{k:d}X_{k:d}^T) \leq \mu_1(X_{k:d}X_{k:d}^T) \leq c_x \sum_{j>k} \lambda_j.
\end{align*}
\end{proof}

\begin{lemma}
\label{lem:xTx_concentration}
    There exists a constant $c_x$ depending only on $\sigma_x$, such that with probability at least $1-\delta$, if $n>k + \operatorname{ln}(1/\delta)$,
    \begin{align*}
        \left\| \frac{1}{n}X_{0:k}^TX_{0:k} - \Sigma_{S,0:k} \right\| \leq c_x \lambda_1 \sqrt{\frac{k+\operatorname{ln}\frac{1}{\delta}}{n}}.
    \end{align*}
\end{lemma}
\begin{proof}
    This follows directly from Theorem~5.39 and Remark~5.40 of \cite{DBLP:journals/corr/abs-1011-3027}, which shows there exists a constant $c_x'$ depending only on $\sigma_x$, such that for any $t\geq 0$, with probability at least $1-2\exp\{-t^2/c_x'\}$:
     \begin{align*}
          \left\| \frac{1}{n}X_{0:k}^TX_{0:k} - \Sigma_{S,0:k} \right\| \leq \lambda_1 \max \left\{ c_x'\sqrt{\frac{k}{n}} + \frac{t}{\sqrt n}, \left( c_x'\sqrt{\frac{k}{n}} + \frac{t}{\sqrt n} \right)^2 \right\}.
     \end{align*}
     Taking $t=\sqrt{c_x' \operatorname{ln}(2/\delta)}$ completes the proof.
\end{proof}

\begin{corollary}
\label{coroly:xTxroot_concentration}
    Under the same conditions as in Lemma~\ref{lem:xTx_concentration}, and on the same event, the following holds:
    \begin{align*}
        \left\| \left(X_{0:k}^TX_{0:k}\right)^{\frac{1}{2}} - \sqrt{n}\Sigma_{S,0:k}^{\frac{1}{2}} \right\| 
        \leq c_x \sqrt {k+\ln{\frac{1}{\delta}}}\lambda_1\lambda_k^{-\frac{1}{2}}.
    \end{align*}
\end{corollary}
\begin{proof}
    According to Proposition~3.2 of \cite{van1980inequality}, for any positive semi-definite matrix $A,B\in\RR^k$, we have 
    \begin{align*}
        \|A-B\| \geq \left(\mu_k\left(A^{\frac{1}{2}}\right)+\mu_k\left(B^{\frac{1}{2}}\right) \right)
        \left\|A^{\frac{1}{2}} - B^{\frac{1}{2}}\right\|.
    \end{align*}
    Therefore,
    \begin{align*}
        \left\| \left(X_{0:k}^TX_{0:k}\right)^{\frac{1}{2}} - \sqrt{n}\Sigma_{S,0:k}^{\frac{1}{2}} \right\| 
        &\leq \frac{1}{\mu_k\left(\sqrt{n}\Sigma_{S,0:k}^{\frac{1}{2}}\right)}  \left\| X_{0:k}^TX_{0:k} - n\Sigma_{S,0:k} \right\| \\
        &= \sqrt{n} \lambda_k^{-\frac{1}{2}} \left\| \frac{1}{n}X_{0:k}^TX_{0:k} - \Sigma_{S,0:k} \right\|. 
    \end{align*}
    By applying Lemma~\ref{lem:xTx_concentration}, the proof is complete.
\end{proof}

\begin{lemma}
\label{lem:sxTxs_concentration}
    There exists a constant $c_x$ depending only on $\sigma_x$, such that for any $n>c_xk$, with probability at least $1-2e^{-n/c_x}$:
    \begin{align*}
        \frac{1}{c_x}n \leq \mu_k\pth{\Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}}  \leq \mu_1\pth{\Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}}  \leq c_x n.
    \end{align*}
\end{lemma}
\begin{proof}
    According to Theorem~5.39 of \cite{DBLP:journals/corr/abs-1011-3027}, there exists a constant $c_x'$ depending only on $\sigma_x$, such that for any $t\geq 0$, with probability at least $1-2\exp\{ -t^2/c_x' \}$:
    \begin{align*}
        \mu_k\pth{\Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}}   
        &\geq \left( \sqrt{n} - c_x'\sqrt{k} - t  \right)^2.  \\ 
        \mu_1\pth{\Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}}  &\leq  \left( \sqrt{n} + c_x'\sqrt{k} + t  \right)^2 .
    \end{align*}
    Let $t=\frac{1}{2}\sqrt{n}$. For $n>16(c_x')^2 k$, with probability at least $1-2\exp \left\{ -n /(4c_x') \right\}$:
    \begin{align*}
        \mu_k\pth{\Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}}  
        &\geq \pth{ \sqrt{n} - \frac{1}{4}\sqrt{n} - \frac{1}{2}\sqrt{n}}^2 = \frac{1}{16}n. \\
        \mu_1\pth{\Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}}  
        &\leq \pth{ \sqrt{n} + \frac{1}{4}\sqrt{n} + \frac{1}{2}\sqrt{n}}^2 = \frac{49}{16}n.
    \end{align*}
    By taking $c_x = \max \sth{16(c_x')^2, 4c_x', 16}$, the proof is complete.
\end{proof}
\begin{remark}
On the same event, the following inequalities also hold:
\begin{align*}
    &\mu_1(X_{0:k}^TX_{0:k}) \leq \| \Sigma_{S,0:k} \| \left\| \Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}} \right\| \leq c_x\lambda_1n. \\
    &\mu_k(X_{0:k}^TX_{0:k}) \geq \mu_k(\Sigma_{S,0:k})  \mu_k\pth{\Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}} \geq \frac{1}{c_x}\lambda_kn.
\end{align*}
\end{remark}

\begin{lemma}
\label{lem:xsTxT_concentration}
    There exists a constant $c_x$ depending only on $\sigma_x$, with probability at least $1-2e^{-n/c_x}$:
    \begin{align*}
        \tr\pth{X_{k:d}\Sigma_{T,k:d}X_{k:d}^T} \leq c_x n\tr\pth{\Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d} \Sigma_{S,k:d}^{\frac{1}{2}} }.
    \end{align*}
\end{lemma}
\begin{proof}
According to Hanson-Wright Inequality~\citep{vershynin2018high}, there exists an absolute constant $c$, such that for any $1\leq i\leq n$,
\begin{align*}
    \left\| Z_{k:d}[i,*] \Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d}\Sigma_{S,k:d}^{\frac{1}{2}} Z_{k:d}[i,*]^T  \right\|_{\psi_1} 
    &\leq c \sigma_x^2 \left\| \Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d}\Sigma_{S,k:d}^{\frac{1}{2}} \right\|_F  \\
    &\leq c \sigma_x^2 \tr \pth{\Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d}\Sigma_{S,k:d}^{\frac{1}{2}}}.
\end{align*}
By Bernstein Inequality~(Proposition~5.16 of \cite{DBLP:journals/corr/abs-1011-3027}), there exists an absolute constant $c'$, for any $t\geq 0$,
\begin{align*}
    &\quad \PP \sth{\frac{1}{n} \left| \sum_{i=1}^n \qth {Z_{k:d}[i,*] \Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d}\Sigma_{S,k:d}^{\frac{1}{2}} Z_{k:d}[i,*]^T - \tr \pth{\Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d}\Sigma_{S,k:d}^{\frac{1}{2}}} } \right| 
     \geq t } \\
     &\leq 2 \exp \sth{-c'n \min \sth{ \frac{t^2}{K^2}, \frac{t}{K} }  },
\end{align*}
where $K=\max_i \left\| Z_{k:d}[i,*] \Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d}\Sigma_{S,k:d}^{\frac{1}{2}} Z_{k:d}[i,*]^T \right\|_{\psi_1}$.

Let $t=c\sigma_x^2 \tr \pth{\Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d}\Sigma_{S,k:d}^{\frac{1}{2}}}$. Then, with probability at least $1-2e^{-c'n}$:
\begin{align*}
    \tr\pth{X_{k:d}\Sigma_{T,k:d}X_{k:d}^T} &= \sum_{i=1}^n  Z_{k:d}[i,*] \Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d}\Sigma_{S,k:d}^{\frac{1}{2}} Z_{k:d}[i,*]^T  \\
    &\leq (1+c\sigma_x^2) n \tr \pth{\Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d}\Sigma_{S,k:d}^{\frac{1}{2}}}.
\end{align*}
By taking $c_x = \max\sth{ 1+c\sigma_x^2, \frac{1}{c'} }$, the proof is complete.
\end{proof}

\begin{lemma}
\label{lem:bxTxb_concentration}
    There exists a constant $c_x$ depending only on $\sigma_x$, with probablity at least $1-2e^{-n/c_x}$:
    \begin{align*}
        (\beta^\star_{k:d})^TX_{k:d}^TX_{k:d}\beta^\star_{k:d} \leq c_x n (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d}.
    \end{align*}
\end{lemma}
\begin{proof}
    The result follows from the proof of Lemma~3 in \cite{DBLP:journals/jmlr/TsiglerB23}, which we restate here for completeness. Consider the isotropic vector $ \qth{(\beta^\star_{k:d})^T\Sigma_{S,k:d}\beta^\star_{k:d}}^{-1/2}X_{k:d}\beta^\star_{k:d}$. For the $i$-th component,
    \begin{align*}
        \left\| \qth{(\beta^\star_{k:d})^T\Sigma_{S,k:d}\beta^\star_{k:d}}^{-\frac{1}{2}}X_{k:d}[i,*]\beta^\star_{k:d} \right\|_{\psi_2} 
        &=   \qth{(\beta^\star_{k:d})^T\Sigma_{S,k:d}\beta^\star_{k:d}}^{-\frac{1}{2}} \left\| Z_{k:d}[i,*]\Sigma_{S,k:d}^{\frac{1}{2}} \beta^\star_{k:d}\right\|_{\psi_2} \\
        &\leq \qth{(\beta^\star_{k:d})^T\Sigma_{S,k:d}\beta^\star_{k:d}}^{-\frac{1}{2}}
        \sigma_x \left\| \Sigma_{S,k:d}^{\frac{1}{2}} \beta^\star_{k:d} \right\| \\
        &=\sigma_x.
    \end{align*}
    By applying Lemma~\ref{lem:sum_sigmaz} for the sequence $\sth{\qth{(\beta^\star_{k:d})^T\Sigma_{S,k:d}\beta^\star_{k:d}}^{-1/2}X_{k:d}[i,*]\beta^\star_{k:d}}_{i=1}^n$, there exists an absolute constant $c$, for any $t\in(0,n)$, with probability at least $1-2e^{-ct}$:
    \begin{align*}
        \frac{(\beta^\star_{k:d})^TX_{k:d}^TX_{k:d}\beta^\star_{k:d}} {(\beta^\star_{k:d})^T\Sigma_{S,k:d}\beta^\star_{k:d}} &\leq n+\sqrt{nt}\sigma_x^2.
    \end{align*}
    Let $t=n/4$, with probability at least $1-2e^{-cn/4}$:
    \begin{align*}
        (\beta^\star_{k:d})^TX_{k:d}^TX_{k:d}\beta^\star_{k:d} \leq (1+\frac{1}{2}\sigma_x^2)n \cdot (\beta^\star_{k:d})^T\Sigma_{S,k:d}\beta^\star_{k:d}.
    \end{align*}
    By taking $c_x =\max \sth{ 1+\frac{1}{2}\sigma_x^2, \frac{4}{c} }$, the proof is complete.
\end{proof}

% % \subsection{Block Decomposition of $X_{k:d}X_{k:d}^T$}
\subsection{Block Decomposition of \texorpdfstring{$X_{k:d}X_{k:d}^T$}{X(k:d)X(k:d)T}}

Let $X_{0:k} = U\tilde{M}^{\frac{1}{2}}V$, where $U\in\RR^{n\times n}$ and $V\in\RR^{d\times d}$ are orthogonal matrices representing the left and right singular vectors, respectively. The matrix $\tilde{M}^{\frac{1}{2}}$ is defined as: 
\begin{align*}
    \tilde{M}^{\frac{1}{2}} = 
    \begin{pmatrix}
    m_1^{\frac{1}{2}} &  &  \\
     & \ddots &  \\
     &  & m_k^{\frac{1}{2}} \\
    \multicolumn{3}{c}{\mathbf{0}^{(n-k)\times k}} \\
    \end{pmatrix}
    \in \RR^{n\times k}.
\end{align*}
Therefore, we have $X_{0:k}X_{0:k}^T = UMU^T$, where $M=\operatorname{diag}(m_1,...,m_k,0,...,0) \in\RR^{n\times n}$. Similarly, $X_{0:k}^TX_{0:k}=V^T M_k V$, where $M_k = \operatorname{diag}(m_1,...,m_k) \in \RR^{k\times k}$. 

Let $\Delta = U^TX_{k:d}X_{k:d}^TU$, and write $\Delta$ in block matrix form as:
\begin{align*}
    \Delta = 
    \begin{pmatrix}
        \Delta_{11} & \Delta_{12} \\
        \Delta_{12}^T & \Delta_{22} \\
    \end{pmatrix},
\end{align*}
where $\Delta_{11} \in \RR^{k\times k}$, $\Delta_{12} \in \RR^{k\times (n-k)}$, and $\Delta_{22} \in \RR^{(n-k)\times (n-k)}$.

We will repeatedly use the first $k$ rows of $(M+\lambda I_n+\Delta)^{-1}$, which we compute here. Because $M+\lambda I_n+\Delta$ and $\lambda I_{n-k} + \Delta_{22}$ are invertible for $\lambda>0$, by block matrix inverse,
\begin{align}
\begin{split}
\label{eq:A_kinverse_firstkrows}
    &\quad (M+\lambda I_n+\Delta)^{-1}[0:k, *] \\
    &= \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1}
    \pth{I_k, - \Delta_{12}(\lambda I_{n-k} + \Delta_{22})^{-1} }.
\end{split}
\end{align}

\begin{corollary}[Corollary of Lemma~\ref{lem:xxT_concentration}]
\label{coroly:Delta}
    Suppose the assumption condNum$(k,\delta,L)$ is satisfied. There exists a constant depending only on $\sigma_x$, such that for any $n<\frac{1}{\lambda_{k+1}} 
    \sum_{j>k}\lambda_j$, % without this assumption, the upper bound will be n \lambda_{k+1} + \sum \lambda_j.
    the following inequalities hold with probability at least $1-\delta-c_xe^{-n/c_x}$, on the same event as in Lemma~\ref{lem:xxT_concentration}.
    \begin{align*}
        &\| \Delta_{11} \|,\| \Delta_{12} \| \leq \|\Delta\| \leq c_x \sum_{j>k} \lambda_j. \\
        &\|(\lambda I_{n-k} + \Delta_{22})^{-1}\| \leq \|\Delta^{-1}\| \leq c_xL\pth{\sum_{j>k}\lambda_j}^{-1}. \\
        &\left\| \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-2} \Delta_{12}^T \right\| \leq c_x^4 L^2. \\
        &\left\| \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T \right\| \leq c_x^3 L \sum_{j>k}\lambda_j. \\
        &\left\| \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T \right\| \leq c_x \sum_{j>k} \lambda_j.
    \end{align*}
\end{corollary}
\begin{proof}
\begin{enumerate}
    \item The first inequality.
    \begin{align*}
        \| \Delta_{11} \|,\| \Delta_{12} \| \leq \|\Delta\| = \| X_{k:d}X_{k:d}^T \| \leq c_x \sum_{j>k} \lambda_j.
    \end{align*}
    \item The second inequality.
    \begin{align*}
        \|(\lambda I_{n-k} + \Delta_{22})^{-1}\| \leq \| \Delta_{22}^{-1}\| \leq \|\Delta^{-1}\| = \| (X_{k:d}X_{k:d}^T)^{-1} \| \leq c_xL\pth{\sum_{j>k}\lambda_j}^{-1},
    \end{align*}
    where the second inequality holds because $\Delta$ is positive definite.
    \item The third inequality.
    \begin{align*}
        \left\| \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-2} \Delta_{12}^T \right\| \leq \| \Delta_{12}\|^2 \|(\lambda I_{n-k} + \Delta_{22})^{-1}\|^2 \leq c_x^4 L^2.
    \end{align*}
    \item The fourth inequality.
    \begin{align*}
         \left\| \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T \right\| \leq \| \Delta_{12}\|^2 \|(\lambda I_{n-k} + \Delta_{22})^{-1}\| \leq c_x^3 L \sum_{j>k}\lambda_j.
    \end{align*}
    \item The last inequality.
    \begin{align*}
        &\quad \left\| \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T \right\| \\
        &= \left\| \Delta_{11} +\lambda I_k - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T \right\| -\lambda \\
        &\leq \|\Delta_{11} + \lambda I_k \| - \lambda \\
        &= \|\Delta_{11}\| \\
        &\leq c_x \sum_{j>k} \lambda_j.
    \end{align*}
    The first inequality holds because $\Delta_{11} +\lambda I_k - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T$ is the Schur complement of the block $\Delta_{11} +\lambda I_k$ of the matrix $\Delta + \lambda I_n$, which is positive definite. Therefore, we have 
    \begin{align*}
        \Delta_{11} +\lambda I_k \succcurlyeq \Delta_{11} +\lambda I_k - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T.
    \end{align*}
\end{enumerate}
\end{proof}


\begin{lemma}
\label{lem:Akinverse_concentration}
Suppose the assumption condNum$(k,\delta,L)$ is satisfied. There exists a constant $c_x>2$ depending only on $\sigma_x$, such that for any $N_1<n<N_2$, with probability at least $1-2\delta-c_xe^{-n/c_x}$, on both events in Lemma~\ref{lem:xxT_concentration} and Lemma~\ref{lem:xTx_concentration},
\begin{align*}
    &\quad \left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} - \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} \right\| \\
    &\leq \frac{c_x^2\pth{\sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^2 L \sum_{j>k}\lambda_j}}{(\lambda+n\lambda_k)^2}.
\end{align*}
where 
\begin{align*}
    N_1 &= \max\sth{ 4c_x^4(k+\ln(1/\delta))\frac{\lambda_1^2}{\lambda_k^2}, 2c_x^4L \lambda_k^{-1}\sum_{j>k}\lambda_j }. \\
    N_2 &= \frac{1}{\lambda_{k+1}} \sum_{j>k}\lambda_j.
\end{align*}
\end{lemma}
\begin{proof}
\begin{align*}
    &\quad \left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} - \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} \right\| \\
    &\leq \left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1}\right\|  \\
    &\quad\cdot  \left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V} - \pth{n\tilde{\Sigma}_{S,0:k}} \right\| \\
    &\quad\cdot \left\| \pth{n\tilde{\Sigma}_{S,0:k}}^{-1}  \right\| \\
    &= \frac{1}{\lambda+n\lambda_k} \left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1}\right\| \\
    &\quad\cdot \left\| X_{0:k}^TX_{0:k} - n\Sigma_{S,0:k} + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V  \right\|.
\end{align*}
According to Lemma~\ref{lem:xTx_concentration}, Corollary~\ref{coroly:Delta}, there exists a constant $c_x>2$ depending only on $\sigma_x$, such that for any $k+\ln(1/\delta)<N_1<n<N_2=\frac{1}{\lambda_{k+1}} 
    \sum_{j>k}\lambda_j$, with probability at least $1-2\delta-c_xe^{-n/c_x}$, on both events in Lemma~\ref{lem:xxT_concentration} and Lemma~\ref{lem:xTx_concentration},
\begin{align*}
    \left\| \frac{1}{n}X_{0:k}^TX_{0:k} - \Sigma_{S,0:k} \right\| &\leq c_x \lambda_1 \sqrt{\frac{k+\operatorname{ln}\frac{1}{\delta}}{n}}. \\
    \left\| \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T \right\| &\leq c_x^3 L \sum_{j>k}\lambda_j.
\end{align*}
\begin{enumerate}
\item $\left\| X_{0:k}^TX_{0:k} - n\Sigma_{S,0:k} + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V  \right\|$.
\begin{align*}
    &\quad\left\| X_{0:k}^TX_{0:k} - n\Sigma_{S,0:k} + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V  \right\| \\
    &\leq  \pth{  \left\| X_{0:k}^TX_{0:k} - n\Sigma_{S,0:k}\right\| + \left\|\pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }  \right\| } \\
    &\leq c_x \sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^3 L \sum_{j>k}\lambda_j.
\end{align*}
\item $\left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1}\right\|$
\begin{align*}
    &\quad\frac{1}{\lambda+n\lambda_k} \left\| X_{0:k}^TX_{0:k} - n\Sigma_{S,0:k} + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V  \right\| \\
    &\leq  \frac{1}{\lambda+n\lambda_k} \pth{c_x \sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^3 L \sum_{j>k}\lambda_j }.
\end{align*}
Since $n>4c_x^4(k+\ln(1/\delta))\frac{\lambda_1^2}{\lambda_k^2}$, 
\begin{align*}
    \frac{1}{\lambda+n\lambda_k} c_x \sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 &\leq \frac{ c_x \sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 }{n\lambda_k} \\
    &= \frac{ c_x \sqrt{(k+\ln\frac{1}{\delta})}\lambda_1 }{\sqrt{n}\lambda_k} \\
    &< \frac{1}{2c_x}.
\end{align*}
Since $n>2c_x^4L \lambda_k^{-1}\sum_{j>k}\lambda_j$,
\begin{align*}
    \frac{1}{\lambda+n\lambda_k} c_x^3 L \sum_{j>k}\lambda_j &\leq \frac{c_x^3 L \sum_{j>k}\lambda_j } {n\lambda_k} \\
    &< \frac{1}{2c_x}.
\end{align*}
Therefore, we have
\begin{align*}
    \quad\frac{1}{\lambda+n\lambda_k} \left\| X_{0:k}^TX_{0:k} - n\Sigma_{S,0:k} + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V  \right\| < \frac{1}{c_x}.
\end{align*}
Now we derive the upper bound for our target.
\begin{align*}
    &\quad\left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1}\right\| \\
    &= \left\| \qth{n\tilde{\Sigma}_{S,0:k} + X_{0:k}^TX_{0:k} -n\Sigma_{S,0:k} + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1}\right\| \\
    &\leq \left\| \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} \right\| 
     \left[1 
     - \left\| \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} \right\| \right. \\
    &\left.\quad\cdot \left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1}\right\| \right]^{-1} \\
    &\leq \frac{1}{\lambda+n\lambda_k} \pth{1-\frac{1}{c_x}}^{-1} \\
    &\leq \frac{c_x}{\lambda+n\lambda_k}.
\end{align*}
The first inequality follows from the result $\|(A+T)^{-1}\| \leq \|A^{-1}\|\pth{1-\|A^{-1}\|\|T\|}^{-1}$, provided that both $A$ and $A+T$ are invertible and $\|A^{-1}\|\|T\|<1$~(see Lemma~3.1 in \cite{wedin1973perturbation}).
\end{enumerate}
Combining the above two inequalities, 
\begin{align*}
    &\quad \left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} - \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} \right\| \\
    &\leq \frac{1}{\lambda+n\lambda_k} \frac{c_x}{\lambda+n\lambda_k} \pth{c_x \sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^3 L \sum_{j>k}\lambda_j} \\
    &= \frac{c_x^2\pth{\sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^2 L \sum_{j>k}\lambda_j}}{(\lambda+n\lambda_k)^2}.
\end{align*}
\end{proof}

\subsection{Bias Variance Decomposition}
We consider the expection of the excess risk $\calR\pth{\hbeta(Y)}=\calR \pth{\hbeta(X\beta^\star) + \hbeta(\boldsymbol{\epsilon})}$ with respect to the distribution of the noise $\boldsymbol{\epsilon}$.
\begin{align*}
    \EE_{\boldsymbol{\epsilon}} \qth{\calR\pth{\hbeta(Y)}} &= \EE_{\boldsymbol{\epsilon}} \qth{\pth{\hbeta(Y)-\beta^\star}^T \Sigma_T \pth{\hbeta(Y)-\beta^\star}} \\
    &= \EE_{\boldsymbol{\epsilon}} \left[ 
    \pth{\hbeta(Y)_{0:k}-\beta^\star_{0:k}}^T \Sigma_{T,0:k} \pth{\hbeta(Y)_{0:k}-\beta^\star_{0:k}} \right. \\
    &\quad\left. + \pth{\hbeta(Y)_{k:d}-\beta^\star_{k:d}}^T \Sigma_{T,k:d} \pth{\hbeta(Y)_{k:d}-\beta^\star_{k:d}} \right. \\
    &\quad\left. + 2\pth{\hbeta(Y)_{0:k}-\beta^\star_{0:k}}^T \Sigma_{T}[0:k,k:d] \pth{\hbeta(Y)_{k:d}-\beta^\star_{k:d}} 
    \right] \\
    &\leq 2\EE_{\boldsymbol{\epsilon}} \qth{\pth{\hbeta(Y)_{0:k}-\beta^\star_{0:k}}^T \Sigma_{T,0:k} \pth{\hbeta(Y)_{0:k}-\beta^\star_{0:k}}} \\
    &\quad + 2\EE_{\boldsymbol{\epsilon}} \qth{\pth{\hbeta(Y)_{k:d}-\beta^\star_{k:d}}^T \Sigma_{T,k:d} \pth{\hbeta(Y)_{k:d}-\beta^\star_{k:d}}} \\
    &= 2\pth{\hbeta(X\beta^\star)_{0:k}-\beta^\star_{0:k}}^T \Sigma_{T,0:k} \pth{\hbeta(X\beta^\star)_{0:k}-\beta^\star_{0:k}} \\
    &\quad + 2\EE_{\boldsymbol{\epsilon}} \qth{\hbeta(\boldsymbol{\epsilon})_{0:k}^T \Sigma_{T,0:k} \hbeta(\boldsymbol{\epsilon})_{0:k}} \\
    &\quad + 2\pth{\hbeta(X\beta^\star)_{k:d}-\beta^\star_{k:d}}^T \Sigma_{T,k:d} \pth{\hbeta(X\beta^\star)_{k:d}-\beta^\star_{k:d}} \\
    &\quad + 2\EE_{\boldsymbol{\epsilon}} \qth{\hbeta(\boldsymbol{\epsilon})_{k:d}^T \Sigma_{T,k:d} \hbeta(\boldsymbol{\epsilon})_{k:d}}. 
\end{align*}
The first inequality follows from the result for a positive definite block quadratic form:
\begin{align*}
    (x_1^T, x_2^T)
    \begin{pmatrix}
        A & B \\
        B^T & D
    \end{pmatrix}
    \begin{pmatrix}
        x_1 \\
        x_2
    \end{pmatrix} = x_1^TAx_1 + 2x_1^TBx_2 + x_1^TDx_1,
\end{align*}
where the positive definiteness implies $x_1^TAx_1 + x_1^TDx_1 \geq 2x_1^TBx_2$.

We decompose the expected excess risk into variance and bias terms.
\begin{align*}
    V &= \EE_{\boldsymbol{\epsilon}} \qth{\hbeta(\boldsymbol{\epsilon})_{0:k}^T \Sigma_{T,0:k} \hbeta(\boldsymbol{\epsilon})_{0:k}}  + \EE_{\boldsymbol{\epsilon}} \qth{\hbeta(\boldsymbol{\epsilon})_{k:d}^T \Sigma_{T,k:d} \hbeta(\boldsymbol{\epsilon})_{k:d}}. \\
    B &= \pth{\hbeta(X\beta^\star)_{0:k}-\beta^\star_{0:k}}^T \Sigma_{T,0:k} \pth{\hbeta(X\beta^\star)_{0:k}-\beta^\star_{0:k}}  \\
    &\quad 
    + \pth{\hbeta(X\beta^\star)_{k:d}-\beta^\star_{k:d}}^T \Sigma_{T,k:d} \pth{\hbeta(X\beta^\star)_{k:d}-\beta^\star_{k:d}}.
\end{align*}

\begin{lemma}
\label{lem:all_concentration}
    Suppose the assumption condNum$(k,\delta,L)$~(Assumption~\ref{assum:condNum}) is satisfied. There exists a constant $c_x>2$ depending only on $\sigma_x$, such that for any $N_1<n<N_2$, with probability at least $1-2\delta-c_xe^{-n/c_x}$, the following inequalities hold at the same time:
\begin{align*}
    \mu_n(X_{k:d}X_{k:d}^T) &\geq \frac{1}{c_xL} \sum_{j>k} \lambda_j. \\
     \mu_1(X_{k:d}X_{k:d}^T) &\leq c_x \sum_{j>k} \lambda_j. \\
    \left\| \frac{1}{n}X_{0:k}^TX_{0:k} - \Sigma_{S,0:k} \right\| &\leq c_x \lambda_1 \sqrt{\frac{k+\operatorname{ln}\frac{1}{\delta}}{n}}. \\
    \left\| \left(X_{0:k}^TX_{0:k}\right)^{\frac{1}{2}} - \sqrt{n}\Sigma_{S,0:k}^{\frac{1}{2}} \right\| 
        &\leq c_x \sqrt {k+\ln{\frac{1}{\delta}}}\lambda_1\lambda_k^{-\frac{1}{2}}. \\
    \mu_k\pth{\Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}} &\geq \frac{1}{c_x}n.  \\
    \mu_1\pth{\Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}}  &\leq c_x n. \\
    \mu_1(X_{0:k}^TX_{0:k})  &\leq c_x\lambda_1n. \\
    \mu_k(X_{0:k}^TX_{0:k})  &\geq \frac{1}{c_x}\lambda_kn.\\
    \tr\pth{X_{k:d}\Sigma_{T,k:d}X_{k:d}^T} &\leq c_x n\tr\pth{\Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d} \Sigma_{S,k:d}^{\frac{1}{2}} }. \\
    (\beta^\star_{k:d})^TX_{k:d}^TX_{k:d}\beta^\star_{k:d} &\leq c_x n (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d}. \\
    \| \Delta_{11} \|,\| \Delta_{12}, \|\Delta\|  \| &\leq  c_x \sum_{j>k} \lambda_j. \\
    \|(\lambda I_{n-k} + \Delta_{22})^{-1}\|, \|\Delta^{-1}\| &\leq  c_xL\pth{\sum_{j>k}\lambda_j}^{-1}. \\
    \left\| \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-2} \Delta_{12}^T \right\| &\leq c_x^4 L^2. \\
    \left\| \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T \right\| &\leq c_x^3 L \sum_{j>k}\lambda_j. \\
    \left\| \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T \right\| &\leq c_x \sum_{j>k} \lambda_j. 
\end{align*}
And, 
\begin{align*}
    &\quad\left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k}   + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} - \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} \right\| \\
    &\leq \frac{c_x^2\pth{\sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^2 L \sum_{j>k}\lambda_j}}{(\lambda+n\lambda_k)^2}.     
\end{align*}
$N_1$ and $N_2$ are defined as follows:
\begin{align*}
    N_1 &= \max\sth{ 4c_x^4(k+\ln(1/\delta))\frac{\lambda_1^2}{\lambda_k^2}, 2c_x^4L \lambda_k^{-1}\sum_{j>k}\lambda_j }. \\
    N_2 &= \frac{1}{\lambda_{k+1}} \sum_{j>k}\lambda_j.
\end{align*}
\end{lemma}
\begin{proof}
    The lemma is a direct corollary from Lemma~\ref{lem:xxT_concentration}, Lemma~\ref{lem:xTx_concentration}, Corollary~\ref{coroly:xTxroot_concentration}, Lemma~\ref{lem:sxTxs_concentration}, Lemma~\ref{lem:xsTxT_concentration}, Lemma~\ref{lem:bxTxb_concentration}, Corollary~\ref{coroly:Delta}, Lemma~\ref{lem:Akinverse_concentration}.
\end{proof}


\subsubsection{Variance in the First \texorpdfstring{$k$}{k} Dimensions}
\begin{lemma}
\label{lem:var_0k}
    Under the same conditions as in Lemma~\ref{lem:all_concentration}, and on the same event, for any $N_1<n<N_2$,
    \begin{align*}
    	\EE_{\boldsymbol{\epsilon}} \qth{\hbeta(\boldsymbol{\epsilon})_{0:k}^T \Sigma_{T,0:k} \hbeta(\boldsymbol{\epsilon})_{0:k}} \leq 16\sigma^2(1+c_x^4L^2)\frac{1}{n} \tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}},
    \end{align*} 
    where
    \begin{equation*}
    \begin{alignedat}{2}
    N_1 &= \max \Bigg\{ 
        & & 4c_x^4 \left( k + \ln \frac{1}{\delta} \right) \lambda_1^4 \lambda_k^{-4}, \\
        & && 2c_x^4 L \lambda_1 \lambda_k^{-2} \sum_{j>k} \lambda_j, \\
        & && 4c_x^4 \left( k + \ln \frac{1}{\delta} \right) \lambda_1^6 \lambda_k^{-8} \|\Sigma_{T,0:k}\|^2 k^2 
        \left( \tr \left[ \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} 
        \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right] \right)^{-2}, \\
        & && 2c_x^4 L \lambda_1^2 \lambda_k^{-4} \left( \sum_{j>k} \lambda_j \right) \|\Sigma_{T,0:k}\| k 
        \left( \tr \left[ \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} 
        \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right] \right)^{-1}
    \Bigg\}, \\
    N_2 &= \frac{1}{\lambda_{k+1}} & & \sum_{j>k} \lambda_j.
    \end{alignedat}
    \end{equation*}
\end{lemma}
\begin{proof}
\begin{align*}
    &\quad \EE_{\boldsymbol{\epsilon}} \qth{\hbeta(\boldsymbol{\epsilon})_{0:k}^T \Sigma_{T,0:k} \hbeta(\boldsymbol{\epsilon})_{0:k}} \\
    &= \EE_{\boldsymbol{\epsilon}} \tr \qth{ \boldsymbol{\epsilon}\boldsymbol{\epsilon}^T (XX^T+\lambda I_n)^{-1} X_{0:k} \Sigma_{T,0:k} X_{0:k}^T (XX^T+\lambda I_n)^{-1}} \\
    &= \sigma^2 \tr \qth{(XX^T+\lambda I_n)^{-1} X_{0:k} \Sigma_{T,0:k} X_{0:k}^T (XX^T+\lambda I_n)^{-1}} \\
    &= \sigma^2 \tr \left[ (UMU^T+U\Delta U^T+\lambda I_n)^{-1} U \tilde{M}^{\frac{1}{2}} V \Sigma_{T,0:k} \right.\\
    &\left. \quad \cdot V^T \pth{\tilde{M}^{\frac{1}{2}}}^T U^T (UMU^T+U\Delta U^T+\lambda I_n)^{-1}  \right] \\
    &= \sigma^2 \tr \left[ U(M+\Delta +\lambda I_n)^{-1}  \tilde{M}^{\frac{1}{2}} V \Sigma_{T,0:k} 
    V^T \pth{\tilde{M}^{\frac{1}{2}}}^T  (M+\Delta +\lambda I_n)^{-1} U^T  \right] \\
    &= \sigma^2 \tr \qth{\pth{\tilde{M}^{\frac{1}{2}}}^T  (M+\Delta +\lambda I_n)^{-1} (M+\Delta +\lambda I_n)^{-1}  \tilde{M}^{\frac{1}{2}} V \Sigma_{T,0:k} 
    V^T   } \\
    &=  \sigma^2 \tr \left[M_k^{\frac{1}{2}} \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1}
    \pth{I_k, - \Delta_{12}(\lambda I_{n-k} + \Delta_{22})^{-1} } \right.\\
    &\left.\quad \cdot \pth{I_k, - \Delta_{12}(\lambda I_{n-k} + \Delta_{22})^{-1} }^T
    \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} M_k^{\frac{1}{2}} \right. \\
    &\left.\quad \cdot V\Sigma_{T,0:k}V^T \right]  \\
    &= \sigma^2 \tr \left[M_k^{\frac{1}{2}} \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right.\\
    &\left.\quad \cdot \pth{I_k + \Delta_{12}(\lambda I_{n-k} + \Delta_{22})^{-2}\Delta_{12}^T }  
    \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} M_k^{\frac{1}{2}} \right. \\
    &\left.\quad \cdot V\Sigma_{T,0:k}V^T \right]  \\
    &= \sigma^2 \tr \left[
     \pth{I_k + \Delta_{12}(\lambda I_{n-k} + \Delta_{22})^{-2}\Delta_{12}^T }  
    \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right. \\
    &\left.\quad \cdot M_k^{\frac{1}{2}} V\Sigma_{T,0:k}V^T M_k^{\frac{1}{2}} \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1}\right]  \\
    &\leq \sigma^2 \left\| I_k + \Delta_{12}(\lambda I_{n-k} + \Delta_{22})^{-2}\Delta_{12}^T  \right\|
    \tr \left[ \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right. \\
    &\left.\quad \cdot M_k^{\frac{1}{2}}  V\Sigma_{T,0:k}V^T M_k^{\frac{1}{2}} \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right] \\
    &\leq \sigma^2 (1+c_x^4L^2) \tr \left[ \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right. \\
    &\left.\quad \cdot M_k^{\frac{1}{2}}  V\Sigma_{T,0:k}V^T M_k^{\frac{1}{2}} \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right] \\
    &= \sigma^2 (1+c_x^4L^2) \tr \left[ \pth{V^T\pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} \right. \\
    &\left.\quad \cdot V^TM_k^{\frac{1}{2}}  V\cdot\Sigma_{T,0:k}\cdot V^T M_k^{\frac{1}{2}}V\cdot \pth{V^T\pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T}V}^{-1} \right] \\
    &= \sigma^2 (1+c_x^4L^2) \tr \left[ \pth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} \right. \\
    &\left.\quad \cdot \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} \right.\\
     &\left.\quad \cdot \pth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} \right].
\end{align*}
The sixth equation follows from Equation~\ref{eq:A_kinverse_firstkrows}. The first inequality follows from the result $\tr[AB] \leq \|A\|\tr[B]$ where the matrix $B$ is positive semi-definite.

We define two quantities that represent concentration error terms:
\begin{align*}
    E_1&=\left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} - \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} \right\|. \\
    E_2 &= \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} - \pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}.
\end{align*}
Since $n> 4c_x^4\pth{k+\ln\frac{1}{\delta}}\lambda_1^6 \lambda_k^{-8}\|\Sigma_{T,0:k}\|^2 k^2\pth{\tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}  } }^{-2}$,\\
and $n> 2c_x^4L \pth{\sum_{j>k} \lambda_j} \lambda_1^2\lambda_k^{-4} \|\Sigma_{T,0:k}\| k\pth{\tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}  } }^{-1}$,
\begin{align*}
    &\quad\|E_1\| \left\|n\tilde{\Sigma}_{S,0:k}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\|  \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\Sigma_{T,0:k}\right\| \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
    &\leq \frac{c_x^2\pth{\sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^2 L \sum_{j>k}\lambda_j}}{(\lambda+n\lambda_k)^2} \pth{\lambda+n\lambda_1} \frac{n\lambda_1}{(\lambda+n\lambda_k)^2} \|\Sigma_{T,0:k} \| \\
    &\leq \frac{c_x^2\pth{\sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^2 L \sum_{j>k}\lambda_j}}{n^2}  \frac{\lambda_1^2}{\lambda_k^4} \|\Sigma_{T,0:k} \| \\
    &=  \frac{c_x^2\sqrt{(k+\ln\frac{1}{\delta})}}{n\sqrt{n}}  \frac{\lambda_1^3}{\lambda_k^4} \|\Sigma_{T,0:k}\|
     + \frac{c_x^4 L \sum_{j>k}\lambda_j}{n^2}  \frac{\lambda_1^2}{\lambda_k^4} \|\Sigma_{T,0:k}\| \\
    &< \frac{1}{2nk}\tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}} + \frac{1}{2nk}\tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}} \\
    &= \frac{1}{k}\tr \qth{\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}}.
\end{align*}
Since $n> 4c_x^4\pth{k+\ln\frac{1}{\delta}}\lambda_1^4 \lambda_k^{-4}$ and $n> 2c_x^4L \pth{\sum_{j>k} \lambda_j} \lambda_1\lambda_k^{-2}$,
\begin{align}
\begin{split}
\label{eq:E1nS_leq1}
	 &\quad\|E_1\| \left\|n\tilde{\Sigma}_{S,0:k}\right\| \\
	 &\leq \frac{c_x^2\pth{\sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^2 L \sum_{j>k}\lambda_j}}{(\lambda+n\lambda_k)^2} \pth{\lambda+n\lambda_1} \\
	 &\leq \frac{c_x^2\pth{\sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^2 L \sum_{j>k}\lambda_j}}{n} \frac{\lambda_1}{\lambda_k^2} \\
	 &= \frac{c_x^2\sqrt{(k+\ln\frac{1}{\delta})}}{\sqrt{n}} \frac{\lambda_1^2}{\lambda_k^2} + \frac{c_x^4 L \sum_{j>k}\lambda_j}{n} \frac{\lambda_1}{\lambda_k^2} \\
	 &< \frac{1}{2} + \frac{1}{2} \\
	 &= 1.
\end{split}
\end{align}
Since $n> c_x^2\pth{k+\ln\frac{1}{\delta}}\lambda_1^4 \lambda_k^{-6}\|\Sigma_{T,0:k}\|^2 k^2\pth{\tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}  } }^{-2}$,
\begin{align*}
	&\quad\|E_2\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\|  \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\Sigma_{T,0:k}\right\| \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
	&\leq c_x \sqrt {k+\ln{\frac{1}{\delta}}}\lambda_1\lambda_k^{-\frac{1}{2}} \pth{n\lambda_k}^{-\frac{1}{2}} \frac{n\lambda_1}{(\lambda+n\lambda_k)^2} \|\Sigma_{T,0:k}\| \\
	&\leq \frac{c_x \sqrt {k+\ln{\frac{1}{\delta}}}}{n\sqrt{n}} \frac{\lambda_1^2}{\lambda_k^3} \|\Sigma_{T,0:k}\| \\
	&\leq \frac{1}{nk} \tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}} \\
	&= \frac{1}{k}\tr \qth{\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}}.
\end{align*}
Since $n> c_x^2\pth{k+\ln\frac{1}{\delta}}\lambda_1^2 \lambda_k^{-2}$,
\begin{align}
\begin{split}
\label{eq:E2nS_leq1}
    &\quad\|E_2\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}}\right\| \\
	&\leq c_x \sqrt {k+\ln{\frac{1}{\delta}}}\lambda_1\lambda_k^{-\frac{1}{2}} \pth{n\lambda_k}^{-\frac{1}{2}} \\
	&= \frac{c_x\sqrt {k+\ln{\frac{1}{\delta}}}}{\sqrt{n}}\frac{\lambda_1}{\lambda_k} \\
	&< 1.
\end{split}
\end{align}
Combing the above four inequalities, we have
\begin{align*}
    &\quad \tr \left[ \pth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} \right. \\
    &\left.\quad\quad \cdot \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} \right.\\
    &\left.\quad\quad \cdot \pth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} \right] \\
    &= \tr \qth{\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}} \\
    &\quad + 2\tr \qth{E_1\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}} \\
    &\quad + 2\tr \qth{\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}E_2\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}} \\
    &\quad +\tr \qth{E_1\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}E_1} \\
    &\quad + \tr \qth{\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}E_2\Sigma_{T,0:k}E_2\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}} \\
    &\quad + 2\tr \qth{E_1\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}E_2\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}} \\
    &\quad + 2\tr \qth{E_1E_2\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}} \\
    &\quad + 2\tr \qth{E_1E_2\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}E_1} \\
    &\quad + 2\tr \qth{E_1E_2\Sigma_{T,0:k}E_2\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}} \\
    &\quad + \tr \qth{E_1E_2\Sigma_{T,0:k}E_2E_1}. 
\end{align*}
In particular,
\begin{align*}
     &\quad \tr \qth{E_1E_2\Sigma_{T,0:k}E_2E_1} \\
     &= \tr \left[E_1 n\tilde{\Sigma}_{S,0:k} \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} E_2 \pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}} \pth{n\tilde{\Sigma}_{S,0:k}}^{\frac{1}{2}} \right. \\ &\left.\quad\cdot\Sigma_{T,0:k} E_2 \pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}} \pth{n\tilde{\Sigma}_{S,0:k}}^{\frac{1}{2}} E_1 n\tilde{\Sigma}_{S,0:k} \pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right] \\
     &\leq k \pth{\|E_1\| \left\|n\tilde{\Sigma}_{S,0:k}\right\|}^2 \pth{\|E_2\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}}\right\|} \\
     &\quad\cdot  \|E_2\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\|  \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\Sigma_{T,0:k}\right\| \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
     &\leq  \tr \qth{\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}}.
\end{align*}
The other terms can be similarly bounded. Therefore,
\begin{align*}
    &\quad \tr \left[ \pth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} \right. \\
    &\left.\quad\quad \cdot \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} \right.\\
    &\left.\quad\quad \cdot \pth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} \right] \\
    &\leq 16 \tr \qth{\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}} \\
    &= \frac{16}{n}  \tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}}.
\end{align*}
The proof is complete by combing all the inequalities above.
\end{proof}

\subsubsection{Variance in the Last \texorpdfstring{$d-k$}{d-k} Dimensions}
\begin{lemma}
\label{lem:var_kd}
    Under the same conditions as in Lemma~\ref{lem:all_concentration}, and on the same event, for any $N_1<n<N_2$,
    \begin{align*}
    	\EE_{\boldsymbol{\epsilon}} \qth{\hbeta(\boldsymbol{\epsilon})_{k:d}^T \Sigma_{T,k:d} \hbeta(\boldsymbol{\epsilon})_{k:d}}
     \leq \sigma^2 c_xn \pth{\lambda+\frac{1}{c_xL} \sum_{j>k} \lambda_j}^{-2} \tr\qth{\Sigma_{S,k:d}^{\frac{1}{2}}\Sigma_{T,k:d} \Sigma_{S,k:d}^{\frac{1}{2}} } .
    \end{align*} 
    where $N_1,N_2$ are defined as in Lemma~\ref{lem:all_concentration}.
\end{lemma}
\begin{proof}
\begin{align*}
    &\quad \EE_{\boldsymbol{\epsilon}} \qth{\hbeta(\boldsymbol{\epsilon})_{k:d}^T \Sigma_{T,k:d} \hbeta(\boldsymbol{\epsilon})_{k:d}} \\
    &= \EE_{\boldsymbol{\epsilon}} \tr \qth{ \boldsymbol{\epsilon}\boldsymbol{\epsilon}^T (XX^T+\lambda I_n)^{-1} X_{k:d} \Sigma_{T,k:d} X_{k:d}^T (XX^T+\lambda I_n)^{-1}} \\
    &= \sigma^2 \tr \qth{(XX^T+\lambda I_n)^{-1} X_{k:d} \Sigma_{T,k:d} X_{k:d}^T (XX^T+\lambda I_n)^{-1}} \\
    &\leq \sigma^2 \left\| (XX^T+\lambda I_n)^{-2} \right\| \tr \qth{X_{k:d} \Sigma_{T,k:d} X_{k:d}^T} \\
    &\leq \sigma^2 \left\| (X_{k:d}X_{k:d}^T+\lambda I_n)^{-2} \right\| \tr \qth{X_{k:d} \Sigma_{T,k:d} X_{k:d}^T} \\
    &\leq \sigma^2  \pth{\lambda+\frac{1}{c_xL} \sum_{j>k} \lambda_j}^{-2} 
    c_x n\tr\qth{\Sigma_{S,k:d}^{\frac{1}{2}}\Sigma_{T,k:d} \Sigma_{S,k:d}^{\frac{1}{2}} }.
\end{align*}
The first inequality follows from the result $\tr [ABA] = \tr [A^2B] \leq \|A^2\| \tr [B]$ where the matrix $B$ is positive semi-definite. The second inequality follows from $XX^T+\lambda I_n \succcurlyeq X_{k:d}X_{k:d}^T+\lambda I_n$.
\end{proof}

\subsubsection{Bias in the First \texorpdfstring{$k$}{k} Dimensions}
The bias in the first $k$ dimensions can be decomposed into two terms.
\begin{align*}
    &\quad \pth{\hbeta(X\beta^\star)_{0:k}-\beta^\star_{0:k}}^T \Sigma_{T,0:k} \pth{\hbeta(X\beta^\star)_{0:k}-\beta^\star_{0:k}} \\
    &= \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X \beta^\star - \beta^\star_{0:k} }^T \Sigma_{T,0:k} \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X \beta^\star - \beta^\star_{0:k} } \\
    &\leq 2\pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \beta^\star_{0:k} - \beta^\star_{0:k} }^T \Sigma_{T,0:k} \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \beta^\star_{0:k} - \beta^\star_{0:k} }  \\
    &\quad + 2 \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \beta^\star_{k:d}}^T \Sigma_{T,0:k} \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \beta^\star_{k:d}}.
\end{align*}
The inequality follows from the result $x_1^TAx_1 + x_2^TAx_2 \geq 2x_1^TAx_2$ where $A$ is positive semi-definite.
\begin{lemma}
\label{lem:bias_0k_1}
    Under the same conditions as in Lemma~\ref{lem:all_concentration}, and on the same event, for any $N_1<n<N_2$,
    \begin{align*}
    &\quad \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \beta^\star_{0:k} - \beta^\star_{0:k} }^T \Sigma_{T,0:k} \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \beta^\star_{0:k} - \beta^\star_{0:k}} \\
    &\leq \frac{4c_x^2}{n^2} \pth{\lambda + c_x \sum_{j>k} \lambda_j}^2 (\beta^\star_{0:k})^T \Sigma_{S,0:k}^{-1}   \beta^\star_{0:k} 
    \left\|\Sigma_{S,0:k}^{-\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}   \right\|.
\end{align*}
    where
    \begin{equation*}
    \begin{alignedat}{2}
    N_1 &= \max \Bigg\{ 
        & & c_x^2 (\lambda + c_x \sum_{j>k} \lambda_j) \lambda_1 \lambda_k^{-2}, \\
        &&& 4c_x^4(k+\ln(1/\delta))\frac{\lambda_1^2}{\lambda_k^2}, \\
        & && 2c_x^4 L \lambda_1 \lambda_k^{-2} \sum_{j>k} \lambda_j
    \Bigg\}, \\
    N_2 &= \frac{1}{\lambda_{k+1}} & & \sum_{j>k} \lambda_j.
    \end{alignedat}
    \end{equation*}
\end{lemma}
\begin{proof}
\begin{align*}
     &\quad \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \beta^\star_{0:k} - \beta^\star_{0:k} }^T \Sigma_{T,0:k} \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \beta^\star_{0:k} - \beta^\star_{0:k}} \\
     &= (\beta^\star_{0:k})^T \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} - I_k}^T \Sigma_{T,0:k} \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} - I_k}\beta^\star_{0:k} \\
     &= (\beta^\star_{0:k})^T \Sigma_{S,0:k}^{-\frac{1}{2}} 
     \pth{\Sigma_{S,0:k}^{\frac{1}{2}} X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \Sigma_{S,0:k}^{\frac{1}{2}} - \Sigma_{S,0:k}}^T \Sigma_{S,0:k}^{-\frac{1}{2}}  \\
     &\quad \cdot \Sigma_{T,0:k} \Sigma_{S,0:k}^{-\frac{1}{2}} 
     \pth{\Sigma_{S,0:k}^{\frac{1}{2}} X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \Sigma_{S,0:k}^{\frac{1}{2}} - \Sigma_{S,0:k}}^T \Sigma_{S,0:k}^{-\frac{1}{2}} \beta^\star_{0:k} \\
     &\leq (\beta^\star_{0:k})^T \Sigma_{S,0:k}^{-1}   \beta^\star_{0:k} 
     \cdot \left\|\Sigma_{S,0:k}^{-\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}   \right\| \\
     &\quad \cdot \left\| \Sigma_{S,0:k}^{\frac{1}{2}} X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \Sigma_{S,0:k}^{\frac{1}{2}} - \Sigma_{S,0:k} \right\|^2.
\end{align*}
Subsequently,
\begin{align*}
    &\quad \left\| \Sigma_{S,0:k}^{\frac{1}{2}} X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \Sigma_{S,0:k}^{\frac{1}{2}} - \Sigma_{S,0:k} \right\| \\
    &= \left\| \Sigma_{S,0:k}^{\frac{1}{2}} 
    V^T \pth{\tilde{M}^{\frac{1}{2}}}^T U^T U (M+\lambda I_n + \Delta)^{-1} U^TU \tilde{M}^{\frac{1}{2}} V
    \Sigma_{S,0:k}^{\frac{1}{2}} - \Sigma_{S,0:k} \right\| \\
    &= \left\| \Sigma_{S,0:k}^{\frac{1}{2}} 
    V^T M_k^{\frac{1}{2}} \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} M_k^{\frac{1}{2}}  V
    \Sigma_{S,0:k}^{\frac{1}{2}} - \Sigma_{S,0:k} \right\| \\
    &= \left\| \Sigma_{S,0:k}^{\frac{1}{2}} 
    \pth{V^T M_k^{-\frac{1}{2}} \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V}^{-1}
    \Sigma_{S,0:k}^{\frac{1}{2}} \right. \\
    &\left.\quad - \Sigma_{S,0:k} \right\| \\
    &= \left\| \Sigma_{S,0:k}^{\frac{1}{2}} 
    \pth{I_k+ V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V}^{-1}
    \Sigma_{S,0:k}^{\frac{1}{2}} \right. \\
    &\left.\quad - \Sigma_{S,0:k} \right\| \\
    &= \left\| \Sigma_{S,0:k}^{\frac{1}{2}} 
    \left( \pth{I_k+ V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V}^{-1} - I_k \right) \right. \\
    &\left.\quad\cdot\Sigma_{S,0:k}^{\frac{1}{2}}  \right\| \\
    &= \left\| \Sigma_{S,0:k}^{\frac{1}{2}}  V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V \right. \\
    &\left.\quad\cdot \pth{I_k+ V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V}^{-1}  
    \Sigma_{S,0:k}^{\frac{1}{2}}  \right\| \\
    &\leq \left\| \Sigma_{S,0:k}^{\frac{1}{2}}  V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V   
    \Sigma_{S,0:k}^{\frac{1}{2}}  \right\| \\
    &\quad +\left\| \Sigma_{S,0:k}^{\frac{1}{2}}  V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V \right. \\
    &\left.\quad\cdot \qth{\pth{I_k+ V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V}^{-1}  -I_k}
    \Sigma_{S,0:k}^{\frac{1}{2}}  \right\|.
\end{align*}
The second equation follows from Equation~\ref{eq:A_kinverse_firstkrows}. 

We will derive upper bounds for both terms in the last equation above.
\begin{enumerate}
    \item The first term.
    \begin{align*}
        &\quad \left\| \Sigma_{S,0:k}^{\frac{1}{2}}  V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V   
    \Sigma_{S,0:k}^{\frac{1}{2}}  \right\| \\
    &\leq \left\| \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T  \right\| 
    \left\| \Sigma_{S,0:k}^{\frac{1}{2}}  V^T M_k^{-1} V  \Sigma_{S,0:k}^{\frac{1}{2}}  \right\| \\
    &= \left\| \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T  \right\| 
    \left\| \pth{\Sigma_{S,0:k}^{-\frac{1}{2}}  \pth{X_{0:k}^TX_{0:k}}^{-1}  \Sigma_{S,0:k}^{-\frac{1}{2}} }^{-1} \right\| \\
    &\leq \pth{\lambda + c_x \sum_{j>k} \lambda_j} \frac{c_x}{n}.
    \end{align*}
    \item The second term.

    Since $n>c_x^2(\lambda + c_x \sum_{j>k} \lambda_j)\lambda_k^{-1}$,
    \begin{align*}
        &\quad \left\| M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}} \right\| \\
        &\leq \left\|M_k^{-1}\right\|  \left\| \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T  \right\| \\
        &\leq \frac{c_x}{n\lambda_k} \pth{\lambda + c_x \sum_{j>k} \lambda_j} \\
        &< \frac{1}{c_x}.
    \end{align*}
    Therefore,
    \begin{align*}
        &\quad \left\| \pth{I_k+ V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V}^{-1}  -I_k \right\| \\
        &\leq \left\| \pth{I_k+ V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V}^{-1} \right\|  \\
        &\quad\cdot \left\| V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V \right\| \\
        &\leq \pth{1-\frac{1}{c_x}}^{-1} \left\| V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V \right\| \\
        &\leq c_x \cdot \frac{c_x}{n\lambda_k} \pth{\lambda + c_x \sum_{j>k} \lambda_j} \\
        &= \frac{c_x^2}{n} \frac{\lambda + c_x \sum_{j>k} \lambda_j}{\lambda_k}.
    \end{align*}
     The second inequality follows from  $\|(A+T)^{-1}\| \leq \|A^{-1}\|\pth{1-\|A^{-1}\|\|T\|}^{-1}$, where both $A$ and $A+T$ are invertible and $\|A^{-1}\|\|T\|<1$. Note that $c_x>2$.

     Since $n>c_x^2 (\lambda + c_x \sum_{j>k} \lambda_j) \lambda_1 \lambda_k^{-2}$,
     \begin{align*}
         &\quad \left\| \Sigma_{S,0:k}^{\frac{1}{2}}  V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V \right. \\
        &\left.\quad\cdot \qth{\pth{I_k+ V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V}^{-1}  -I_k}
        \Sigma_{S,0:k}^{\frac{1}{2}}  \right\| \\
        &\leq \| \Sigma_{S,0:k}\| \left\| M_k^{-1} \right\| \left\| \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T \right\| \\
        &\quad \cdot \left\| \pth{I_k+ V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V}^{-1}  -I_k \right\| \\
        &\leq \lambda_1 \frac{c_x}{n\lambda_k} \pth{\lambda + c_x \sum_{j>k} \lambda_j} \frac{c_x^2}{n} \frac{\lambda + c_x \sum_{j>k} \lambda_j}{\lambda_k} \\
        &= \frac{1}{n}\frac{c_x^3}{n}\lambda_1\lambda_k^{-2} \pth{\lambda + c_x \sum_{j>k} \lambda_j}^2 \\
        &< \frac{c_x}{n} \pth{\lambda + c_x \sum_{j>k} \lambda_j}.
     \end{align*}
\end{enumerate}
Combining both terms above, we have
\begin{align*}
    \left\| \Sigma_{S,0:k}^{\frac{1}{2}} X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \Sigma_{S,0:k}^{\frac{1}{2}} - \Sigma_{S,0:k} \right\|
    \leq \frac{2c_x}{n} \pth{\lambda + c_x \sum_{j>k} \lambda_j}.
\end{align*}
Therefore, 
\begin{align*}
    &\quad \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \beta^\star_{0:k} - \beta^\star_{0:k} }^T \Sigma_{T,0:k} \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \beta^\star_{0:k} - \beta^\star_{0:k}} \\
    &\leq (\beta^\star_{0:k})^T \Sigma_{S,0:k}^{-1}   \beta^\star_{0:k} 
     \cdot \left\|\Sigma_{S,0:k}^{-\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}   \right\| \\
    &\quad \cdot \left\| \Sigma_{S,0:k}^{\frac{1}{2}} X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \Sigma_{S,0:k}^{\frac{1}{2}} - \Sigma_{S,0:k} \right\|^2 \\
    &\leq \frac{4c_x^2}{n^2} \pth{\lambda + c_x \sum_{j>k} \lambda_j}^2 (\beta^\star_{0:k})^T \Sigma_{S,0:k}^{-1}   \beta^\star_{0:k} 
    \left\|\Sigma_{S,0:k}^{-\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}   \right\|.
\end{align*}
\end{proof}

\begin{lemma}
\label{lem:bias_0k_2}
    Under the same conditions as in Lemma~\ref{lem:all_concentration}, and on the same event, for any $N_1<n<N_2$,
    \begin{align*}
    &\quad \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \beta^\star_{k:d}}^T \Sigma_{T,0:k} \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \beta^\star_{k:d}} \\
    &\leq 16c_x(1+c_x^4L^2)  \left\| \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right\|  (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d}.
    \end{align*}
    where
    \begin{equation*}
    \begin{alignedat}{2}
    N_1 &= \max \Bigg\{ 
        & & 4c_x^4 \left( k + \ln \frac{1}{\delta} \right) \lambda_1^4 \lambda_k^{-4}, \\
        & && 2c_x^4 L \lambda_1 \lambda_k^{-2} \sum_{j>k} \lambda_j, \\
        & &&  4c_x^4\pth{k+\ln\frac{1}{\delta}}\lambda_1^6 \lambda_k^{-8}\|\Sigma_{T,0:k}\|^2 \left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}   \right\|^{-2}, \\
        & && 2c_x^4L \pth{\sum_{j>k} \lambda_j} \lambda_1^2\lambda_k^{-4} \|\Sigma_{T,0:k}\| \left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}   \right\|^{-1}
    \Bigg\}, \\
    N_2 &= \frac{1}{\lambda_{k+1}} & & \sum_{j>k} \lambda_j.
    \end{alignedat}
    \end{equation*}
\end{lemma}
\begin{proof}
\begin{align*}
    &\quad \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \beta^\star_{k:d}}^T \Sigma_{T,0:k} \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \beta^\star_{k:d}}   \\
    &\leq \left\| (XX^T+\lambda I_n)^{-1} X_{0:k}\Sigma_{T,0:k}X_{0:k}^T (XX^T+\lambda I_n)^{-1} \right\| \cdot (\beta^\star_{k:d})^T X_{k:d}^TX_{k:d}\beta^\star_{k:d}.
\end{align*}
From Lemma~\ref{lem:all_concentration}, 
\begin{align*}
     (\beta^\star_{k:d})^T X_{k:d}^TX_{k:d}\beta^\star_{k:d} \leq c_x n (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d}.
\end{align*}
In the following, we derive an upper bound for the other term.
\begin{align*}
    &\quad \left\| (XX^T+\lambda I_n)^{-1} X_{0:k}\Sigma_{T,0:k}X_{0:k}^T (XX^T+\lambda I_n)^{-1} \right\| \\
    &= \left\| (M+\lambda I_n + \Delta)^{-1} \tilde{M}^{\frac{1}{2}} V \Sigma_{T,0:k} V^T \pth{\tilde{M}^{\frac{1}{2}}}^T  (M+\lambda I_n + \Delta)^{-1} \right\| \\
    &= \left\| \Sigma_{T,0:k}^{\frac{1}{2}} V^T \pth{\tilde{M}^{\frac{1}{2}}}^T  (M+\lambda I_n + \Delta)^{-2} \tilde{M}^{\frac{1}{2}} V \Sigma_{T,0:k}^{\frac{1}{2}} \right\| \\
    &= \left\| \Sigma_{T,0:k}^{\frac{1}{2}} V^T M_{k}^{\frac{1}{2}} \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right. \\
    &\left.\quad \cdot \pth{I_k + \Delta_{12}(\lambda I_{n-k} + \Delta_{22})^{-2}\Delta_{12}^T}
    \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right. \\
    &\left. \quad \cdot M_{k}^{\frac{1}{2}} V  \Sigma_{T,0:k}^{\frac{1}{2}}  \right\| \\
    &\leq \left\| I_k + \Delta_{12}(\lambda I_{n-k} + \Delta_{22})^{-2}\Delta_{12}^T \right\| \\
    &\quad \cdot \left\| \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1}  M_{k}^{\frac{1}{2}} V  \Sigma_{T,0:k} \right. \\
    &\left.\quad\cdot V^TM_{k}^{\frac{1}{2}}\pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right\| \\
    &\leq (1+c_x^4L^2)  \left\| \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1}  M_{k}^{\frac{1}{2}} V  \Sigma_{T,0:k} \right. \\
    &\left.\quad\cdot V^TM_{k}^{\frac{1}{2}}\pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right\| \\
    &= (1+c_x^4L^2) \left\| \pth{V^T \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }  V}^{-1} \right.\\
    &\left.\quad\cdot V^TM_{k}^{\frac{1}{2}} V \Sigma_{T,0:k}  V^TM_{k}^{\frac{1}{2}} V \right.\\
    &\left.\quad\cdot \pth{V^T \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }  V}^{-1} \right\| \\
    &= (1+c_x^4L^2) \left\| \pth{X_{0:k}^TX_{0:k} +\lambda I_k + V^T(\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T)V }^{-1} \right.\\
    &\left.\quad\cdot  \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} \Sigma_{T,0:k} \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} \right. \\
    &\left.\quad\cdot  \pth{X_{0:k}^TX_{0:k} +\lambda I_k + V^T(\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T)V }^{-1} \right\|.
\end{align*}
The third equation follows from Equation~\ref{eq:A_kinverse_firstkrows}.

We define two quantities that represent concentration error terms:
\begin{align*}
    E_1&=\left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} - \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} \right\|. \\
    E_2 &= \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} - \pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}.
\end{align*}
Since $n> 4c_x^4\pth{k+\ln\frac{1}{\delta}}\lambda_1^6 \lambda_k^{-8}\|\Sigma_{T,0:k}\|^2 \left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}   \right\|^{-2}$,\\
and $n> 2c_x^4L \pth{\sum_{j>k} \lambda_j} \lambda_1^2\lambda_k^{-4} \|\Sigma_{T,0:k}\| \left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}   \right\|^{-1}$,
\begin{align*}
    &\quad\|E_1\| \left\|n\tilde{\Sigma}_{S,0:k}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\|  \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\Sigma_{T,0:k}\right\| \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
    &\leq \frac{c_x^2\pth{\sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^2 L \sum_{j>k}\lambda_j}}{(\lambda+n\lambda_k)^2} \pth{\lambda+n\lambda_1} \frac{n\lambda_1}{(\lambda+n\lambda_k)^2} \|\Sigma_{T,0:k} \| \\
    &\leq \frac{c_x^2\pth{\sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^2 L \sum_{j>k}\lambda_j}}{n^2}  \frac{\lambda_1^2}{\lambda_k^4} \|\Sigma_{T,0:k} \| \\
    &=  \frac{c_x^2\sqrt{(k+\ln\frac{1}{\delta})}}{n\sqrt{n}}  \frac{\lambda_1^3}{\lambda_k^4} \|\Sigma_{T,0:k}\|
     + \frac{c_x^4 L \sum_{j>k}\lambda_j}{n^2}  \frac{\lambda_1^2}{\lambda_k^4} \|\Sigma_{T,0:k}\| \\
    &< \frac{1}{2n}\left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}\right\| + \frac{1}{2n}\left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}\right\| \\
    &= \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\|.
\end{align*}
Similar to Equation~\ref{eq:E1nS_leq1}, since $n> 4c_x^4\pth{k+\ln\frac{1}{\delta}}\lambda_1^4 \lambda_k^{-4}$ and $n> 2c_x^4L \pth{\sum_{j>k} \lambda_j} \lambda_1\lambda_k^{-2}$,
\begin{align*}
    \|E_1\| \left\|n\tilde{\Sigma}_{S,0:k}\right\| < 1.
\end{align*}
Since $n> c_x^2\pth{k+\ln\frac{1}{\delta}}\lambda_1^4 \lambda_k^{-6}\|\Sigma_{T,0:k}\|^2 \left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}   \right\|^{-2}$,
\begin{align*}
	&\quad\|E_2\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\|  \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\Sigma_{T,0:k}\right\| \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
	&\leq c_x \sqrt {k+\ln{\frac{1}{\delta}}}\lambda_1\lambda_k^{-\frac{1}{2}} \pth{n\lambda_k}^{-\frac{1}{2}} \frac{n\lambda_1}{(\lambda+n\lambda_k)^2} \|\Sigma_{T,0:k}\| \\
	&\leq \frac{c_x \sqrt {k+\ln{\frac{1}{\delta}}}}{n\sqrt{n}} \frac{\lambda_1^2}{\lambda_k^3} \|\Sigma_{T,0:k}\| \\
	&\leq \frac{1}{n}\left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}\right\| \\
	&=\left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\|.
\end{align*}
Similar to Equation~\ref{eq:E2nS_leq1}, since $n> c_x^2\pth{k+\ln\frac{1}{\delta}}\lambda_1^2 \lambda_k^{-2}$,
\begin{align*}
    \|E_2\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}}\right\| < 1.
\end{align*}
Combining the four inequalities above,
\begin{align*}
    &\quad \left\| \pth{X_{0:k}^TX_{0:k} +\lambda I_k + V^T(\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T)V }^{-1} \right.\\
    &\left.\quad\cdot  \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} \Sigma_{T,0:k} \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} \right. \\
    &\left.\quad\cdot  \pth{X_{0:k}^TX_{0:k} +\lambda I_k + V^T(\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T)V }^{-1} \right\| \\
    &\leq \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1} \right\| \\
    &\quad + 2\left\|E_1\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
    &\quad + 2\left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}E_2\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
    &\quad +\left\|E_1\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}E_1\right\| \\
    &\quad + \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}E_2\Sigma_{T,0:k}E_2\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
    &\quad + 2\left\|E_1\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}E_2\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
    &\quad + 2\left\|E_1E_2\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
    &\quad + 2\left\|E_1E_2\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}E_1\right\| \\
    &\quad + 2\left\|E_1E_2\Sigma_{T,0:k}E_2\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
    &\quad + \left\|E_1E_2\Sigma_{T,0:k}E_2E_1\right\|. 
\end{align*}
In particular,
\begin{align*}
     &\quad \left\|E_1E_2\Sigma_{T,0:k}E_2E_1\right\|\\
     &= \left\|E_1 n\tilde{\Sigma}_{S,0:k} \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} E_2 \pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}} \pth{n\tilde{\Sigma}_{S,0:k}}^{\frac{1}{2}} \right. \\ &\left.\quad\cdot\Sigma_{T,0:k} E_2 \pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}} \pth{n\tilde{\Sigma}_{S,0:k}}^{\frac{1}{2}} E_1 n\tilde{\Sigma}_{S,0:k} \pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
     &\leq  \pth{\|E_1\| \left\|n\tilde{\Sigma}_{S,0:k}\right\|}^2 \pth{\|E_2\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}}\right\|} \\
     &\quad\cdot  \|E_2\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\|  \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\Sigma_{T,0:k}\right\| \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
     &\leq \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\|.
\end{align*}
The other terms can be similarly bounded. Therefore,
\begin{align*}
     &\quad \left\| \pth{X_{0:k}^TX_{0:k} +\lambda I_k + V^T(\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T)V }^{-1} \right.\\
    &\left.\quad\cdot  \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} \Sigma_{T,0:k} \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} \right. \\
    &\left.\quad\cdot  \pth{X_{0:k}^TX_{0:k} +\lambda I_k + V^T(\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T)V }^{-1} \right\| \\
    &\leq 16 \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
    &= \frac{16}{n} \left\| \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right\|.
\end{align*}

\end{proof}

\subsubsection{Bias in the Last \texorpdfstring{$d-k$}{d-k} Dimensions}
The upper bound for the bias in the last $d-k$ dimensions is extended from \cite{DBLP:journals/jmlr/TsiglerB23}'s Lemma~28. The bias can be decomposed into three terms.
\begin{align*}
    &\quad \pth{\hbeta(X\beta^\star)_{k:d}-\beta^\star_{k:d}}^T \Sigma_{T,k:d} \pth{\hbeta(X\beta^\star)_{k:d}-\beta^\star_{k:d}} \\
    &\leq 3 (\beta_{k:d}^\star)^T\Sigma_{T,k:d}\beta_{k:d}^\star \\
    &\quad + 3(\beta_{k:d}^\star)^TX_{k:d}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \Sigma_{T,k:d} X_{k:d}^T (XX^T+\lambda I_n)^{-1} X_{k:d}  \beta_{k:d}^\star \\
    &\quad + 3(\beta_{0:k}^\star)^TX_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \Sigma_{T,k:d} X_{k:d}^T (XX^T+\lambda I_n)^{-1} X_{0:k}  \beta_{0:k}^\star.
\end{align*}
\begin{lemma}
\label{lem:bias_kd_1}
    Under the same conditions as in Lemma~\ref{lem:all_concentration}, and on the same event, for any $N_1<n<N_2$,
    \begin{align*}
    	&\quad (\beta_{k:d}^\star)^TX_{k:d}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \Sigma_{T,k:d} X_{k:d}^T (XX^T+\lambda I_n)^{-1} X_{k:d}  \beta_{k:d}^\star \\
        &\leq c_x \pth{\lambda + \frac{1}{c_xL}\sum_j \lambda_j}^{-1} n \|\Sigma_{T,k:d}\| (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d}.
    \end{align*} 
    where $N_1,N_2$ are defined as in Lemma~\ref{lem:all_concentration}.
\end{lemma}
\begin{proof}
\begin{align*}
    &\quad (\beta_{k:d}^\star)^TX_{k:d}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \Sigma_{T,k:d} X_{k:d}^T (XX^T+\lambda I_n)^{-1} X_{k:d}  \beta_{k:d}^\star \\
    &\leq \| \Sigma_{T,k:d} \| (\beta_{k:d}^\star)^TX_{k:d}^T(XX^T+\lambda I_n)^{-1} X_{k:d}  X_{k:d}^T (XX^T+\lambda I_n)^{-1} X_{k:d}  \beta_{k:d}^\star \\
    &\leq \| \Sigma_{T,k:d} \| (\beta_{k:d}^\star)^TX_{k:d}^T(XX^T+\lambda I_n)^{-1}(XX^T+\lambda I_n) (XX^T+\lambda I_n)^{-1} X_{k:d}  \beta_{k:d}^\star \\
    &\leq \|\Sigma_{T,k:d}\| \left\| (XX^T+\lambda I_n)^{-1} \right\| (\beta_{k:d}^\star)^TX_{k:d}^TX_{k:d}  \beta_{k:d}^\star \\
    &\leq \|\Sigma_{T,k:d}\| \left\| (X_{k:d}X_{k:d}^T+\lambda I_n)^{-1} \right\| (\beta_{k:d}^\star)^TX_{k:d}^TX_{k:d}  \beta_{k:d}^\star \\
    &\leq \|\Sigma_{T,k:d}\| \pth{\lambda + \frac{1}{c_xL}\sum_j \lambda_j}^{-1} c_x n (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d}.
\end{align*}
The fourth inequality follows from $XX^T+\lambda I_n \succcurlyeq X_{k:d}X_{k:d}^T+\lambda I_n$.
\end{proof}

\begin{lemma}
\label{lem:bias_kd_2}
    Under the same conditions as in Lemma~\ref{lem:all_concentration}, and on the same event, for any $N_1<n<N_2$,
    \begin{align*}
        &\quad (\beta_{0:k}^\star)^TX_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \Sigma_{T,k:d} X_{k:d}^T (XX^T+\lambda I_n)^{-1} X_{0:k}  \beta_{0:k}^\star \\
    	&\leq \frac{c_x^3}{n} \frac{\pth{\lambda + c_x\sum_{j>k}\lambda_j}^2}{\lambda+c_x^{-1}L^{-1}\sum_{j>k}\lambda_j} \|\Sigma_{T,k:d}\|(\beta_{0:k}^\star)^T \Sigma_{S,0:k}^{-1}\beta_{0:k}^\star.
    \end{align*} 
    where $N_1,N_2$ are defined as in Lemma~\ref{lem:all_concentration}.
\end{lemma}
\begin{proof}
    It can be verified by Woodbury matrix identity that:
    \begin{align*}
        (XX^T+\lambda I_n)^{-1}X_{0:k} = (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k} \pth{I_k +X_{0:k}^T (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k} }^{-1}.
    \end{align*}
    Therefore,
    \begin{align*}
        &\quad (\beta_{0:k}^\star)^TX_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \Sigma_{T,k:d} X_{k:d}^T (XX^T+\lambda I_n)^{-1} X_{0:k}  \beta_{0:k}^\star \\
        &=  \left\| \Sigma_{T,k:d}^{\frac{1}{2}} X_{k:d}^T  (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k} \pth{I_k +X_{0:k}^T (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k} }^{-1} \beta_{0:k}^\star \right\|^2 \\
        &\leq \|\Sigma_{T,k:d}\| \left\| (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{k:d}X_{k:d}^T  (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1}  \right\| \\
        &\quad\cdot \left\|  X_{0:k} \pth{I_k +X_{0:k}^T (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k} }^{-1} \beta_{0:k}^\star  \right\|^2 \\
        &=  \|\Sigma_{T,k:d}\| \left\| (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{k:d}X_{k:d}^T  (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1}  \right\| \\
        &\quad\cdot \left\|  X_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}} \pth{\Sigma_{S,0:k}^{-1} +\Sigma_{S,0:k}^{-\frac{1}{2}}X_{0:k}^T (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k}\Sigma_{S,0:k}^{-\frac{1}{2}} }^{-1}\Sigma_{S,0:k}^{-\frac{1}{2}} \beta_{0:k}^\star  \right\|^2 \\
        &\leq  \|\Sigma_{T,k:d}\| \left\| (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1}  \right\| \left\| \Sigma_{S,0:k}^{-\frac{1}{2}}X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}} \right\| \\
        &\quad\cdot \left\| \pth{\Sigma_{S,0:k}^{-1} +\Sigma_{S,0:k}^{-\frac{1}{2}}X_{0:k}^T (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k}\Sigma_{S,0:k}^{-\frac{1}{2}} }^{-2} \right\| (\beta_{0:k}^\star)^T \Sigma_{S,0:k}^{-1}\beta_{0:k}^\star.
    \end{align*}
    In particular,
    \begin{align*}
        &\quad \left\| \pth{\Sigma_{S,0:k}^{-1} +\Sigma_{S,0:k}^{-\frac{1}{2}}X_{0:k}^T (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k}\Sigma_{S,0:k}^{-\frac{1}{2}} }^{-1} \right\| \\
        &\leq \left\| \pth{\Sigma_{S,0:k}^{-\frac{1}{2}}X_{0:k}^T (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k}\Sigma_{S,0:k}^{-\frac{1}{2}} }^{-1} \right\| \\
        &\leq \left\| X_{k:d}X_{k:d}^T + \lambda I_n \right\| \left\| \pth{\Sigma_{S,0:k}^{-\frac{1}{2}}X_{0:k}^TX_{0:k}\Sigma_{S,0:k}^{-\frac{1}{2}} }^{-1} \right\| \\
        &\leq \pth{\lambda + c_x\sum_{j>k}\lambda_j} \frac{c_x}{n}.
    \end{align*}
    The second inequality follows from $\mu_{\text{min}}(ABA^T) \geq \mu_{\text{min}}(B)\mu_{\text{min}}(AA^T)$ where the matrix $B$ is positive definite.
    
    Therefore,
    \begin{align*}
        &\quad (\beta_{0:k}^\star)^TX_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \Sigma_{T,k:d} X_{k:d}^T (XX^T+\lambda I_n)^{-1} X_{0:k}  \beta_{0:k}^\star \\
        &\leq \|\Sigma_{T,k:d}\| \left\| (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1}  \right\| \left\| \Sigma_{S,0:k}^{-\frac{1}{2}}X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}} \right\| \\
        &\quad\cdot \left\| \pth{\Sigma_{S,0:k}^{-1} +\Sigma_{S,0:k}^{-\frac{1}{2}}X_{0:k}^T (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k}\Sigma_{S,0:k}^{-\frac{1}{2}} }^{-2} \right\| (\beta_{0:k}^\star)^T \Sigma_{S,0:k}^{-1}\beta_{0:k}^\star \\
        &\leq  \|\Sigma_{T,k:d}\| \pth{\lambda+\frac{1}{c_xL}\sum_{j>k}\lambda_j}^{-1} c_xn \pth{\lambda + c_x\sum_{j>k}\lambda_j}^2 \frac{c_x^2}{n^2} (\beta_{0:k}^\star)^T \Sigma_{S,0:k}^{-1}\beta_{0:k}^\star \\
        &= \frac{c_x^3}{n} \frac{\pth{\lambda + c_x\sum_{j>k}\lambda_j}^2}{\lambda+c_x^{-1}L^{-1}\sum_{j>k}\lambda_j} \|\Sigma_{T,k:d}\|(\beta_{0:k}^\star)^T \Sigma_{S,0:k}^{-1}\beta_{0:k}^\star.
    \end{align*}
    
\end{proof}

\subsection{Main Results}
\begin{theorem}
Suppose the assumption condNum$(k,\delta,L)$~(Assumption~\ref{assum:condNum}) is satisfied. There exists a constant $c_x>2$ depending only on $\sigma_x$, such that for any $c_xN_1<n<N_2$, with probability at least $1-2\delta-c_xe^{-n/c_x}$,
\begin{align*}
    \frac{V}{c_x\sigma^2} &\leq  \frac{L^2}{n} \tr \qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}} + L^2n\big(\lambda+\sum_{j>k}\lambda_j\big)^{-2} \tr\qth{\Sigma_{S,k:d}^{\frac{1}{2}}\Sigma_{T,k:d} \Sigma_{S,k:d}^{\frac{1}{2}} }.  \\
    \frac{B}{c_x} &\leq (\beta^\star_{0:k})^T\Sigma_{S,0:k}^{-1} \beta^\star_{0:k} \Big[ \frac{1}{n^2} \big(\lambda+\sum_{j>k}\lambda_j\big)^2 \left\|\Sigma_{S,0:k}^{-\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}   \right\| + \frac{L}{n} \big(\lambda+\sum_{j>k}\lambda_j\big) \|\Sigma_{T,k:d}\| \Big] \\
    & + (\beta^\star_{k:d})^T\Sigma_{S,k:d}\beta^\star_{k:d} \Big[  L^2 \left\| \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}\right\| + Ln \big(\lambda+\sum_{j>k}\lambda_j\big)^{-1}\|\Sigma_{T,k:d} \| \Big] \\
    & +  (\beta^\star_{k:d})^T\Sigma_{T,k:d}\beta^\star_{k:d}.
\end{align*}
$N_1,N_2$ are defined as follows:
\begin{equation*}
    \begin{alignedat}{2}
    N_1 &= \max \Bigg\{ 
        & & \big( k + \ln \frac{1}{\delta} \big) \lambda_1^4 \lambda_k^{-4}, \\
        & && L \lambda_1 \lambda_k^{-2} \sum_{j>k} \lambda_j, \\
        & && \lambda_1 \lambda_k^{-2}\big(\lambda+\sum_{j>k}\lambda_k\big), \\
        & && \big( k + \ln \frac{1}{\delta} \big) \lambda_1^6 \lambda_k^{-8} \|\Sigma_{T,0:k}\|^2 k^2 
        \left( \tr \left[ \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} 
        \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right] \right)^{-2}, \\
        & && L \lambda_1^2 \lambda_k^{-4} \big( \sum_{j>k} \lambda_j \big) \|\Sigma_{T,0:k}\| k 
        \left( \tr \left[ \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} 
        \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right] \right)^{-1}
    \Bigg\}, \\
    N_2 &= \lambda_{k+1}^{-1} & & \sum_{j>k} \lambda_j.
    \end{alignedat}
    \end{equation*}
\end{theorem}
\begin{proof}
The theorem follows from Lemma~\ref{lem:all_concentration}, Lemma~\ref{lem:var_0k}, Lemma~\ref{lem:var_kd}, Lemma~\ref{lem:bias_0k_1}, Lemma~\ref{lem:bias_0k_2}, Lemma~\ref{lem:bias_kd_1} and Lemma~\ref{lem:bias_kd_2}. For a constant $c_x'>2$ depending only on $\sigma_x$, these lemmas hold for values of $n$ that satisfy the following inequalities:
\begin{align*}
    n &> 4c_x'^4(k+\ln(1/\delta))\lambda_1^2\lambda_k^{-2}, \\
    n &> 2c_x'^4L \lambda_k^{-1}\sum_{j>k}\lambda_j, \\
    n &> 4c_x'^4 \left( k + \ln \frac{1}{\delta} \right) \lambda_1^4 \lambda_k^{-4}, \\
    n &> 2c_x'^4 L \lambda_1 \lambda_k^{-2} \sum_{j>k} \lambda_j, \\
    n &> 4c_x'^4 \left( k + \ln \frac{1}{\delta} \right) \lambda_1^6 \lambda_k^{-8} \|\Sigma_{T,0:k}\|^2 k^2 
        \left( \tr \left[ \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} 
        \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right] \right)^{-2}, \\
    n &> 2c_x'^4 L \lambda_1^2 \lambda_k^{-4} \left( \sum_{j>k} \lambda_j \right) \|\Sigma_{T,0:k}\| k 
        \left( \tr \left[ \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} 
        \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right] \right)^{-1}, \\
    n &> c_x'^2 (\lambda + c_x \sum_{j>k} \lambda_j) \lambda_1 \lambda_k^{-2}, \\
    n &> 4c_x'^4\pth{k+\ln\frac{1}{\delta}}\lambda_1^6 \lambda_k^{-8}\|\Sigma_{T,0:k}\|^2 \left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}   \right\|^{-2}, \\
    n &> 2c_x'^4L \pth{\sum_{j>k} \lambda_j} \lambda_1^2\lambda_k^{-4} \|\Sigma_{T,0:k}\| \left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}   \right\|^{-1}, \\
    n &< \lambda_{k+1}^{-1} \sum_{j>k} \lambda_j.
\end{align*}
A sufficient condition for all the inequalities above is given by $4c_x'^4N_1<n<N_2$. This follows from the following facts:
\begin{align*}
    \lambda_1\lambda_k^{-1} &\geq 1, \\
    c_x' &> 2, \\
    k \left( \tr \left[ \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} 
        \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right] \right)^{-1} &\geq \left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}   \right\|^{-1}.    
\end{align*}
Then, with probability at least $1-2\delta-c_x'e^{-n/c_x'}$:
\begin{align*}
    V &\leq 16\sigma^2(1+c_x'^4L^2)\frac{1}{n} \tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}} \\
    &\quad + \sigma^2 c_x'n \pth{\lambda+\frac{1}{c_x'L} \sum_{j>k} \lambda_j}^{-2} \tr\qth{\Sigma_{S,k:d}^{\frac{1}{2}}\Sigma_{T,k:d} \Sigma_{S,k:d}^{\frac{1}{2}} } \\
    &\leq 32\sigma^2c_x'^4L^2\frac{1}{n} \tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}} \\
    &\quad + \sigma^2 c_x'^3L^2 n \pth{\lambda+\sum_{j>k}\lambda_j}^{-2} \tr\qth{\Sigma_{S,k:d}^{\frac{1}{2}}\Sigma_{T,k:d} \Sigma_{S,k:d}^{\frac{1}{2}} }, \\
    B &\leq \frac{8c_x'^2}{n^2} \pth{\lambda + c_x' \sum_{j>k} \lambda_j}^2 (\beta^\star_{0:k})^T \Sigma_{S,0:k}^{-1}   \beta^\star_{0:k} 
    \left\|\Sigma_{S,0:k}^{-\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}   \right\| \\
    &\quad + 32c_x'(1+c_x'^4L^2)  \left\| \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right\|  (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d} \\
    &\quad + 3c_x' \pth{\lambda + \frac{1}{c_x'L}\sum_j \lambda_j}^{-1} n \|\Sigma_{T,k:d}\| (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d} \\
    &\quad + 3\frac{c_x'^3}{n} \frac{\pth{\lambda + c_x'\sum_{j>k}\lambda_j}^2}{\lambda+c_x'^{-1}L^{-1}\sum_{j>k}\lambda_j} \|\Sigma_{T,k:d}\|(\beta_{0:k}^\star)^T \Sigma_{S,0:k}^{-1}\beta_{0:k}^\star \\
    &\quad + 3 (\beta_{k:d}^\star)^T\Sigma_{T,k:d}\beta_{k:d}^\star \\
    &\leq 8c_x'^4\frac{1}{n^2} \pth{\lambda + \sum_{j>k} \lambda_j}^2 \left\|\Sigma_{S,0:k}^{-\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}  \right\| 
    (\beta^\star_{0:k})^T \Sigma_{S,0:k}^{-1}   \beta^\star_{0:k} \\
    &\quad + 64c_x'^5L^2  \left\| \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right\|  (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d} \\ 
    &\quad + 3c_x'^2L n \pth{\lambda + \sum_j \lambda_j}^{-1}  \|\Sigma_{T,k:d}\| (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d} \\
    &\quad + 3c_x'^5L\frac{1}{n} \pth{\lambda + \sum_{j>k}\lambda_j} \|\Sigma_{T,k:d}\|(\beta_{0:k}^\star)^T \Sigma_{S,0:k}^{-1}\beta_{0:k}^\star \\
    &\quad + 3 (\beta_{k:d}^\star)^T\Sigma_{T,k:d}\beta_{k:d}^\star.
\end{align*}
By taking $c_x = 64c_x'^5$, the proof is complete.
\end{proof}


==> ridge_proof_deprecated_v2.tex <==
\section{Ridge Regression}
Let $X = (x_1, ..., x_n)^T \in \mathbb R^{n\times d}$, $Y = (y_1,...,y_n)^T \in \RR^d$ and $\boldsymbol{\epsilon}=(\epsilon_1,...,\epsilon_n)^T\in\RR^d$. We denote the first $k$ columns of $X$ as $X_{0:k}$ and the remaining $d-k$ columns as $X_{k:d}$. Similarly, $\beta^\star_{0:k}$ and $\beta^\star_{k:d}$ represent the corresponding components of $\beta^\star$. $\Sigma_{S,0:k}$, $\Sigma_{S,k:d}$ are the corresponding blocks on the diagonal of $\Sigma_S$. The $i$-th eigenvalue of a matrix is denoted by $\mu_i(\cdot)$. Define $Z = X\Sigma_S^{-1/2}$, where the rows of $Z$ are i.i.d. centered isotropic random vectors. Additionally, we assume the rows of $Z$ are $\sigma_x$-sub-gaussian, where the sub-gaussian norm is defined as follows. 

For a random variable $s$, the sub-gaussian norm $\|s\|_{\psi_2}$ is given by:
\begin{align*}
    \|s\|_{\psi_2} = \inf\left\{t>0: \EE\left[\exp \frac{s^2}{t^2} \right] \leq 2 \right\}.
\end{align*}

For a random vector $S$, the sub-gaussian norm $\|S\|_{\psi_2}$ is given by:
\begin{align*}
    \|S\|_{\psi_2} = \sup_{v\neq 0} \frac{\| \langle S, v \rangle \|_{\psi_2}}{\|v\|}.
\end{align*}

For $\lambda>0$, consider the ridge estimator:
\begin{align*}
    \hbeta(Y) &= X^T(XX^T+\lambda I_n)^{-1}Y \\
    &= X^T(XX^T+\lambda I_n)^{-1}X\beta^\star + X^T(XX^T+\lambda I_n)^{-1}\boldsymbol{\epsilon} \\
    &= \hbeta(X\beta^\star) + \hbeta(\boldsymbol{\epsilon}),
\end{align*}
where we define $\hbeta(X\beta^\star)=X^T(XX^T+\lambda I_n)^{-1}X\beta^\star$ and $\hbeta(\boldsymbol{\epsilon})=X^T(XX^T+\lambda I_n)^{-1}\boldsymbol{\epsilon}$. Additionally, we define $\tilde{\Sigma}_S = \Sigma_S + \frac{\lambda}{n}I_d$.
\begin{myassumption}[CondNum$(k,\delta,L)$]
\label{assum:condNum}
    Define a matrix $A_k = \lambda I_n + X_{k:d}X_{k:d}^T$. With probability at least $1-\delta$, $A_k$ is positive definite and has a condition number no greater than $L$, i.e.,
    \begin{align*}
        \frac{\mu_1(A_k)}{\mu_n(A_k)} \leq L.
    \end{align*}
\end{myassumption}

\subsection{Concentration Inequalities}
Denote the element of a matrix $X$ in the $i$-th row and the $j$-th column as $X[i,j]$, and the $i$-th row of the matrix $X$ as $X[i,*]$.

\begin{lemma}[Lemma~20 of \cite{DBLP:journals/jmlr/TsiglerB23}]
\label{lem:sigmaz}
Let $z$ be a sub-gaussian vector in $\mathbb{R}^p$ with $\|z\|_{\psi_2} \leq \sigma_x$, and consider $\Sigma = \operatorname{diag}(\lambda_1, \dots, \lambda_p)$ where the sequence $\{\lambda_j\}_{j=1}^p$ is positive and non-increasing. Then there exists some absolute constant $c$, for any $t > 0$, with probability at least $1-2e^{-t/c}$:
\begin{align*}
    \|\Sigma^{1/2} z\|^2 \leq c \sigma_x^2 \left( t \lambda_1 + \sum_{j=1}^p \lambda_j \right).
\end{align*}
\end{lemma}

\begin{lemma}[Lemma~23 of \cite{DBLP:journals/jmlr/TsiglerB23}]
\label{lem:ringAk}
Let \( \mathring{A}_k \) represent the matrix $X_{k:d}X_{k:d}^T$ with its diagonal elements set to zero: 
\begin{align*}
    \mathring{A}_k[i,j] = (1 - \delta_{i,j})(X_{k:d}X_{k:d}^T)[i,j].
\end{align*}
Then there exists some absolute constant \( c \), for any \( t > 0 \), with probability at least \( 1 - 4e^{-t/c} \):
\[
\|\mathring{A}_k\| \leq c\sigma_x^2 \sqrt{(t+n) \left( \lambda_{k+1}^2 (t+n) + \sum_{j > k} \lambda_j^2 \right)}.
\]
\end{lemma} 

\begin{lemma}[Lemma~21 of \cite{DBLP:journals/jmlr/TsiglerB23}] 
\label{lem:sum_sigmaz}
Suppose $\{z_i\}_{i=1}^n$ is a sequence of independent isotropic sub-gaussian random vectors, where \(\| z_i \|_{\psi_2} \leq \sigma\). Let \(\Sigma = \text{diag}(\lambda_1, \dots, \lambda_p)\) represent a diagonal matrix with a positive, non-increasing sequence \(\{ \lambda_i \}_{i=1}^p\). Then there exists some absolute constant \(c\), for any \(t \in (0, n)\), with probability at least \(1 - 2 e^{-ct}\):
\[
(n - \sqrt{nt} \sigma^2) \sum_{j=1}^p \lambda_j \leq \sum_{i=1}^n \|\Sigma^{1/2} z_i\|^2 
\leq (n + \sqrt{nt} \sigma^2) \sum_{j=1}^p \lambda_j.
\]
\end{lemma}

\begin{lemma}
\label{lem:xxT_concentration}
    Under the assumption CondNum$(k,\delta,L)$ (Assumption~\ref{assum:condNum}), there exists a constant $c_x$, depending only on $\sigma_x$, such that 
    for any $n<\lambda_{k+1}^{-1}
    \big(\lambda + \sum_{j>k}\lambda_j\big)$, % without this assumption, the upper bound will be n \lambda_{k+1} + \sum \lambda_j.
    with probability at least $1-\delta-c_xe^{-n/c_x}$:
    \begin{align*}
        \frac{1}{c_xL} \pth{\lambda+\sum_{j>k} \lambda_j} \leq \mu_n(A_k) \leq \mu_1(A_k) \leq c_x\pth{\lambda+\sum_{j>k} \lambda_j}.
    \end{align*}
\end{lemma}
\begin{proof}
This result follows from the proof of Lemma~3 in \cite{DBLP:journals/jmlr/TsiglerB23}, which establishes both upper and lower bounds of $\mu_1(A_k)$. By combining the lower bound with the assumption CondNum, we derive a lower bound of $\mu_n(A_k)$. For completeness, we restate the entire proof here.

According to lemma~\ref{lem:sigmaz} and lemma~\ref{lem:ringAk}, there exists an absolute constant c, such that for any $t>0$:
\begin{enumerate}
    \item for all $1\leq i \leq n$, with probability at least $1-2e^{-t/c}$:
    \begin{align*}
        \| X_{k:d}[i,*]\|^2 \leq c \sigma_x^2 \left( t \lambda_{k+1} + \sum_{j>k} \lambda_j \right).
    \end{align*}
    \item with probability at least $1-4e^{-t/c}$:
    \begin{align*}
        \|\mathring{A}_k\| \leq c\sigma_x^2 \sqrt{(t+n) \left( \lambda_{k+1}^2 (t+n) + \sum_{j > k} \lambda_j^2 \right)}.
    \end{align*}
\end{enumerate}
Since $\mu_1(A_k) \leq \lambda + \|\mathring{A}_k\| + \max_i \| X_{k:d}[i,*] \|^2$,
by setting $t=n$, we have with probability at least $1-(2n+4)e^{-n/c}$:
\begin{align}
    \mu_1(A_k) &\leq \lambda + c\sigma_x^2 \left( n\lambda_{k+1} + \sum_{j > k} \lambda_j + \sqrt{(2n \lambda_{k+1})^2 + 2n\sum_{j > k} \lambda_j^2 } 
     \right) \notag \\
     &\leq  \lambda + c\sigma_x^2 \left( n\lambda_{k+1} + \sum_{j > k} \lambda_j + 2n \lambda_{k+1} + \sqrt{2n\sum_{j > k} \lambda_j^2} \right) \notag \\
     &\leq \lambda +c\sigma_x^2 \left( n\lambda_{k+1} + \sum_{j > k} \lambda_j + 2n \lambda_{k+1} + \sqrt{2n\lambda_{k+1}\sum_{j > k} \lambda_j} \right)  \notag \\
     &\leq \lambda +c\sigma_x^2 \left( n\lambda_{k+1} + \sum_{j > k} \lambda_j + 2n \lambda_{k+1} + n\lambda_{k+1} + \frac{1}{2}\sum_{j > k} \lambda_j \right)  \notag \\
     &\leq \lambda + 4c\sigma_x^2 \left( n\lambda_{k+1} + \sum_{j > k} \lambda_j \right)  \notag \\
     &\leq \max\sth{1, 4c\sigma_x^2} \pth{\lambda + \sum_{j > k} \lambda_j + n\lambda_{k+1} }  \notag \\
     \label{eq:lem_xxT_concentration_1}
     &\leq 2\max\sth{1, 4c\sigma_x^2} \pth{\lambda + \sum_{j > k} \lambda_j }.
\end{align}
The last inequality follows from $n<\lambda_{k+1}^{-1}
    \big(\lambda + \sum_{j>k}\lambda_j\big)$.

On the other hand, by applying Lemma~\ref{lem:sum_sigmaz} with $t=\frac{n}{4\sigma_x^4}$, there exists an absolute constant $c'$, such that with probability at least $1 - 2 \exp\left\{-\frac{c'}{4\sigma_x^4}n \right\}$:
\begin{align*}
    \sum_{i=1}^n \|X_{k:d}[i,*]\|^2 \geq \frac{1}{2}n \sum_{j>k} \lambda_j.
\end{align*}
On this event,
\begin{align*}
    \mu_1(A_k) &\geq \lambda + \frac{1}{n} \operatorname{tr} (X_{k:d}X_{k:d}^T) \\
    &= \lambda + \frac{1}{n} \sum_{i=1}^n \|X_{k:d}[i,*]\|^2 \\
    &\geq \lambda + \frac{1}{2} \sum_{j>k} \lambda_j \\
    &\geq \frac{1}{2} \pth{\lambda + \sum_{j>k} \lambda_j}.
\end{align*}
By the assumption CondNum$(k,\delta,L)$, we have with probability at least $1-\delta-2 \exp\left\{-\frac{c'}{4\sigma_x^4}n \right\}$:
\begin{align}
\begin{split}
\label{eq:lem_xxT_concentration_2}
    \mu_n(A_k) \geq \frac{1}{L} \mu_1(A_k) \geq \frac{1}{2L} 
    \pth{\lambda + \sum_{j>k} \lambda_j}.
\end{split}
\end{align}
Combining Equation~\ref{eq:lem_xxT_concentration_1} and~\ref{eq:lem_xxT_concentration_2}, there exists a constant $c_x$ depending only on $\sigma_x$, such that with probability at least $1-\delta-c_x e^{-n/c_x}$:
\begin{align*}
    \frac{1}{c_xL} \pth{\lambda+\sum_{j>k} \lambda_j} \leq \mu_n(A_k) \leq \mu_1(A_k) \leq c_x\pth{\lambda+\sum_{j>k} \lambda_j}.
\end{align*}
\end{proof}

\begin{lemma}
\label{lem:xTx_concentration}
    There exists a constant $c_x$ depending only on $\sigma_x$, such that with probability at least $1-\delta$, if $n>k + \operatorname{ln}(1/\delta)$,
    \begin{align*}
        \left\| \frac{1}{n}X_{0:k}^TX_{0:k} - \Sigma_{S,0:k} \right\| \leq c_x \lambda_1 \sqrt{\frac{k+\operatorname{ln}\frac{1}{\delta}}{n}}.
    \end{align*}
\end{lemma}
\begin{proof}
    This follows directly from Theorem~5.39 and Remark~5.40 of \cite{DBLP:journals/corr/abs-1011-3027}, which shows there exists a constant $c_x'$ depending only on $\sigma_x$, such that for any $t\geq 0$, with probability at least $1-2\exp\{-t^2/c_x'\}$:
     \begin{align*}
          \left\| \frac{1}{n}X_{0:k}^TX_{0:k} - \Sigma_{S,0:k} \right\| \leq \lambda_1 \max \left\{ c_x'\sqrt{\frac{k}{n}} + \frac{t}{\sqrt n}, \left( c_x'\sqrt{\frac{k}{n}} + \frac{t}{\sqrt n} \right)^2 \right\}.
     \end{align*}
     Taking $t=\sqrt{c_x' \operatorname{ln}(2/\delta)}$ completes the proof.
\end{proof}

\begin{corollary}
\label{coroly:xTxroot_concentration}
    Under the same conditions as in Lemma~\ref{lem:xTx_concentration}, and on the same event, the following holds:
    \begin{align*}
        \left\| \left(X_{0:k}^TX_{0:k}\right)^{\frac{1}{2}} - \sqrt{n}\Sigma_{S,0:k}^{\frac{1}{2}} \right\| 
        \leq c_x \sqrt {k+\ln{\frac{1}{\delta}}}\lambda_1\lambda_k^{-\frac{1}{2}}.
    \end{align*}
\end{corollary}
\begin{proof}
    According to Proposition~3.2 of \cite{van1980inequality}, for any positive semi-definite matrix $A,B\in\RR^k$, we have 
    \begin{align*}
        \|A-B\| \geq \left(\mu_k\left(A^{\frac{1}{2}}\right)+\mu_k\left(B^{\frac{1}{2}}\right) \right)
        \left\|A^{\frac{1}{2}} - B^{\frac{1}{2}}\right\|.
    \end{align*}
    Therefore,
    \begin{align*}
        \left\| \left(X_{0:k}^TX_{0:k}\right)^{\frac{1}{2}} - \sqrt{n}\Sigma_{S,0:k}^{\frac{1}{2}} \right\| 
        &\leq \frac{1}{\mu_k\left(\sqrt{n}\Sigma_{S,0:k}^{\frac{1}{2}}\right)}  \left\| X_{0:k}^TX_{0:k} - n\Sigma_{S,0:k} \right\| \\
        &= \sqrt{n} \lambda_k^{-\frac{1}{2}} \left\| \frac{1}{n}X_{0:k}^TX_{0:k} - \Sigma_{S,0:k} \right\|. 
    \end{align*}
    By applying Lemma~\ref{lem:xTx_concentration}, the proof is complete.
\end{proof}

\begin{lemma}
\label{lem:sxTxs_concentration}
    There exists a constant $c_x$ depending only on $\sigma_x$, such that for any $n>c_xk$, with probability at least $1-2e^{-n/c_x}$:
    \begin{align*}
        \frac{1}{c_x}n \leq \mu_k\pth{\Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}}  \leq \mu_1\pth{\Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}}  \leq c_x n.
    \end{align*}
\end{lemma}
\begin{proof}
    According to Theorem~5.39 of \cite{DBLP:journals/corr/abs-1011-3027}, there exists a constant $c_x'$ depending only on $\sigma_x$, such that for any $t\geq 0$, with probability at least $1-2\exp\{ -t^2/c_x' \}$:
    \begin{align*}
        \mu_k\pth{\Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}}   
        &\geq \left( \sqrt{n} - c_x'\sqrt{k} - t  \right)^2.  \\ 
        \mu_1\pth{\Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}}  &\leq  \left( \sqrt{n} + c_x'\sqrt{k} + t  \right)^2 .
    \end{align*}
    Let $t=\frac{1}{2}\sqrt{n}$. For $n>16(c_x')^2 k$, with probability at least $1-2\exp \left\{ -n /(4c_x') \right\}$:
    \begin{align*}
        \mu_k\pth{\Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}}  
        &\geq \pth{ \sqrt{n} - \frac{1}{4}\sqrt{n} - \frac{1}{2}\sqrt{n}}^2 = \frac{1}{16}n. \\
        \mu_1\pth{\Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}}  
        &\leq \pth{ \sqrt{n} + \frac{1}{4}\sqrt{n} + \frac{1}{2}\sqrt{n}}^2 = \frac{49}{16}n.
    \end{align*}
    By taking $c_x = \max \sth{16(c_x')^2, 4c_x', 16}$, the proof is complete.
\end{proof}
\begin{remark}
On the same event, the following inequalities also hold:
\begin{align*}
    &\mu_1(X_{0:k}^TX_{0:k}) \leq \| \Sigma_{S,0:k} \| \left\| \Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}} \right\| \leq c_x\lambda_1n. \\
    &\mu_k(X_{0:k}^TX_{0:k}) \geq \mu_k(\Sigma_{S,0:k})  \mu_k\pth{\Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}} \geq \frac{1}{c_x}\lambda_kn.
\end{align*}
\end{remark}

\begin{lemma}
\label{lem:xsTxT_concentration}
    There exists a constant $c_x$ depending only on $\sigma_x$, with probability at least $1-2e^{-n/c_x}$:
    \begin{align*}
        \tr\pth{X_{k:d}\Sigma_{T,k:d}X_{k:d}^T} \leq c_x n\tr\pth{\Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d} \Sigma_{S,k:d}^{\frac{1}{2}} }.
    \end{align*}
\end{lemma}
\begin{proof}
According to Hanson-Wright Inequality~\citep{vershynin2018high}, there exists an absolute constant $c$, such that for any $1\leq i\leq n$,
\begin{align*}
    \left\| Z_{k:d}[i,*] \Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d}\Sigma_{S,k:d}^{\frac{1}{2}} Z_{k:d}[i,*]^T  \right\|_{\psi_1} 
    &\leq c \sigma_x^2 \left\| \Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d}\Sigma_{S,k:d}^{\frac{1}{2}} \right\|_F  \\
    &\leq c \sigma_x^2 \tr \pth{\Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d}\Sigma_{S,k:d}^{\frac{1}{2}}}.
\end{align*}
By Bernstein Inequality~(Proposition~5.16 of \cite{DBLP:journals/corr/abs-1011-3027}), there exists an absolute constant $c'$, for any $t\geq 0$,
\begin{align*}
    &\quad \PP \sth{\frac{1}{n} \left| \sum_{i=1}^n \qth {Z_{k:d}[i,*] \Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d}\Sigma_{S,k:d}^{\frac{1}{2}} Z_{k:d}[i,*]^T - \tr \pth{\Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d}\Sigma_{S,k:d}^{\frac{1}{2}}} } \right| 
     \geq t } \\
     &\leq 2 \exp \sth{-c'n \min \sth{ \frac{t^2}{K^2}, \frac{t}{K} }  },
\end{align*}
where $K=\max_i \left\| Z_{k:d}[i,*] \Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d}\Sigma_{S,k:d}^{\frac{1}{2}} Z_{k:d}[i,*]^T \right\|_{\psi_1}$.

Let $t=c\sigma_x^2 \tr \pth{\Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d}\Sigma_{S,k:d}^{\frac{1}{2}}}$. Then, with probability at least $1-2e^{-c'n}$:
\begin{align*}
    \tr\pth{X_{k:d}\Sigma_{T,k:d}X_{k:d}^T} &= \sum_{i=1}^n  Z_{k:d}[i,*] \Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d}\Sigma_{S,k:d}^{\frac{1}{2}} Z_{k:d}[i,*]^T  \\
    &\leq (1+c\sigma_x^2) n \tr \pth{\Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d}\Sigma_{S,k:d}^{\frac{1}{2}}}.
\end{align*}
By taking $c_x = \max\sth{ 1+c\sigma_x^2, \frac{1}{c'} }$, the proof is complete.
\end{proof}

\begin{lemma}
\label{lem:bxTxb_concentration}
    There exists a constant $c_x$ depending only on $\sigma_x$, with probablity at least $1-2e^{-n/c_x}$:
    \begin{align*}
        (\beta^\star_{k:d})^TX_{k:d}^TX_{k:d}\beta^\star_{k:d} \leq c_x n (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d}.
    \end{align*}
\end{lemma}
\begin{proof}
    The result follows from the proof of Lemma~3 in \cite{DBLP:journals/jmlr/TsiglerB23}, which we restate here for completeness. Consider the isotropic vector $ \qth{(\beta^\star_{k:d})^T\Sigma_{S,k:d}\beta^\star_{k:d}}^{-1/2}X_{k:d}\beta^\star_{k:d}$. For the $i$-th component,
    \begin{align*}
        \left\| \qth{(\beta^\star_{k:d})^T\Sigma_{S,k:d}\beta^\star_{k:d}}^{-\frac{1}{2}}X_{k:d}[i,*]\beta^\star_{k:d} \right\|_{\psi_2} 
        &=   \qth{(\beta^\star_{k:d})^T\Sigma_{S,k:d}\beta^\star_{k:d}}^{-\frac{1}{2}} \left\| Z_{k:d}[i,*]\Sigma_{S,k:d}^{\frac{1}{2}} \beta^\star_{k:d}\right\|_{\psi_2} \\
        &\leq \qth{(\beta^\star_{k:d})^T\Sigma_{S,k:d}\beta^\star_{k:d}}^{-\frac{1}{2}}
        \sigma_x \left\| \Sigma_{S,k:d}^{\frac{1}{2}} \beta^\star_{k:d} \right\| \\
        &=\sigma_x.
    \end{align*}
    By applying Lemma~\ref{lem:sum_sigmaz} for the sequence $\sth{\qth{(\beta^\star_{k:d})^T\Sigma_{S,k:d}\beta^\star_{k:d}}^{-1/2}X_{k:d}[i,*]\beta^\star_{k:d}}_{i=1}^n$, there exists an absolute constant $c$, for any $t\in(0,n)$, with probability at least $1-2e^{-ct}$:
    \begin{align*}
        \frac{(\beta^\star_{k:d})^TX_{k:d}^TX_{k:d}\beta^\star_{k:d}} {(\beta^\star_{k:d})^T\Sigma_{S,k:d}\beta^\star_{k:d}} &\leq n+\sqrt{nt}\sigma_x^2.
    \end{align*}
    Let $t=n/4$, with probability at least $1-2e^{-cn/4}$:
    \begin{align*}
        (\beta^\star_{k:d})^TX_{k:d}^TX_{k:d}\beta^\star_{k:d} \leq (1+\frac{1}{2}\sigma_x^2)n \cdot (\beta^\star_{k:d})^T\Sigma_{S,k:d}\beta^\star_{k:d}.
    \end{align*}
    By taking $c_x =\max \sth{ 1+\frac{1}{2}\sigma_x^2, \frac{4}{c} }$, the proof is complete.
\end{proof}

% % \subsection{Block Decomposition of $X_{k:d}X_{k:d}^T$}
\subsection{Block Decomposition of \texorpdfstring{$X_{k:d}X_{k:d}^T$}{X(k:d)X(k:d)T}}

Let $X_{0:k} = U\tilde{M}^{\frac{1}{2}}V$, where $U\in\RR^{n\times n}$ and $V\in\RR^{d\times d}$ are orthogonal matrices representing the left and right singular vectors, respectively. The matrix $\tilde{M}^{\frac{1}{2}}$ is defined as: 
\begin{align*}
    \tilde{M}^{\frac{1}{2}} = 
    \begin{pmatrix}
    m_1^{\frac{1}{2}} &  &  \\
     & \ddots &  \\
     &  & m_k^{\frac{1}{2}} \\
    \multicolumn{3}{c}{\mathbf{0}^{(n-k)\times k}} \\
    \end{pmatrix}
    \in \RR^{n\times k}.
\end{align*}
Therefore, we have $X_{0:k}X_{0:k}^T = UMU^T$, where $M=\operatorname{diag}(m_1,...,m_k,0,...,0) \in\RR^{n\times n}$. Similarly, $X_{0:k}^TX_{0:k}=V^T M_k V$, where $M_k = \operatorname{diag}(m_1,...,m_k) \in \RR^{k\times k}$. 

Let $\Delta = U^TX_{k:d}X_{k:d}^TU$, and write $\Delta$ in block matrix form as:
\begin{align*}
    \Delta = 
    \begin{pmatrix}
        \Delta_{11} & \Delta_{12} \\
        \Delta_{12}^T & \Delta_{22} \\
    \end{pmatrix},
\end{align*}
where $\Delta_{11} \in \RR^{k\times k}$, $\Delta_{12} \in \RR^{k\times (n-k)}$, and $\Delta_{22} \in \RR^{(n-k)\times (n-k)}$.

We will repeatedly use the first $k$ rows of $(M+\lambda I_n+\Delta)^{-1}$, which we compute here. Because $M+\lambda I_n+\Delta$ and $\lambda I_{n-k} + \Delta_{22}$ are invertible for $\lambda>0$, by block matrix inverse,
\begin{align}
\begin{split}
\label{eq:A_kinverse_firstkrows}
    &\quad (M+\lambda I_n+\Delta)^{-1}[0:k, *] \\
    &= \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1}
    \pth{I_k, - \Delta_{12}(\lambda I_{n-k} + \Delta_{22})^{-1} }.
\end{split}
\end{align}

\begin{corollary}[Corollary of Lemma~\ref{lem:xxT_concentration}]
\label{coroly:Delta}
    Suppose the assumption condNum$(k,\delta,L)$ is satisfied. There exists a constant depending only on $\sigma_x$, such that for any $n<\lambda_{k+1}^{-1}
    \big(\lambda+\sum_{j>k}\lambda_j\big)$, % without this assumption, the upper bound will be n \lambda_{k+1} + \sum \lambda_j.
    the following inequalities hold with probability at least $1-\delta-c_xe^{-n/c_x}$, on the same event as in Lemma~\ref{lem:xxT_concentration}.
    \begin{align*}
        &\| \Delta_{11} \|,\| \Delta_{12} \| \leq \|\Delta\| \leq c_x\pth{\lambda+\sum_{j>k} \lambda_j}. \\
        &\|(\lambda I_{n-k} + \Delta_{22})^{-1}\| \leq \|\Delta^{-1}\| \leq c_xL\pth{\lambda+\sum_{j>k}\lambda_j}^{-1}. \\
        &\left\| \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-2} \Delta_{12}^T \right\| \leq c_x^4 L^2. \\
        &\left\| \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T \right\| \leq c_x^3 L \pth{\lambda+\sum_{j>k} \lambda_j}. \\
        &\left\| \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T \right\| \leq c_x \pth{\lambda+\sum_{j>k} \lambda_j}.
    \end{align*}
\end{corollary}
\begin{proof}
\begin{enumerate}
    \item The first inequality.
    \begin{align*}
        \| \Delta_{11} \|,\| \Delta_{12} \| \leq \|\Delta\| = \| X_{k:d}X_{k:d}^T \| \leq \|A_k\| \leq c_x\pth{\lambda+\sum_{j>k} \lambda_j}.
    \end{align*}
    \item The second inequality.
    \begin{align*}
        \|(\lambda I_{n-k} + \Delta_{22})^{-1}\|  \leq \|(\lambda I_n + \Delta)^{-1}\| = \| A_k^{-1} \| \leq c_xL\pth{\lambda+\sum_{j>k}\lambda_j}^{-1},
    \end{align*}
    where the first inequality holds because $\lambda I_n + \Delta$ is positive definite.
    \item The third inequality.
    \begin{align*}
        \left\| \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-2} \Delta_{12}^T \right\| \leq \| \Delta_{12}\|^2 \|(\lambda I_{n-k} + \Delta_{22})^{-1}\|^2 \leq c_x^4 L^2.
    \end{align*}
    \item The fourth inequality.
    \begin{align*}
         \left\| \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T \right\| \leq \| \Delta_{12}\|^2 \|(\lambda I_{n-k} + \Delta_{22})^{-1}\| \leq c_x^3L \pth{
         \lambda+ \sum_{j>k}\lambda_j}.
    \end{align*}
    \item The last inequality.
    \begin{align*}
        &\quad \left\| \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T \right\| \\
        &= \left\| \Delta_{11} +\lambda I_k - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T \right\| -\lambda \\
        &\leq \|\Delta_{11} + \lambda I_k \| - \lambda \\
        &= \|\Delta_{11}\| \\
        &\leq c_x \pth{
         \lambda+ \sum_{j>k}\lambda_j}.
    \end{align*}
    The first inequality holds because $\Delta_{11} +\lambda I_k - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T$ is the Schur complement of the block $\Delta_{11} +\lambda I_k$ of the matrix $\Delta + \lambda I_n$, which is positive definite. Therefore, we have 
    \begin{align*}
        \Delta_{11} +\lambda I_k \succcurlyeq \Delta_{11} +\lambda I_k - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T.
    \end{align*}
\end{enumerate}
\end{proof}


\begin{lemma}
\label{lem:Akinverse_concentration}
Suppose the assumption condNum$(k,\delta,L)$ is satisfied. There exists a constant $c_x>2$ depending only on $\sigma_x$, such that for any $N_1<n<N_2$, with probability at least $1-2\delta-c_xe^{-n/c_x}$, on both events in Lemma~\ref{lem:xxT_concentration} and Lemma~\ref{lem:xTx_concentration},
\begin{align*}
    &\quad \left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} - \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} \right\| \\
    &\leq \frac{c_x^2\pth{\sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^2 L \pth{\lambda+\sum_{j>k}\lambda_j } }}{(\lambda+n\lambda_k)^2}.
\end{align*}
where 
\begin{align*}
    N_1 &= \max\sth{ 4c_x^4(k+\ln(1/\delta))\frac{\lambda_1^2}{\lambda_k^2}, 2c_x^4L \lambda_k^{-1}\pth{\lambda+\sum_{j>k}\lambda_j }}. \\
    N_2 &= \frac{1}{\lambda_{k+1}} \pth{\lambda+\sum_{j>k}\lambda_j}.
\end{align*}
\end{lemma}
\begin{proof}
\begin{align*}
    &\quad \left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} - \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} \right\| \\
    &\leq \left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1}\right\|  \\
    &\quad\cdot  \left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V} - \pth{n\tilde{\Sigma}_{S,0:k}} \right\| \\
    &\quad\cdot \left\| \pth{n\tilde{\Sigma}_{S,0:k}}^{-1}  \right\| \\
    &= \frac{1}{\lambda+n\lambda_k} \left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1}\right\| \\
    &\quad\cdot \left\| X_{0:k}^TX_{0:k} - n\Sigma_{S,0:k} + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V  \right\|.
\end{align*}
According to Lemma~\ref{lem:xTx_concentration}, Corollary~\ref{coroly:Delta}, there exists a constant $c_x>2$ depending only on $\sigma_x$, such that for any $k+\ln(1/\delta)<N_1<n<N_2=\lambda_{k+1}^{-1}
    \big(\lambda+\sum_{j>k}\lambda_j\big)$, with probability at least $1-2\delta-c_xe^{-n/c_x}$, on both events in Lemma~\ref{lem:xxT_concentration} and Lemma~\ref{lem:xTx_concentration},
\begin{align*}
    \left\| \frac{1}{n}X_{0:k}^TX_{0:k} - \Sigma_{S,0:k} \right\| &\leq c_x \lambda_1 \sqrt{\frac{k+\operatorname{ln}\frac{1}{\delta}}{n}}. \\
    \left\| \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T \right\| &\leq c_x^3 L \pth{\lambda+\sum_{j>k}\lambda_j}.
\end{align*}
\begin{enumerate}
\item $\left\| X_{0:k}^TX_{0:k} - n\Sigma_{S,0:k} + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V  \right\|$.
\begin{align*}
    &\quad\left\| X_{0:k}^TX_{0:k} - n\Sigma_{S,0:k} + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V  \right\| \\
    &\leq    \left\| X_{0:k}^TX_{0:k} - n\Sigma_{S,0:k}\right\| + \left\|\pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }  \right\| \\
    &\leq c_x \sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^3 L \pth{\lambda+\sum_{j>k}\lambda_j}.
\end{align*}
\item $\left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1}\right\|$
\begin{align*}
    &\quad\frac{1}{\lambda+n\lambda_k} \left\| X_{0:k}^TX_{0:k} - n\Sigma_{S,0:k} + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V  \right\| \\
    &\leq  \frac{1}{\lambda+n\lambda_k} \pth{c_x \sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^3 L \pth{\lambda+\sum_{j>k}\lambda_j} }.
\end{align*}
Since $n>4c_x^4(k+\ln(1/\delta))\frac{\lambda_1^2}{\lambda_k^2}$, 
\begin{align*}
    \frac{1}{\lambda+n\lambda_k} c_x \sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 &\leq \frac{ c_x \sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 }{n\lambda_k} \\
    &= \frac{ c_x \sqrt{(k+\ln\frac{1}{\delta})}\lambda_1 }{\sqrt{n}\lambda_k} \\
    &< \frac{1}{2c_x}.
\end{align*}
Since $n>2c_x^4L \lambda_k^{-1}\big(\lambda +\sum_{j>k}\lambda_j \big)$,
\begin{align*}
    \frac{1}{\lambda+n\lambda_k} c_x^3 L \pth{\lambda+\sum_{j>k}\lambda_j} &\leq \frac{c_x^3 L \pth{\lambda+\sum_{j>k}\lambda_j} } {n\lambda_k} \\
    &< \frac{1}{2c_x}.
\end{align*}
Therefore, we have
\begin{align*}
    \quad\frac{1}{\lambda+n\lambda_k} \left\| X_{0:k}^TX_{0:k} - n\Sigma_{S,0:k} + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V  \right\| < \frac{1}{c_x}.
\end{align*}
Now we derive the upper bound for our target.
\begin{align*}
    &\quad\left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1}\right\| \\
    &= \left\| \qth{n\tilde{\Sigma}_{S,0:k} + X_{0:k}^TX_{0:k} -n\Sigma_{S,0:k} + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1}\right\| \\
    &\leq \left\| \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} \right\| 
     \left[1 
     - \left\| \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} \right\| \right. \\
    &\left.\quad\cdot \left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1}\right\| \right]^{-1} \\
    &\leq \frac{1}{\lambda+n\lambda_k} \pth{1-\frac{1}{c_x}}^{-1} \\
    &\leq \frac{c_x}{\lambda+n\lambda_k}.
\end{align*}
The first inequality follows from the result $\|(A+T)^{-1}\| \leq \|A^{-1}\|\pth{1-\|A^{-1}\|\|T\|}^{-1}$, provided that both $A$ and $A+T$ are invertible and $\|A^{-1}\|\|T\|<1$~(see Lemma~3.1 in \cite{wedin1973perturbation}).
\end{enumerate}
Combining the above two inequalities, 
\begin{align*}
    &\quad \left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} - \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} \right\| \\
    &\leq \frac{1}{\lambda+n\lambda_k} \frac{c_x}{\lambda+n\lambda_k} \pth{c_x \sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^3 L \pth{\lambda+\sum_{j>k}\lambda_j}} \\
    &= \frac{c_x^2\pth{\sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^2 L \pth{\lambda+\sum_{j>k}\lambda_j}}}{(\lambda+n\lambda_k)^2}.
\end{align*}
\end{proof}

\subsection{Bias Variance Decomposition}
We consider the expection of the excess risk $\calR\pth{\hbeta(Y)}=\calR \pth{\hbeta(X\beta^\star) + \hbeta(\boldsymbol{\epsilon})}$ with respect to the distribution of the noise $\boldsymbol{\epsilon}$.
\begin{align*}
    \EE_{\boldsymbol{\epsilon}} \qth{\calR\pth{\hbeta(Y)}} &= \EE_{\boldsymbol{\epsilon}} \qth{\pth{\hbeta(Y)-\beta^\star}^T \Sigma_T \pth{\hbeta(Y)-\beta^\star}} \\
    &= \EE_{\boldsymbol{\epsilon}} \left[ 
    \pth{\hbeta(Y)_{0:k}-\beta^\star_{0:k}}^T \Sigma_{T,0:k} \pth{\hbeta(Y)_{0:k}-\beta^\star_{0:k}} \right. \\
    &\quad\left. + \pth{\hbeta(Y)_{k:d}-\beta^\star_{k:d}}^T \Sigma_{T,k:d} \pth{\hbeta(Y)_{k:d}-\beta^\star_{k:d}} \right. \\
    &\quad\left. + 2\pth{\hbeta(Y)_{0:k}-\beta^\star_{0:k}}^T \Sigma_{T}[0:k,k:d] \pth{\hbeta(Y)_{k:d}-\beta^\star_{k:d}} 
    \right] \\
    &\leq 2\EE_{\boldsymbol{\epsilon}} \qth{\pth{\hbeta(Y)_{0:k}-\beta^\star_{0:k}}^T \Sigma_{T,0:k} \pth{\hbeta(Y)_{0:k}-\beta^\star_{0:k}}} \\
    &\quad + 2\EE_{\boldsymbol{\epsilon}} \qth{\pth{\hbeta(Y)_{k:d}-\beta^\star_{k:d}}^T \Sigma_{T,k:d} \pth{\hbeta(Y)_{k:d}-\beta^\star_{k:d}}} \\
    &= 2\pth{\hbeta(X\beta^\star)_{0:k}-\beta^\star_{0:k}}^T \Sigma_{T,0:k} \pth{\hbeta(X\beta^\star)_{0:k}-\beta^\star_{0:k}} \\
    &\quad + 2\EE_{\boldsymbol{\epsilon}} \qth{\hbeta(\boldsymbol{\epsilon})_{0:k}^T \Sigma_{T,0:k} \hbeta(\boldsymbol{\epsilon})_{0:k}} \\
    &\quad + 2\pth{\hbeta(X\beta^\star)_{k:d}-\beta^\star_{k:d}}^T \Sigma_{T,k:d} \pth{\hbeta(X\beta^\star)_{k:d}-\beta^\star_{k:d}} \\
    &\quad + 2\EE_{\boldsymbol{\epsilon}} \qth{\hbeta(\boldsymbol{\epsilon})_{k:d}^T \Sigma_{T,k:d} \hbeta(\boldsymbol{\epsilon})_{k:d}}. 
\end{align*}
The first inequality follows from the result for a positive definite block quadratic form:
\begin{align*}
    (x_1^T, x_2^T)
    \begin{pmatrix}
        A & B \\
        B^T & D
    \end{pmatrix}
    \begin{pmatrix}
        x_1 \\
        x_2
    \end{pmatrix} = x_1^TAx_1 + 2x_1^TBx_2 + x_1^TDx_1,
\end{align*}
where the positive definiteness implies $x_1^TAx_1 + x_1^TDx_1 \geq 2x_1^TBx_2$.

We decompose the expected excess risk into variance and bias terms.
\begin{align*}
    V &= \EE_{\boldsymbol{\epsilon}} \qth{\hbeta(\boldsymbol{\epsilon})_{0:k}^T \Sigma_{T,0:k} \hbeta(\boldsymbol{\epsilon})_{0:k}}  + \EE_{\boldsymbol{\epsilon}} \qth{\hbeta(\boldsymbol{\epsilon})_{k:d}^T \Sigma_{T,k:d} \hbeta(\boldsymbol{\epsilon})_{k:d}}. \\
    B &= \pth{\hbeta(X\beta^\star)_{0:k}-\beta^\star_{0:k}}^T \Sigma_{T,0:k} \pth{\hbeta(X\beta^\star)_{0:k}-\beta^\star_{0:k}}  \\
    &\quad 
    + \pth{\hbeta(X\beta^\star)_{k:d}-\beta^\star_{k:d}}^T \Sigma_{T,k:d} \pth{\hbeta(X\beta^\star)_{k:d}-\beta^\star_{k:d}}.
\end{align*}

\begin{lemma}
\label{lem:all_concentration}
    Suppose the assumption condNum$(k,\delta,L)$~(Assumption~\ref{assum:condNum}) is satisfied. There exists a constant $c_x>2$ depending only on $\sigma_x$, such that for any $N_1<n<N_2$, with probability at least $1-2\delta-c_xe^{-n/c_x}$, the following inequalities hold at the same time:
\begin{align*}
    \mu_n(A_k) &\geq \frac{1}{c_xL} \pth{\lambda+\sum_{j>k}\lambda_j}. \\
     \mu_1(A_k) &\leq c_x \pth{\lambda+\sum_{j>k}\lambda_j}. \\
    \left\| \frac{1}{n}X_{0:k}^TX_{0:k} - \Sigma_{S,0:k} \right\| &\leq c_x \lambda_1 \sqrt{\frac{k+\operatorname{ln}\frac{1}{\delta}}{n}}. \\
    \left\| \left(X_{0:k}^TX_{0:k}\right)^{\frac{1}{2}} - \sqrt{n}\Sigma_{S,0:k}^{\frac{1}{2}} \right\| 
        &\leq c_x \sqrt {k+\ln{\frac{1}{\delta}}}\lambda_1\lambda_k^{-\frac{1}{2}}. \\
    \mu_k\pth{\Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}} &\geq \frac{1}{c_x}n.  \\
    \mu_1\pth{\Sigma_{S,0:k}^{-\frac{1}{2}} X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}}  &\leq c_x n. \\
    \mu_1(X_{0:k}^TX_{0:k})  &\leq c_x\lambda_1n. \\
    \mu_k(X_{0:k}^TX_{0:k})  &\geq \frac{1}{c_x}\lambda_kn.\\
    \tr\pth{X_{k:d}\Sigma_{T,k:d}X_{k:d}^T} &\leq c_x n\tr\pth{\Sigma_{S,k:d}^{\frac{1}{2}} \Sigma_{T,k:d} \Sigma_{S,k:d}^{\frac{1}{2}} }. \\
    (\beta^\star_{k:d})^TX_{k:d}^TX_{k:d}\beta^\star_{k:d} &\leq c_x n (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d}. \\
    \| \Delta_{11} \|,\| \Delta_{12}, \|\Delta\|  \| &\leq  c_x \pth{\lambda+\sum_{j>k}\lambda_j}. \\
    \|(\lambda I_{n-k} + \Delta_{22})^{-1}\|, \|\Delta^{-1}\| &\leq  c_xL\pth{\lambda+\sum_{j>k}\lambda_j}^{-1}. \\
    \left\| \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-2} \Delta_{12}^T \right\| &\leq c_x^4 L^2. \\
    \left\| \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T \right\| &\leq c_x^3 L \pth{\lambda+\sum_{j>k}\lambda_j}. \\
    \left\| \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T \right\| &\leq c_x \pth{\lambda+\sum_{j>k}\lambda_j}. 
\end{align*}
And, 
\begin{align*}
    &\quad\left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k}   + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} - \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} \right\| \\
    &\leq \frac{c_x^2\pth{\sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^2 L \pth{\lambda+\sum_{j>k}\lambda_j}}}{(\lambda+n\lambda_k)^2}.     
\end{align*}
$N_1$ and $N_2$ are defined as follows:
\begin{align*}
    N_1 &= \max\sth{ 4c_x^4(k+\ln(1/\delta))\frac{\lambda_1^2}{\lambda_k^2}, 2c_x^4L \lambda_k^{-1}\pth{\lambda+\sum_{j>k}\lambda_j} }. \\
    N_2 &= \frac{1}{\lambda_{k+1}} \pth{\lambda+\sum_{j>k}\lambda_j}.
\end{align*}
\end{lemma}
\begin{proof}
    The lemma is a direct corollary from Lemma~\ref{lem:xxT_concentration}, Lemma~\ref{lem:xTx_concentration}, Corollary~\ref{coroly:xTxroot_concentration}, Lemma~\ref{lem:sxTxs_concentration}, Lemma~\ref{lem:xsTxT_concentration}, Lemma~\ref{lem:bxTxb_concentration}, Corollary~\ref{coroly:Delta}, Lemma~\ref{lem:Akinverse_concentration}.
\end{proof}


\subsubsection{Variance in the First \texorpdfstring{$k$}{k} Dimensions}
\begin{lemma}
\label{lem:var_0k}
    Under the same conditions as in Lemma~\ref{lem:all_concentration}, and on the same event, for any $N_1<n<N_2$,
    \begin{align*}
    	\EE_{\boldsymbol{\epsilon}} \qth{\hbeta(\boldsymbol{\epsilon})_{0:k}^T \Sigma_{T,0:k} \hbeta(\boldsymbol{\epsilon})_{0:k}} \leq 16\sigma^2(1+c_x^4L^2)\frac{1}{n} \tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}},
    \end{align*} 
    where
    \begin{equation*}
    \begin{alignedat}{2}
    N_1 &= \max \Bigg\{ 
        & & 4c_x^4 \left( k + \ln \frac{1}{\delta} \right) \lambda_1^4 \lambda_k^{-4}, \\
        & && 2c_x^4 L \lambda_1 \lambda_k^{-2} \pth{\lambda+\sum_{j>k}\lambda_j}, \\
        & && 4c_x^4 \left( k + \ln \frac{1}{\delta} \right) \lambda_1^6 \lambda_k^{-8} \|\Sigma_{T,0:k}\|^2 k^2 
        \left( \tr \left[ \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} 
        \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right] \right)^{-2}, \\
        & && 2c_x^4 L \lambda_1^2 \lambda_k^{-4} \left( \lambda+\sum_{j>k} \lambda_j \right) \|\Sigma_{T,0:k}\| k 
        \left( \tr \left[ \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} 
        \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right] \right)^{-1}
    \Bigg\}, \\
    N_2 &= \frac{1}{\lambda_{k+1}} & & \pth{\lambda+\sum_{j>k}\lambda_j}.
    \end{alignedat}
    \end{equation*}
\end{lemma}
\begin{proof}
\begin{align*}
    &\quad \EE_{\boldsymbol{\epsilon}} \qth{\hbeta(\boldsymbol{\epsilon})_{0:k}^T \Sigma_{T,0:k} \hbeta(\boldsymbol{\epsilon})_{0:k}} \\
    &= \EE_{\boldsymbol{\epsilon}} \tr \qth{ \boldsymbol{\epsilon}\boldsymbol{\epsilon}^T (XX^T+\lambda I_n)^{-1} X_{0:k} \Sigma_{T,0:k} X_{0:k}^T (XX^T+\lambda I_n)^{-1}} \\
    &= \sigma^2 \tr \qth{(XX^T+\lambda I_n)^{-1} X_{0:k} \Sigma_{T,0:k} X_{0:k}^T (XX^T+\lambda I_n)^{-1}} \\
    &= \sigma^2 \tr \left[ (UMU^T+U\Delta U^T+\lambda I_n)^{-1} U \tilde{M}^{\frac{1}{2}} V \Sigma_{T,0:k} \right.\\
    &\left. \quad \cdot V^T \pth{\tilde{M}^{\frac{1}{2}}}^T U^T (UMU^T+U\Delta U^T+\lambda I_n)^{-1}  \right] \\
    &= \sigma^2 \tr \left[ U(M+\Delta +\lambda I_n)^{-1}  \tilde{M}^{\frac{1}{2}} V \Sigma_{T,0:k} 
    V^T \pth{\tilde{M}^{\frac{1}{2}}}^T  (M+\Delta +\lambda I_n)^{-1} U^T  \right] \\
    &= \sigma^2 \tr \qth{\pth{\tilde{M}^{\frac{1}{2}}}^T  (M+\Delta +\lambda I_n)^{-1} (M+\Delta +\lambda I_n)^{-1}  \tilde{M}^{\frac{1}{2}} V \Sigma_{T,0:k} 
    V^T   } \\
    &=  \sigma^2 \tr \left[M_k^{\frac{1}{2}} \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1}
    \pth{I_k, - \Delta_{12}(\lambda I_{n-k} + \Delta_{22})^{-1} } \right.\\
    &\left.\quad \cdot \pth{I_k, - \Delta_{12}(\lambda I_{n-k} + \Delta_{22})^{-1} }^T
    \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} M_k^{\frac{1}{2}} \right. \\
    &\left.\quad \cdot V\Sigma_{T,0:k}V^T \right]  \\
    &= \sigma^2 \tr \left[M_k^{\frac{1}{2}} \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right.\\
    &\left.\quad \cdot \pth{I_k + \Delta_{12}(\lambda I_{n-k} + \Delta_{22})^{-2}\Delta_{12}^T }  
    \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} M_k^{\frac{1}{2}} \right. \\
    &\left.\quad \cdot V\Sigma_{T,0:k}V^T \right]  \\
    &= \sigma^2 \tr \left[
     \pth{I_k + \Delta_{12}(\lambda I_{n-k} + \Delta_{22})^{-2}\Delta_{12}^T }  
    \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right. \\
    &\left.\quad \cdot M_k^{\frac{1}{2}} V\Sigma_{T,0:k}V^T M_k^{\frac{1}{2}} \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1}\right]  \\
    &\leq \sigma^2 \left\| I_k + \Delta_{12}(\lambda I_{n-k} + \Delta_{22})^{-2}\Delta_{12}^T  \right\|
    \tr \left[ \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right. \\
    &\left.\quad \cdot M_k^{\frac{1}{2}}  V\Sigma_{T,0:k}V^T M_k^{\frac{1}{2}} \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right] \\
    &\leq \sigma^2 (1+c_x^4L^2) \tr \left[ \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right. \\
    &\left.\quad \cdot M_k^{\frac{1}{2}}  V\Sigma_{T,0:k}V^T M_k^{\frac{1}{2}} \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right] \\
    &= \sigma^2 (1+c_x^4L^2) \tr \left[ \pth{V^T\pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} \right. \\
    &\left.\quad \cdot V^TM_k^{\frac{1}{2}}  V\cdot\Sigma_{T,0:k}\cdot V^T M_k^{\frac{1}{2}}V\cdot \pth{V^T\pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T}V}^{-1} \right] \\
    &= \sigma^2 (1+c_x^4L^2) \tr \left[ \pth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} \right. \\
    &\left.\quad \cdot \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} \right.\\
     &\left.\quad \cdot \pth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} \right].
\end{align*}
The sixth equation follows from Equation~\ref{eq:A_kinverse_firstkrows}. The first inequality follows from the result $\tr[AB] \leq \|A\|\tr[B]$ where the matrix $B$ is positive semi-definite.

We define two quantities that represent concentration error terms:
\begin{align*}
    E_1&=\left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} - \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} \right\|. \\
    E_2 &= \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} - \pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}.
\end{align*}
Since $n> 4c_x^4\pth{k+\ln\frac{1}{\delta}}\lambda_1^6 \lambda_k^{-8}\|\Sigma_{T,0:k}\|^2 k^2\pth{\tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}  } }^{-2}$,\\
and $n> 2c_x^4L \pth{\lambda+\sum_{j>k} \lambda_j} \lambda_1^2\lambda_k^{-4} \|\Sigma_{T,0:k}\| k\pth{\tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}  } }^{-1}$,
\begin{align*}
    &\quad\|E_1\| \left\|n\tilde{\Sigma}_{S,0:k}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\|  \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\Sigma_{T,0:k}\right\| \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
    &\leq \frac{c_x^2\pth{\sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^2 L \pth{\lambda+\sum_{j>k}\lambda_j}}}{(\lambda+n\lambda_k)^2} \pth{\lambda+n\lambda_1} \frac{n\lambda_1}{(\lambda+n\lambda_k)^2} \|\Sigma_{T,0:k} \| \\
    &\leq \frac{c_x^2\pth{\sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^2 L \pth{\lambda+\sum_{j>k}\lambda_j}}}{n^2}  \frac{\lambda_1^2}{\lambda_k^4} \|\Sigma_{T,0:k} \| \\
    &=  \frac{c_x^2\sqrt{(k+\ln\frac{1}{\delta})}}{n\sqrt{n}}  \frac{\lambda_1^3}{\lambda_k^4} \|\Sigma_{T,0:k}\|
     + \frac{c_x^4 L\pth{\lambda+\sum_{j>k}\lambda_j}}{n^2}  \frac{\lambda_1^2}{\lambda_k^4} \|\Sigma_{T,0:k}\| \\
    &< \frac{1}{2nk}\tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}} + \frac{1}{2nk}\tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}} \\
    &= \frac{1}{k}\tr \qth{\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}}.
\end{align*}
Since $n> 4c_x^4\pth{k+\ln\frac{1}{\delta}}\lambda_1^4 \lambda_k^{-4}$ and $n> 2c_x^4L \pth{\lambda+\sum_{j>k} \lambda_j} \lambda_1\lambda_k^{-2}$,
\begin{align}
\begin{split}
\label{eq:E1nS_leq1}
	 &\quad\|E_1\| \left\|n\tilde{\Sigma}_{S,0:k}\right\| \\
	 &\leq \frac{c_x^2\pth{\sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^2 L \pth{\lambda+\sum_{j>k}\lambda_j}}}{(\lambda+n\lambda_k)^2} \pth{\lambda+n\lambda_1} \\
	 &\leq \frac{c_x^2\pth{\sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^2 L \pth{\lambda+\sum_{j>k}\lambda_j}}}{n} \frac{\lambda_1}{\lambda_k^2} \\
	 &= \frac{c_x^2\sqrt{(k+\ln\frac{1}{\delta})}}{\sqrt{n}} \frac{\lambda_1^2}{\lambda_k^2} + \frac{c_x^4 L \pth{\lambda+\sum_{j>k}\lambda_j}}{n} \frac{\lambda_1}{\lambda_k^2} \\
	 &< \frac{1}{2} + \frac{1}{2} \\
	 &= 1.
\end{split}
\end{align}
Since $n> c_x^2\pth{k+\ln\frac{1}{\delta}}\lambda_1^4 \lambda_k^{-6}\|\Sigma_{T,0:k}\|^2 k^2\pth{\tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}  } }^{-2}$,
\begin{align*}
	&\quad\|E_2\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\|  \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\Sigma_{T,0:k}\right\| \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
	&\leq c_x \sqrt {k+\ln{\frac{1}{\delta}}}\lambda_1\lambda_k^{-\frac{1}{2}} \pth{n\lambda_k}^{-\frac{1}{2}} \frac{n\lambda_1}{(\lambda+n\lambda_k)^2} \|\Sigma_{T,0:k}\| \\
	&\leq \frac{c_x \sqrt {k+\ln{\frac{1}{\delta}}}}{n\sqrt{n}} \frac{\lambda_1^2}{\lambda_k^3} \|\Sigma_{T,0:k}\| \\
	&\leq \frac{1}{nk} \tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}} \\
	&= \frac{1}{k}\tr \qth{\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}}.
\end{align*}
Since $n> c_x^2\pth{k+\ln\frac{1}{\delta}}\lambda_1^2 \lambda_k^{-2}$,
\begin{align}
\begin{split}
\label{eq:E2nS_leq1}
    &\quad\|E_2\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}}\right\| \\
	&\leq c_x \sqrt {k+\ln{\frac{1}{\delta}}}\lambda_1\lambda_k^{-\frac{1}{2}} \pth{n\lambda_k}^{-\frac{1}{2}} \\
	&= \frac{c_x\sqrt {k+\ln{\frac{1}{\delta}}}}{\sqrt{n}}\frac{\lambda_1}{\lambda_k} \\
	&< 1.
\end{split}
\end{align}
Combing the above four inequalities, we have
\begin{align*}
    &\quad \tr \left[ \pth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} \right. \\
    &\left.\quad\quad \cdot \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} \right.\\
    &\left.\quad\quad \cdot \pth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} \right] \\
    &= \tr \qth{\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}} \\
    &\quad + 2\tr \qth{E_1\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}} \\
    &\quad + 2\tr \qth{\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}E_2\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}} \\
    &\quad +\tr \qth{E_1\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}E_1} \\
    &\quad + \tr \qth{\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}E_2\Sigma_{T,0:k}E_2\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}} \\
    &\quad + 2\tr \qth{E_1\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}E_2\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}} \\
    &\quad + 2\tr \qth{E_1E_2\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}} \\
    &\quad + 2\tr \qth{E_1E_2\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}E_1} \\
    &\quad + 2\tr \qth{E_1E_2\Sigma_{T,0:k}E_2\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}} \\
    &\quad + \tr \qth{E_1E_2\Sigma_{T,0:k}E_2E_1}. 
\end{align*}
In particular,
\begin{align*}
     &\quad \tr \qth{E_1E_2\Sigma_{T,0:k}E_2E_1} \\
     &= \tr \left[E_1 n\tilde{\Sigma}_{S,0:k} \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} E_2 \pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}} \pth{n\tilde{\Sigma}_{S,0:k}}^{\frac{1}{2}} \right. \\ &\left.\quad\cdot\Sigma_{T,0:k} E_2 \pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}} \pth{n\tilde{\Sigma}_{S,0:k}}^{\frac{1}{2}} E_1 n\tilde{\Sigma}_{S,0:k} \pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right] \\
     &\leq k \pth{\|E_1\| \left\|n\tilde{\Sigma}_{S,0:k}\right\|}^2 \pth{\|E_2\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}}\right\|} \\
     &\quad\cdot  \|E_2\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\|  \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\Sigma_{T,0:k}\right\| \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
     &\leq  \tr \qth{\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}}.
\end{align*}
The other terms can be similarly bounded. Therefore,
\begin{align*}
    &\quad \tr \left[ \pth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} \right. \\
    &\left.\quad\quad \cdot \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} \right.\\
    &\left.\quad\quad \cdot \pth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} \right] \\
    &\leq 16 \tr \qth{\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}} \\
    &= \frac{16}{n}  \tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}}.
\end{align*}
The proof is complete by combing all the inequalities above.
\end{proof}

\subsubsection{Variance in the Last \texorpdfstring{$d-k$}{d-k} Dimensions}
\begin{lemma}
\label{lem:var_kd}
    Under the same conditions as in Lemma~\ref{lem:all_concentration}, and on the same event, for any $N_1<n<N_2$,
    \begin{align*}
    	\EE_{\boldsymbol{\epsilon}} \qth{\hbeta(\boldsymbol{\epsilon})_{k:d}^T \Sigma_{T,k:d} \hbeta(\boldsymbol{\epsilon})_{k:d}}
     \leq \sigma^2 c_x^3L^2n \pth{\lambda+\sum_{j>k} \lambda_j}^{-2} \tr\qth{\Sigma_{S,k:d}^{\frac{1}{2}}\Sigma_{T,k:d} \Sigma_{S,k:d}^{\frac{1}{2}} } .
    \end{align*} 
    where $N_1,N_2$ are defined as in Lemma~\ref{lem:all_concentration}.
\end{lemma}
\begin{proof}
\begin{align*}
    &\quad \EE_{\boldsymbol{\epsilon}} \qth{\hbeta(\boldsymbol{\epsilon})_{k:d}^T \Sigma_{T,k:d} \hbeta(\boldsymbol{\epsilon})_{k:d}} \\
    &= \EE_{\boldsymbol{\epsilon}} \tr \qth{ \boldsymbol{\epsilon}\boldsymbol{\epsilon}^T (XX^T+\lambda I_n)^{-1} X_{k:d} \Sigma_{T,k:d} X_{k:d}^T (XX^T+\lambda I_n)^{-1}} \\
    &= \sigma^2 \tr \qth{(XX^T+\lambda I_n)^{-1} X_{k:d} \Sigma_{T,k:d} X_{k:d}^T (XX^T+\lambda I_n)^{-1}} \\
    &\leq \sigma^2 \left\| (XX^T+\lambda I_n)^{-2} \right\| \tr \qth{X_{k:d} \Sigma_{T,k:d} X_{k:d}^T} \\
    &\leq \sigma^2 \left\| (X_{k:d}X_{k:d}^T+\lambda I_n)^{-2} \right\| \tr \qth{X_{k:d} \Sigma_{T,k:d} X_{k:d}^T} \\
    &\leq \sigma^2  \pth{\frac{1}{c_xL} \pth{\lambda+\sum_{j>k} \lambda_j}}^{-2} 
    c_x n\tr\qth{\Sigma_{S,k:d}^{\frac{1}{2}}\Sigma_{T,k:d} \Sigma_{S,k:d}^{\frac{1}{2}} } \\
    &= \sigma^2 c_x^3L^2n \pth{\lambda+\sum_{j>k} \lambda_j}^{-2} \tr\qth{\Sigma_{S,k:d}^{\frac{1}{2}}\Sigma_{T,k:d} \Sigma_{S,k:d}^{\frac{1}{2}} }.
\end{align*}
The first inequality follows from the result $\tr [ABA] = \tr [A^2B] \leq \|A^2\| \tr [B]$ where the matrix $B$ is positive semi-definite. The second inequality follows from $XX^T+\lambda I_n \succcurlyeq X_{k:d}X_{k:d}^T+\lambda I_n$.
\end{proof}

\subsubsection{Bias in the First \texorpdfstring{$k$}{k} Dimensions}
The bias in the first $k$ dimensions can be decomposed into two terms.
\begin{align*}
    &\quad \pth{\hbeta(X\beta^\star)_{0:k}-\beta^\star_{0:k}}^T \Sigma_{T,0:k} \pth{\hbeta(X\beta^\star)_{0:k}-\beta^\star_{0:k}} \\
    &= \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X \beta^\star - \beta^\star_{0:k} }^T \Sigma_{T,0:k} \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X \beta^\star - \beta^\star_{0:k} } \\
    &\leq 2\pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \beta^\star_{0:k} - \beta^\star_{0:k} }^T \Sigma_{T,0:k} \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \beta^\star_{0:k} - \beta^\star_{0:k} }  \\
    &\quad + 2 \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \beta^\star_{k:d}}^T \Sigma_{T,0:k} \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \beta^\star_{k:d}}.
\end{align*}
The inequality follows from the result $x_1^TAx_1 + x_2^TAx_2 \geq 2x_1^TAx_2$ where $A$ is positive semi-definite.
\begin{lemma}
\label{lem:bias_0k_1}
    Under the same conditions as in Lemma~\ref{lem:all_concentration}, and on the same event, for any $N_1<n<N_2$,
    \begin{align*}
    &\quad \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \beta^\star_{0:k} - \beta^\star_{0:k} }^T \Sigma_{T,0:k} \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \beta^\star_{0:k} - \beta^\star_{0:k}} \\
    &\leq \frac{16c_x^4}{n^2} \pth{\lambda +  \sum_{j>k} \lambda_j}^2 (\beta^\star_{0:k})^T \Sigma_{S,0:k}^{-1}   \beta^\star_{0:k} 
    \left\|\Sigma_{S,0:k}^{-\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}   \right\|.
\end{align*}
    where
    \begin{equation*}
    \begin{alignedat}{2}
    N_1 &= \max \Bigg\{ 
        & & 2c_x^3 (\lambda +\sum_{j>k} \lambda_j) \lambda_1 \lambda_k^{-2}, \\
        &&& 4c_x^4(k+\ln(1/\delta))\lambda_1^2\lambda_k^{-2}, \\
        & && 2c_x^4L \lambda_k^{-1}\pth{\lambda+\sum_{j>k}\lambda_j} 
    \Bigg\}, \\
    N_2 &= \frac{1}{\lambda_{k+1}} & & \pth{\lambda+\sum_{j>k} \lambda_j}.
    \end{alignedat}
    \end{equation*}
\end{lemma}
\begin{proof}
\begin{align*}
     &\quad \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \beta^\star_{0:k} - \beta^\star_{0:k} }^T \Sigma_{T,0:k} \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \beta^\star_{0:k} - \beta^\star_{0:k}} \\
     &= (\beta^\star_{0:k})^T \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} - I_k}^T \Sigma_{T,0:k} \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} - I_k}\beta^\star_{0:k} \\
     &= (\beta^\star_{0:k})^T \Sigma_{S,0:k}^{-\frac{1}{2}} 
     \pth{\Sigma_{S,0:k}^{\frac{1}{2}} X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \Sigma_{S,0:k}^{\frac{1}{2}} - \Sigma_{S,0:k}}^T \Sigma_{S,0:k}^{-\frac{1}{2}}  \\
     &\quad \cdot \Sigma_{T,0:k} \Sigma_{S,0:k}^{-\frac{1}{2}} 
     \pth{\Sigma_{S,0:k}^{\frac{1}{2}} X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \Sigma_{S,0:k}^{\frac{1}{2}} - \Sigma_{S,0:k}}^T \Sigma_{S,0:k}^{-\frac{1}{2}} \beta^\star_{0:k} \\
     &\leq (\beta^\star_{0:k})^T \Sigma_{S,0:k}^{-1}   \beta^\star_{0:k} 
     \cdot \left\|\Sigma_{S,0:k}^{-\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}   \right\| \\
     &\quad \cdot \left\| \Sigma_{S,0:k}^{\frac{1}{2}} X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \Sigma_{S,0:k}^{\frac{1}{2}} - \Sigma_{S,0:k} \right\|^2.
\end{align*}
Subsequently,
\begin{align*}
    &\quad \left\| \Sigma_{S,0:k}^{\frac{1}{2}} X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \Sigma_{S,0:k}^{\frac{1}{2}} - \Sigma_{S,0:k} \right\| \\
    &= \left\| \Sigma_{S,0:k}^{\frac{1}{2}} 
    V^T \pth{\tilde{M}^{\frac{1}{2}}}^T U^T U (M+\lambda I_n + \Delta)^{-1} U^TU \tilde{M}^{\frac{1}{2}} V
    \Sigma_{S,0:k}^{\frac{1}{2}} - \Sigma_{S,0:k} \right\| \\
    &= \left\| \Sigma_{S,0:k}^{\frac{1}{2}} 
    V^T M_k^{\frac{1}{2}} \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} M_k^{\frac{1}{2}}  V
    \Sigma_{S,0:k}^{\frac{1}{2}} - \Sigma_{S,0:k} \right\| \\
    &= \left\| \Sigma_{S,0:k}^{\frac{1}{2}} 
    \pth{V^T M_k^{-\frac{1}{2}} \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V}^{-1}
    \Sigma_{S,0:k}^{\frac{1}{2}} \right. \\
    &\left.\quad - \Sigma_{S,0:k} \right\| \\
    &= \left\| \Sigma_{S,0:k}^{\frac{1}{2}} 
    \pth{I_k+ V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V}^{-1}
    \Sigma_{S,0:k}^{\frac{1}{2}} \right. \\
    &\left.\quad - \Sigma_{S,0:k} \right\| \\
    &= \left\| \Sigma_{S,0:k}^{\frac{1}{2}} 
    \left( \pth{I_k+ V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V}^{-1} - I_k \right) \right. \\
    &\left.\quad\cdot\Sigma_{S,0:k}^{\frac{1}{2}}  \right\| \\
    &= \left\| \Sigma_{S,0:k}^{\frac{1}{2}}  V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V \right. \\
    &\left.\quad\cdot \pth{I_k+ V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V}^{-1}  
    \Sigma_{S,0:k}^{\frac{1}{2}}  \right\| \\
    &\leq \left\| \Sigma_{S,0:k}^{\frac{1}{2}}  V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V   
    \Sigma_{S,0:k}^{\frac{1}{2}}  \right\| \\
    &\quad +\left\| \Sigma_{S,0:k}^{\frac{1}{2}}  V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V \right. \\
    &\left.\quad\cdot \qth{\pth{I_k+ V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V}^{-1}  -I_k}
    \Sigma_{S,0:k}^{\frac{1}{2}}  \right\|.
\end{align*}
The second equation follows from Equation~\ref{eq:A_kinverse_firstkrows}. 

We will derive upper bounds for both terms in the last equation above.
\begin{enumerate}
    \item The first term.
    \begin{align*}
        &\quad \left\| \Sigma_{S,0:k}^{\frac{1}{2}}  V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V   
    \Sigma_{S,0:k}^{\frac{1}{2}}  \right\| \\
    &\leq \left\| \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T  \right\| 
    \left\| \Sigma_{S,0:k}^{\frac{1}{2}}  V^T M_k^{-1} V  \Sigma_{S,0:k}^{\frac{1}{2}}  \right\| \\
    &= \left\| \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T  \right\| 
    \left\| \pth{\Sigma_{S,0:k}^{-\frac{1}{2}}  \pth{X_{0:k}^TX_{0:k}}^{-1}  \Sigma_{S,0:k}^{-\frac{1}{2}} }^{-1} \right\| \\
    &\leq \pth{\lambda +  c_x\pth{\lambda+\sum_{j>k} \lambda_j}} \frac{c_x}{n} \\
    &\leq \frac{2c_x^2}{n} \pth{\lambda +  \sum_{j>k} \lambda_j}.
    \end{align*}
    The inequality follows from $c_x>2$.
    \item The second term.

    Since $n>2c_x^3(\lambda +  \sum_{j>k} \lambda_j)\lambda_k^{-1}$,
    \begin{align*}
        &\quad \left\| M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}} \right\| \\
        &\leq \left\|M_k^{-1}\right\|  \left\| \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T  \right\| \\
        &\leq \frac{c_x}{n\lambda_k} \cdot 2c_x\pth{\lambda + \sum_{j>k} \lambda_j} \\
        &< \frac{1}{c_x}.
    \end{align*}
    Therefore,
    \begin{align*}
        &\quad \left\| \pth{I_k+ V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V}^{-1}  -I_k \right\| \\
        &\leq \left\| \pth{I_k+ V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V}^{-1} \right\|  \\
        &\quad\cdot \left\| V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V \right\| \\
        &\leq \pth{1-\frac{1}{c_x}}^{-1} \left\| V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V \right\| \\
        &\leq c_x \cdot \frac{c_x}{n\lambda_k} \cdot 2c_x\pth{\lambda + \sum_{j>k} \lambda_j} \\
        &= \frac{2c_x^3}{n} \frac{\lambda +\sum_{j>k} \lambda_j}{\lambda_k}.
    \end{align*}
     The second inequality follows from  $\|(A+T)^{-1}\| \leq \|A^{-1}\|\pth{1-\|A^{-1}\|\|T\|}^{-1}$, where both $A$ and $A+T$ are invertible and $\|A^{-1}\|\|T\|<1$. Note that $c_x>2$.

     Since $n>2c_x^3 (\lambda +\sum_{j>k} \lambda_j) \lambda_1 \lambda_k^{-2}$,
     \begin{align*}
         &\quad \left\| \Sigma_{S,0:k}^{\frac{1}{2}}  V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V \right. \\
        &\left.\quad\cdot \qth{\pth{I_k+ V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V}^{-1}  -I_k}
        \Sigma_{S,0:k}^{\frac{1}{2}}  \right\| \\
        &\leq \| \Sigma_{S,0:k}\| \left\| M_k^{-1} \right\| \left\| \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T \right\| \\
        &\quad \cdot \left\| \pth{I_k+ V^T M_k^{-\frac{1}{2}} \pth{\lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T } M_k^{-\frac{1}{2}}  V}^{-1}  -I_k \right\| \\
        &\leq \lambda_1\cdot \frac{c_x}{n\lambda_k} \cdot2c_x\pth{\lambda + \sum_{j>k} \lambda_j} \cdot \frac{2c_x^3}{n} \frac{\lambda + \sum_{j>k} \lambda_j}{\lambda_k} \\
        &= \frac{1}{n}\cdot\frac{4c_x^5}{n}\lambda_1\lambda_k^{-2} \pth{\lambda + \sum_{j>k} \lambda_j}^2 \\
        &< \frac{2c_x^2}{n} \pth{\lambda + \sum_{j>k} \lambda_j}.
     \end{align*}
\end{enumerate}
Combining both terms above, we have
\begin{align*}
    \left\| \Sigma_{S,0:k}^{\frac{1}{2}} X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \Sigma_{S,0:k}^{\frac{1}{2}} - \Sigma_{S,0:k} \right\|
    \leq \frac{4c_x^2}{n} \pth{\lambda +\sum_{j>k} \lambda_j}.
\end{align*}
Therefore, 
\begin{align*}
    &\quad \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \beta^\star_{0:k} - \beta^\star_{0:k} }^T \Sigma_{T,0:k} \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \beta^\star_{0:k} - \beta^\star_{0:k}} \\
    &\leq (\beta^\star_{0:k})^T \Sigma_{S,0:k}^{-1}   \beta^\star_{0:k} 
     \cdot \left\|\Sigma_{S,0:k}^{-\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}   \right\| \\
    &\quad \cdot \left\| \Sigma_{S,0:k}^{\frac{1}{2}} X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{0:k} \Sigma_{S,0:k}^{\frac{1}{2}} - \Sigma_{S,0:k} \right\|^2 \\
    &\leq \frac{16c_x^4}{n^2} \pth{\lambda +  \sum_{j>k} \lambda_j}^2 (\beta^\star_{0:k})^T \Sigma_{S,0:k}^{-1}   \beta^\star_{0:k} 
    \left\|\Sigma_{S,0:k}^{-\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}   \right\|.
\end{align*}
\end{proof}

\begin{lemma}
\label{lem:bias_0k_2}
    Under the same conditions as in Lemma~\ref{lem:all_concentration}, and on the same event, for any $N_1<n<N_2$,
    \begin{align*}
    &\quad \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \beta^\star_{k:d}}^T \Sigma_{T,0:k} \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \beta^\star_{k:d}} \\
    &\leq 16c_x(1+c_x^4L^2)  \left\| \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right\|  (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d}.
    \end{align*}
    where
    \begin{equation*}
    \begin{alignedat}{2}
    N_1 &= \max \Bigg\{ 
        & & 4c_x^4 \left( k + \ln \frac{1}{\delta} \right) \lambda_1^4 \lambda_k^{-4}, \\
        & && 2c_x^4 L \lambda_1 \lambda_k^{-2} \pth{\lambda+\sum_{j>k} \lambda_j}, \\
        & &&  4c_x^4\pth{k+\ln\frac{1}{\delta}}\lambda_1^6 \lambda_k^{-8}\|\Sigma_{T,0:k}\|^2 \left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}   \right\|^{-2}, \\
        & && 2c_x^4L \pth{\lambda+\sum_{j>k} \lambda_j} \lambda_1^2\lambda_k^{-4} \|\Sigma_{T,0:k}\| \left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}   \right\|^{-1}
    \Bigg\}, \\
    N_2 &= \frac{1}{\lambda_{k+1}} & & \pth{\lambda+\sum_{j>k} \lambda_j}.
    \end{alignedat}
    \end{equation*}
\end{lemma}
\begin{proof}
\begin{align*}
    &\quad \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \beta^\star_{k:d}}^T \Sigma_{T,0:k} \pth{ X_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \beta^\star_{k:d}}   \\
    &\leq \left\| (XX^T+\lambda I_n)^{-1} X_{0:k}\Sigma_{T,0:k}X_{0:k}^T (XX^T+\lambda I_n)^{-1} \right\| \cdot (\beta^\star_{k:d})^T X_{k:d}^TX_{k:d}\beta^\star_{k:d}.
\end{align*}
From Lemma~\ref{lem:all_concentration}, 
\begin{align*}
     (\beta^\star_{k:d})^T X_{k:d}^TX_{k:d}\beta^\star_{k:d} \leq c_x n (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d}.
\end{align*}
In the following, we derive an upper bound for the other term.
\begin{align*}
    &\quad \left\| (XX^T+\lambda I_n)^{-1} X_{0:k}\Sigma_{T,0:k}X_{0:k}^T (XX^T+\lambda I_n)^{-1} \right\| \\
    &= \left\| (M+\lambda I_n + \Delta)^{-1} \tilde{M}^{\frac{1}{2}} V \Sigma_{T,0:k} V^T \pth{\tilde{M}^{\frac{1}{2}}}^T  (M+\lambda I_n + \Delta)^{-1} \right\| \\
    &= \left\| \Sigma_{T,0:k}^{\frac{1}{2}} V^T \pth{\tilde{M}^{\frac{1}{2}}}^T  (M+\lambda I_n + \Delta)^{-2} \tilde{M}^{\frac{1}{2}} V \Sigma_{T,0:k}^{\frac{1}{2}} \right\| \\
    &= \left\| \Sigma_{T,0:k}^{\frac{1}{2}} V^T M_{k}^{\frac{1}{2}} \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right. \\
    &\left.\quad \cdot \pth{I_k + \Delta_{12}(\lambda I_{n-k} + \Delta_{22})^{-2}\Delta_{12}^T}
    \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right. \\
    &\left. \quad \cdot M_{k}^{\frac{1}{2}} V  \Sigma_{T,0:k}^{\frac{1}{2}}  \right\| \\
    &\leq \left\| I_k + \Delta_{12}(\lambda I_{n-k} + \Delta_{22})^{-2}\Delta_{12}^T \right\| \\
    &\quad \cdot \left\| \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1}  M_{k}^{\frac{1}{2}} V  \Sigma_{T,0:k} \right. \\
    &\left.\quad\cdot V^TM_{k}^{\frac{1}{2}}\pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right\| \\
    &\leq (1+c_x^4L^2)  \left\| \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1}  M_{k}^{\frac{1}{2}} V  \Sigma_{T,0:k} \right. \\
    &\left.\quad\cdot V^TM_{k}^{\frac{1}{2}}\pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }^{-1} \right\| \\
    &= (1+c_x^4L^2) \left\| \pth{V^T \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }  V}^{-1} \right.\\
    &\left.\quad\cdot V^TM_{k}^{\frac{1}{2}} V \Sigma_{T,0:k}  V^TM_{k}^{\frac{1}{2}} V \right.\\
    &\left.\quad\cdot \pth{V^T \pth{M_k + \lambda I_k + \Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }  V}^{-1} \right\| \\
    &= (1+c_x^4L^2) \left\| \pth{X_{0:k}^TX_{0:k} +\lambda I_k + V^T(\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T)V }^{-1} \right.\\
    &\left.\quad\cdot  \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} \Sigma_{T,0:k} \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} \right. \\
    &\left.\quad\cdot  \pth{X_{0:k}^TX_{0:k} +\lambda I_k + V^T(\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T)V }^{-1} \right\|.
\end{align*}
The third equation follows from Equation~\ref{eq:A_kinverse_firstkrows}.

We define two quantities that represent concentration error terms:
\begin{align*}
    E_1&=\left\| \qth{X_{0:k}^TX_{0:k} + \lambda I_k + V^T \pth{\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T }V}^{-1} - \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} \right\|. \\
    E_2 &= \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} - \pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}.
\end{align*}
Since $n> 4c_x^4\pth{k+\ln\frac{1}{\delta}}\lambda_1^6 \lambda_k^{-8}\|\Sigma_{T,0:k}\|^2 \left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}   \right\|^{-2}$,\\
and $n> 2c_x^4L \pth{\lambda+\sum_{j>k} \lambda_j} \lambda_1^2\lambda_k^{-4} \|\Sigma_{T,0:k}\| \left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}   \right\|^{-1}$,
\begin{align*}
    &\quad\|E_1\| \left\|n\tilde{\Sigma}_{S,0:k}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\|  \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\Sigma_{T,0:k}\right\| \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
    &\leq \frac{c_x^2\pth{\sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^2 L \pth{\lambda+\sum_{j>k}\lambda_j}}}{(\lambda+n\lambda_k)^2} \pth{\lambda+n\lambda_1} \frac{n\lambda_1}{(\lambda+n\lambda_k)^2} \|\Sigma_{T,0:k} \| \\
    &\leq \frac{c_x^2\pth{\sqrt{n(k+\ln\frac{1}{\delta})}\lambda_1 + c_x^2 L \pth{\lambda+\sum_{j>k}\lambda_j}}}{n^2}  \frac{\lambda_1^2}{\lambda_k^4} \|\Sigma_{T,0:k} \| \\
    &=  \frac{c_x^2\sqrt{(k+\ln\frac{1}{\delta})}}{n\sqrt{n}}  \frac{\lambda_1^3}{\lambda_k^4} \|\Sigma_{T,0:k}\|
     + \frac{c_x^4 L \pth{\lambda+\sum_{j>k}\lambda_j}}{n^2}  \frac{\lambda_1^2}{\lambda_k^4} \|\Sigma_{T,0:k}\| \\
    &< \frac{1}{2n}\left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}\right\| + \frac{1}{2n}\left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}\right\| \\
    &= \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\|.
\end{align*}
Similar to Equation~\ref{eq:E1nS_leq1}, since $n> 4c_x^4\pth{k+\ln\frac{1}{\delta}}\lambda_1^4 \lambda_k^{-4}$ and $n> 2c_x^4L \pth{\lambda+\sum_{j>k} \lambda_j} \lambda_1\lambda_k^{-2}$,
\begin{align*}
    \|E_1\| \left\|n\tilde{\Sigma}_{S,0:k}\right\| < 1.
\end{align*}
Since $n> c_x^2\pth{k+\ln\frac{1}{\delta}}\lambda_1^4 \lambda_k^{-6}\|\Sigma_{T,0:k}\|^2 \left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}   \right\|^{-2}$,
\begin{align*}
	&\quad\|E_2\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\|  \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\Sigma_{T,0:k}\right\| \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
	&\leq c_x \sqrt {k+\ln{\frac{1}{\delta}}}\lambda_1\lambda_k^{-\frac{1}{2}} \pth{n\lambda_k}^{-\frac{1}{2}} \frac{n\lambda_1}{(\lambda+n\lambda_k)^2} \|\Sigma_{T,0:k}\| \\
	&\leq \frac{c_x \sqrt {k+\ln{\frac{1}{\delta}}}}{n\sqrt{n}} \frac{\lambda_1^2}{\lambda_k^3} \|\Sigma_{T,0:k}\| \\
	&\leq \frac{1}{n}\left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}\right\| \\
	&=\left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\|.
\end{align*}
Similar to Equation~\ref{eq:E2nS_leq1}, since $n> c_x^2\pth{k+\ln\frac{1}{\delta}}\lambda_1^2 \lambda_k^{-2}$,
\begin{align*}
    \|E_2\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}}\right\| < 1.
\end{align*}
Combining the four inequalities above,
\begin{align*}
    &\quad \left\| \pth{X_{0:k}^TX_{0:k} +\lambda I_k + V^T(\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T)V }^{-1} \right.\\
    &\left.\quad\cdot  \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} \Sigma_{T,0:k} \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} \right. \\
    &\left.\quad\cdot  \pth{X_{0:k}^TX_{0:k} +\lambda I_k + V^T(\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T)V }^{-1} \right\| \\
    &\leq \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1} \right\| \\
    &\quad + 2\left\|E_1\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
    &\quad + 2\left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}E_2\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
    &\quad +\left\|E_1\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}E_1\right\| \\
    &\quad + \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}E_2\Sigma_{T,0:k}E_2\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
    &\quad + 2\left\|E_1\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}E_2\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
    &\quad + 2\left\|E_1E_2\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
    &\quad + 2\left\|E_1E_2\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}E_1\right\| \\
    &\quad + 2\left\|E_1E_2\Sigma_{T,0:k}E_2\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
    &\quad + \left\|E_1E_2\Sigma_{T,0:k}E_2E_1\right\|. 
\end{align*}
In particular,
\begin{align*}
     &\quad \left\|E_1E_2\Sigma_{T,0:k}E_2E_1\right\|\\
     &= \left\|E_1 n\tilde{\Sigma}_{S,0:k} \pth{n\tilde{\Sigma}_{S,0:k}}^{-1} E_2 \pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}} \pth{n\tilde{\Sigma}_{S,0:k}}^{\frac{1}{2}} \right. \\ &\left.\quad\cdot\Sigma_{T,0:k} E_2 \pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}} \pth{n\tilde{\Sigma}_{S,0:k}}^{\frac{1}{2}} E_1 n\tilde{\Sigma}_{S,0:k} \pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
     &\leq  \pth{\|E_1\| \left\|n\tilde{\Sigma}_{S,0:k}\right\|}^2 \pth{\|E_2\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}}\right\|} \\
     &\quad\cdot  \|E_2\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\|  \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\Sigma_{T,0:k}\right\| \left\|\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\right\| \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
     &\leq \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\|.
\end{align*}
The other terms can be similarly bounded. Therefore,
\begin{align*}
     &\quad \left\| \pth{X_{0:k}^TX_{0:k} +\lambda I_k + V^T(\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T)V }^{-1} \right.\\
    &\left.\quad\cdot  \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} \Sigma_{T,0:k} \pth{X_{0:k}^TX_{0:k}}^{\frac{1}{2}} \right. \\
    &\left.\quad\cdot  \pth{X_{0:k}^TX_{0:k} +\lambda I_k + V^T(\Delta_{11} - \Delta_{12} (\lambda I_{n-k} + \Delta_{22})^{-1} \Delta_{12}^T)V }^{-1} \right\| \\
    &\leq 16 \left\|\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\Sigma_{T,0:k}\pth{n\Sigma_{S,0:k}}^{\frac{1}{2}}\pth{n\tilde{\Sigma}_{S,0:k}}^{-1}\right\| \\
    &= \frac{16}{n} \left\| \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right\|.
\end{align*}

\end{proof}

\subsubsection{Bias in the Last \texorpdfstring{$d-k$}{d-k} Dimensions}
The upper bound for the bias in the last $d-k$ dimensions is extended from \cite{DBLP:journals/jmlr/TsiglerB23}'s Lemma~28. The bias can be decomposed into three terms.
\begin{align*}
    &\quad \pth{\hbeta(X\beta^\star)_{k:d}-\beta^\star_{k:d}}^T \Sigma_{T,k:d} \pth{\hbeta(X\beta^\star)_{k:d}-\beta^\star_{k:d}} \\
    &\leq 3 (\beta_{k:d}^\star)^T\Sigma_{T,k:d}\beta_{k:d}^\star \\
    &\quad + 3(\beta_{k:d}^\star)^TX_{k:d}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \Sigma_{T,k:d} X_{k:d}^T (XX^T+\lambda I_n)^{-1} X_{k:d}  \beta_{k:d}^\star \\
    &\quad + 3(\beta_{0:k}^\star)^TX_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \Sigma_{T,k:d} X_{k:d}^T (XX^T+\lambda I_n)^{-1} X_{0:k}  \beta_{0:k}^\star.
\end{align*}
\begin{lemma}
\label{lem:bias_kd_1}
    Under the same conditions as in Lemma~\ref{lem:all_concentration}, and on the same event, for any $N_1<n<N_2$,
    \begin{align*}
    	&\quad (\beta_{k:d}^\star)^TX_{k:d}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \Sigma_{T,k:d} X_{k:d}^T (XX^T+\lambda I_n)^{-1} X_{k:d}  \beta_{k:d}^\star \\
        &\leq c_x^2L \pth{\lambda + \sum_j \lambda_j}^{-1} n \|\Sigma_{T,k:d}\| (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d}.
    \end{align*} 
    where $N_1,N_2$ are defined as in Lemma~\ref{lem:all_concentration}.
\end{lemma}
\begin{proof}
\begin{align*}
    &\quad (\beta_{k:d}^\star)^TX_{k:d}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \Sigma_{T,k:d} X_{k:d}^T (XX^T+\lambda I_n)^{-1} X_{k:d}  \beta_{k:d}^\star \\
    &\leq \| \Sigma_{T,k:d} \| (\beta_{k:d}^\star)^TX_{k:d}^T(XX^T+\lambda I_n)^{-1} X_{k:d}  X_{k:d}^T (XX^T+\lambda I_n)^{-1} X_{k:d}  \beta_{k:d}^\star \\
    &\leq \| \Sigma_{T,k:d} \| (\beta_{k:d}^\star)^TX_{k:d}^T(XX^T+\lambda I_n)^{-1}(XX^T+\lambda I_n) (XX^T+\lambda I_n)^{-1} X_{k:d}  \beta_{k:d}^\star \\
    &\leq \|\Sigma_{T,k:d}\| \left\| (XX^T+\lambda I_n)^{-1} \right\| (\beta_{k:d}^\star)^TX_{k:d}^TX_{k:d}  \beta_{k:d}^\star \\
    &\leq \|\Sigma_{T,k:d}\| \left\| (X_{k:d}X_{k:d}^T+\lambda I_n)^{-1} \right\| (\beta_{k:d}^\star)^TX_{k:d}^TX_{k:d}  \beta_{k:d}^\star \\
    &\leq \|\Sigma_{T,k:d}\| \pth{\frac{1}{c_xL}\pth{\lambda+\sum_j \lambda_j}}^{-1} c_x n (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d} \\
    &= c_x^2L \pth{\lambda + \sum_j \lambda_j}^{-1} n \|\Sigma_{T,k:d}\| (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d}.
\end{align*}
The fourth inequality follows from $XX^T+\lambda I_n \succcurlyeq X_{k:d}X_{k:d}^T+\lambda I_n$.
\end{proof}

\begin{lemma}
\label{lem:bias_kd_2}
    Under the same conditions as in Lemma~\ref{lem:all_concentration}, and on the same event, for any $N_1<n<N_2$,
    \begin{align*}
        &\quad (\beta_{0:k}^\star)^TX_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \Sigma_{T,k:d} X_{k:d}^T (XX^T+\lambda I_n)^{-1} X_{0:k}  \beta_{0:k}^\star \\
    	&\leq \frac{c_x^6}{n} L \pth{\lambda+\sum_{j>k}\lambda_j} \|\Sigma_{T,k:d}\|(\beta_{0:k}^\star)^T \Sigma_{S,0:k}^{-1}\beta_{0:k}^\star.
    \end{align*} 
    where $N_1,N_2$ are defined as in Lemma~\ref{lem:all_concentration}.
\end{lemma}
\begin{proof}
    It can be verified by Woodbury matrix identity that:
    \begin{align*}
        (XX^T+\lambda I_n)^{-1}X_{0:k} = (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k} \pth{I_k +X_{0:k}^T (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k} }^{-1}.
    \end{align*}
    Therefore,
    \begin{align*}
        &\quad (\beta_{0:k}^\star)^TX_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \Sigma_{T,k:d} X_{k:d}^T (XX^T+\lambda I_n)^{-1} X_{0:k}  \beta_{0:k}^\star \\
        &=  \left\| \Sigma_{T,k:d}^{\frac{1}{2}} X_{k:d}^T  (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k} \pth{I_k +X_{0:k}^T (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k} }^{-1} \beta_{0:k}^\star \right\|^2 \\
        &\leq \|\Sigma_{T,k:d}\| \left\| (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{k:d}X_{k:d}^T  (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1}  \right\| \\
        &\quad\cdot \left\|  X_{0:k} \pth{I_k +X_{0:k}^T (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k} }^{-1} \beta_{0:k}^\star  \right\|^2 \\
        &=  \|\Sigma_{T,k:d}\| \left\| (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{k:d}X_{k:d}^T  (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1}  \right\| \\
        &\quad\cdot \left\|  X_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}} \pth{\Sigma_{S,0:k}^{-1} +\Sigma_{S,0:k}^{-\frac{1}{2}}X_{0:k}^T (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k}\Sigma_{S,0:k}^{-\frac{1}{2}} }^{-1}\Sigma_{S,0:k}^{-\frac{1}{2}} \beta_{0:k}^\star  \right\|^2 \\
        &\leq  \|\Sigma_{T,k:d}\| \left\| (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1}  \right\| \left\| \Sigma_{S,0:k}^{-\frac{1}{2}}X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}} \right\| \\
        &\quad\cdot \left\| \pth{\Sigma_{S,0:k}^{-1} +\Sigma_{S,0:k}^{-\frac{1}{2}}X_{0:k}^T (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k}\Sigma_{S,0:k}^{-\frac{1}{2}} }^{-2} \right\| (\beta_{0:k}^\star)^T \Sigma_{S,0:k}^{-1}\beta_{0:k}^\star.
    \end{align*}
    In particular,
    \begin{align*}
        &\quad \left\| \pth{\Sigma_{S,0:k}^{-1} +\Sigma_{S,0:k}^{-\frac{1}{2}}X_{0:k}^T (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k}\Sigma_{S,0:k}^{-\frac{1}{2}} }^{-1} \right\| \\
        &\leq \left\| \pth{\Sigma_{S,0:k}^{-\frac{1}{2}}X_{0:k}^T (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k}\Sigma_{S,0:k}^{-\frac{1}{2}} }^{-1} \right\| \\
        &\leq \left\| X_{k:d}X_{k:d}^T + \lambda I_n \right\| \left\| \pth{\Sigma_{S,0:k}^{-\frac{1}{2}}X_{0:k}^TX_{0:k}\Sigma_{S,0:k}^{-\frac{1}{2}} }^{-1} \right\| \\
        &\leq c_x\pth{\lambda + \sum_{j>k}\lambda_j} \frac{c_x}{n} \\
        &= \frac{c_x^2}{n}\pth{\lambda + \sum_{j>k}\lambda_j}.
    \end{align*}
    The second inequality follows from $\mu_{\text{min}}(ABA^T) \geq \mu_{\text{min}}(B)\mu_{\text{min}}(AA^T)$ where the matrix $B$ is positive definite.
    
    Therefore,
    \begin{align*}
        &\quad (\beta_{0:k}^\star)^TX_{0:k}^T(XX^T+\lambda I_n)^{-1} X_{k:d} \Sigma_{T,k:d} X_{k:d}^T (XX^T+\lambda I_n)^{-1} X_{0:k}  \beta_{0:k}^\star \\
        &\leq \|\Sigma_{T,k:d}\| \left\| (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1}  \right\| \left\| \Sigma_{S,0:k}^{-\frac{1}{2}}X_{0:k}^TX_{0:k} \Sigma_{S,0:k}^{-\frac{1}{2}} \right\| \\
        &\quad\cdot \left\| \pth{\Sigma_{S,0:k}^{-1} +\Sigma_{S,0:k}^{-\frac{1}{2}}X_{0:k}^T (X_{k:d}X_{k:d}^T + \lambda I_n)^{-1} X_{0:k}\Sigma_{S,0:k}^{-\frac{1}{2}} }^{-2} \right\| (\beta_{0:k}^\star)^T \Sigma_{S,0:k}^{-1}\beta_{0:k}^\star \\
        &\leq  \|\Sigma_{T,k:d}\| \cdot \pth{\frac{1}{c_xL}\pth{\lambda+\sum_{j>k}\lambda_j}}^{-1} \cdot c_xn \cdot \frac{c_x^4}{n^2}\pth{\lambda + \sum_{j>k}\lambda_j}^2 \cdot  (\beta_{0:k}^\star)^T \Sigma_{S,0:k}^{-1}\beta_{0:k}^\star \\
        &= \frac{c_x^6}{n} L \pth{\lambda+\sum_{j>k}\lambda_j} \|\Sigma_{T,k:d}\|(\beta_{0:k}^\star)^T \Sigma_{S,0:k}^{-1}\beta_{0:k}^\star.
    \end{align*}
    
\end{proof}

\subsection{Main Results}
\begin{theorem}
Suppose the assumption condNum$(k,\delta,L)$~(Assumption~\ref{assum:condNum}) is satisfied. There exists a constant $c_x>2$ depending only on $\sigma_x$, such that for any $c_xN_1<n<N_2$, with probability at least $1-2\delta-c_xe^{-n/c_x}$,
\begin{align*}
    \frac{V}{c_x\sigma^2} &\leq  \frac{L^2}{n} \tr \qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}} + L^2n\big(\lambda+\sum_{j>k}\lambda_j\big)^{-2} \tr\qth{\Sigma_{S,k:d}^{\frac{1}{2}}\Sigma_{T,k:d} \Sigma_{S,k:d}^{\frac{1}{2}} }.  \\
    \frac{B}{c_x} &\leq (\beta^\star_{0:k})^T\Sigma_{S,0:k}^{-1} \beta^\star_{0:k} \Big[ \frac{1}{n^2} \big(\lambda+\sum_{j>k}\lambda_j\big)^2 \left\|\Sigma_{S,0:k}^{-\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}   \right\| + \frac{L}{n} \big(\lambda+\sum_{j>k}\lambda_j\big) \|\Sigma_{T,k:d}\| \Big] \\
    & + (\beta^\star_{k:d})^T\Sigma_{S,k:d}\beta^\star_{k:d} \Big[  L^2 \left\| \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}\right\| + Ln \big(\lambda+\sum_{j>k}\lambda_j\big)^{-1}\|\Sigma_{T,k:d} \| \Big] \\
    & +  (\beta^\star_{k:d})^T\Sigma_{T,k:d}\beta^\star_{k:d}.
\end{align*}
$N_1,N_2$ are defined as follows:
\begin{equation*}
    \begin{alignedat}{2}
    N_1 &= \max \Bigg\{ 
        & & \big( k + \ln \frac{1}{\delta} \big) \lambda_1^4 \lambda_k^{-4}, \\
        & && L \lambda_1 \lambda_k^{-2} \big(\lambda+\sum_{j>k} \lambda_j\big), \\
        & && \big( k + \ln \frac{1}{\delta} \big) \lambda_1^6 \lambda_k^{-8} \|\Sigma_{T,0:k}\|^2 k^2 
        \left( \tr \left[ \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} 
        \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right] \right)^{-2}, \\
        & && L \lambda_1^2 \lambda_k^{-4} \big( \lambda+\sum_{j>k} \lambda_j \big) \|\Sigma_{T,0:k}\| k 
        \left( \tr \left[ \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} 
        \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right] \right)^{-1}
    \Bigg\}, \\
    N_2 &= \lambda_{k+1}^{-1} & & \big(\lambda+\sum_{j>k} \lambda_j\big).
    \end{alignedat}
    \end{equation*}
\end{theorem}
\begin{proof}
The theorem follows from Lemma~\ref{lem:all_concentration}, Lemma~\ref{lem:var_0k}, Lemma~\ref{lem:var_kd}, Lemma~\ref{lem:bias_0k_1}, Lemma~\ref{lem:bias_0k_2}, Lemma~\ref{lem:bias_kd_1} and Lemma~\ref{lem:bias_kd_2}. For a constant $c_x'>2$ depending only on $\sigma_x$, these lemmas hold for values of $n$ that satisfy the following inequalities:
\begin{align*}
    n &> 4c_x'^4(k+\ln(1/\delta))\lambda_1^2\lambda_k^{-2}, \\
    n &> 2c_x'^4L \lambda_k^{-1}\pth{\lambda+\sum_{j>k}\lambda_j}, \\
    n &> 4c_x'^4 \left( k + \ln \frac{1}{\delta} \right) \lambda_1^4 \lambda_k^{-4}, \\
    n &> 2c_x'^4 L \lambda_1 \lambda_k^{-2} \pth{\lambda+\sum_{j>k}\lambda_j}, \\
    n &> 4c_x'^4 \left( k + \ln \frac{1}{\delta} \right) \lambda_1^6 \lambda_k^{-8} \|\Sigma_{T,0:k}\|^2 k^2 
        \left( \tr \left[ \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} 
        \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right] \right)^{-2}, \\
    n &> 2c_x'^4 L \lambda_1^2 \lambda_k^{-4} \left( \lambda+\sum_{j>k} \lambda_j \right) \|\Sigma_{T,0:k}\| k 
        \left( \tr \left[ \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} 
        \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right] \right)^{-1}, \\
    n &> 2c_x'^3 (\lambda +\sum_{j>k} \lambda_j) \lambda_1 \lambda_k^{-2}, \\
    n &> 4c_x'^4\pth{k+\ln\frac{1}{\delta}}\lambda_1^6 \lambda_k^{-8}\|\Sigma_{T,0:k}\|^2 \left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}   \right\|^{-2}, \\
    n &> 2c_x'^4L \pth{\lambda+\sum_{j>k} \lambda_j} \lambda_1^2\lambda_k^{-4} \|\Sigma_{T,0:k}\| \left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}   \right\|^{-1}, \\
    n &< \lambda_{k+1}^{-1} \left( \lambda+\sum_{j>k} \lambda_j \right).
\end{align*}
A sufficient condition for all the inequalities above is given by $4c_x'^4N_1<n<N_2$. This follows from the following facts:
\begin{align*}
    \lambda_1\lambda_k^{-1} &\geq 1, \\
    c_x' &> 2, \\
    L&\geq1, \\
    k \left( \tr \left[ \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} 
        \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right] \right)^{-1} &\geq \left\|\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}   \right\|^{-1}.    
\end{align*}
Then, with probability at least $1-2\delta-c_x'e^{-n/c_x'}$:
\begin{align*}
    V &\leq 16\sigma^2(1+c_x'^4L^2)\frac{1}{n} \tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}} \\
    &\quad + \sigma^2 c_x'^3L^2n \pth{\lambda+\sum_{j>k} \lambda_j}^{-2} \tr\qth{\Sigma_{S,k:d}^{\frac{1}{2}}\Sigma_{T,k:d} \Sigma_{S,k:d}^{\frac{1}{2}} } \\
    &\leq 32\sigma^2c_x'^4L^2\frac{1}{n} \tr\qth{\tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1}} \\
    &\quad + \sigma^2 c_x'^3L^2 n \pth{\lambda+\sum_{j>k}\lambda_j}^{-2} \tr\qth{\Sigma_{S,k:d}^{\frac{1}{2}}\Sigma_{T,k:d} \Sigma_{S,k:d}^{\frac{1}{2}} }, \\
    B &\leq \frac{16c_x'^4}{n^2} \pth{\lambda +  \sum_{j>k} \lambda_j}^2 (\beta^\star_{0:k})^T \Sigma_{S,0:k}^{-1}   \beta^\star_{0:k} 
    \left\|\Sigma_{S,0:k}^{-\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}   \right\| \\
    &\quad + 32c_x'(1+c_x'^4L^2)  \left\| \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right\|  (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d} \\
    &\quad + 3c_x'^2L \pth{\lambda + \sum_j \lambda_j}^{-1} n \|\Sigma_{T,k:d}\| (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d} \\
    &\quad + 3\frac{c_x'^6}{n} L \pth{\lambda+\sum_{j>k}\lambda_j} \|\Sigma_{T,k:d}\|(\beta_{0:k}^\star)^T \Sigma_{S,0:k}^{-1}\beta_{0:k}^\star \\
    &\quad + 3 (\beta_{k:d}^\star)^T\Sigma_{T,k:d}\beta_{k:d}^\star \\
    &\leq 16c_x'^4\frac{1}{n^2} \pth{\lambda + \sum_{j>k} \lambda_j}^2 \left\|\Sigma_{S,0:k}^{-\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{-\frac{1}{2}}  \right\| 
    (\beta^\star_{0:k})^T \Sigma_{S,0:k}^{-1}   \beta^\star_{0:k} \\
    &\quad + 64c_x'^5L^2  \left\| \tilde{\Sigma}_{S,0:k}^{-1} \Sigma_{S,0:k}^{\frac{1}{2}} \Sigma_{T,0:k} \Sigma_{S,0:k}^{\frac{1}{2}} \tilde{\Sigma}_{S,0:k}^{-1} \right\|  (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d} \\ 
    &\quad + 3c_x'^2L n \pth{\lambda + \sum_j \lambda_j}^{-1}  \|\Sigma_{T,k:d}\| (\beta^\star_{k:d})^T \Sigma_{S,k:d} \beta^\star_{k:d} \\
    &\quad + 3c_x'^6L\frac{1}{n} \pth{\lambda + \sum_{j>k}\lambda_j} \|\Sigma_{T,k:d}\|(\beta_{0:k}^\star)^T \Sigma_{S,0:k}^{-1}\beta_{0:k}^\star \\
    &\quad + 3 (\beta_{k:d}^\star)^T\Sigma_{T,k:d}\beta_{k:d}^\star.
\end{align*}
By taking $c_x = 64c_x'^6$, the proof is complete.
\end{proof}

